PERKS: a Locality-Optimized Execution Model for Iterative Memory-bound GPU Applications

Iterative memory-bound solvers commonly occur in HPC codes. Typical GPU implementations have a loop on the host side that invokes the GPU kernel as much as time/algorithm steps there are. The termination of each kernel implicitly acts the barrier required after advancing the solution every time step. We propose an execution model for running memory-bound iterative GPU kernels: PERsistent KernelS (PERKS). In this model, the time loop is moved inside persistent kernel, and device-wide barriers are used for synchronization. We then reduce the traffic to device memory by caching subset of the output in each time step in the unused registers and shared memory. PERKS can be generalized to any iterative solver: they largely independent of the solver's implementation. We explain the design principle of PERKS and demonstrate effectiveness of PERKS for a wide range of iterative 2D/3D stencil benchmarks (geomean speedup of $2.12$x for 2D stencils and $1.24$x for 3D stencils over state-of-art libraries), and a Krylov subspace conjugate gradient solver (geomean speedup of $4.86$x in smaller SpMV datasets from SuiteSparse and $1.43$x in larger SpMV datasets over a state-of-art library). All PERKS-based implementations available at: https://github.com/neozhang307/PERKS.

==> 02_5_motivation_NOT_USED.tex <==

\section{Motivation}
\color{blue}




\subsection{Resources Usage}\label{sec:resource}



\textbf{\textit{No need all on-chip resources be occupied to saturate a device.} }
Take our double precision js2d5pt stencil implementation as an example. We used spacial blocking and shared memory to optimized it achieve 72.8\% of theoretical peak performance in A100 in a domain size of ($ 2304\times 2304$). In the same setting, we varied the concurrently running thread block per stream multiprocessor (TB/SM) and plot its performance in Fig~\ref{Fig:showcase}. We plot the remaining resources for each TB/SM. 
As the Fig~\ref{Fig:showcase} shows, as TB/SM decreases, the performance of js2d5pt decrease a little bit (73.4-62.5 GCells/s). 
At the same time, freed shared memory and registers gradually increased. Even at its peak performance setting, about 16.8 MB of shared memory and register files are not in use. 
But because register per thread is 44 in this situation, it is not possible to consume all resources at any setting. So the answer for first question is: no need to use all on-chip resources to saturate a device. 

\textbf{\textit{Then what to do with these resources remained?}} Many researchers focused on squeezing these resources with complicated parallel algorithms\lingqi{note to self: find citation}. Instead of proposing a new complex algorithm, \textbf{why don't we use these remained resources to hold or cache data?} To illustrate the potential of this simple idea, we plot the project performance by using the remaining resources to cache data in js2d5pt in the save figure. Fig~\ref{Fig:showcase} shows that simply using half of remained registers might produce 2.37x speedup.  

Even though this idea is simple, the obstacle is that: 1) Currently GPU programming relies heavily on launching sequences of kernel functions; 2) Yet the on-chip resources are doomed to be reset between different kernel functions. To solve this issue, an alternative way to program with kernel persisted, and a new assumption for CUDA execution model is necessary.

% \begin{comment}
\subsection{Why PERKS now}
\lingqi{Wahib: I think Execution Model defines the behavior of thread block and grids. Yet I think this could not well emphasize the main contribution in this paper. I think, persistent kernel is easily come up idea, given grid synchronization. But making register and shared memory (as a whole) persistent too, showing potential cache schema, showing potential programmability(todo), performance model and evaluation, wouldn't be some idea easily come up with. And we might additionally bring a question about the trade of between concurrency and resource to cache. I think a "method" or "a way to program" could not summarize the research, "scheme" might not enough too, I put my idea here in case we might come better expression}
\wahib{@Lingqi: What you are listing above is the challenges against making PERKS works, and not contributions. And yes indeed, we need to emphasize that. I will add a "challenges" paragraph to add to the introduction section}

% \lingqi{Motivation, performance model, and evaluation plan to express as such narrative: any baseline (concurrency enough or not enough ->(resource remained)->PERKS(might reduce concurrency, yet performance model could )->(concurrency not enough)->optimization)}
% \lingqi{Original paper (for PPoPP) assume that baseline should have enough concurrency. But I think this might not be that practical for most of audiences. (And some of current kernel seems not that optimized either)}

The existing GPU Execution Model only defines the behavior of parallel components. It does do expose enough details for on-chip resources, i.e. registers and shared memory, especially when these resources can be shared between functions. 

Why people haven't noticed this disadvantage in existing Execution Model? One reason might be that the on-chip resources haven't increased to current size that its performance should not be negligible. Another reason is that a "function" or "method" usually equals to a single kernel, for the purpose of programmability. Two reasons why people usually draw equate these concepts: 1) kernel launch with order can act as an implicit device-wide synchronization; 2) a kernel has its own parallel parameters, different task or different functions might need different parallel parameters. The first issue is solve by latest CUDA APIs for cooperative group. The grid-level synchronization provided by CUDA APIs can be an alternative way fro device-wide synchronization. For the second issue, admittedly, it is still a problem. And an unsuitable parameter might cause lower concurrency to fully utilize the device. However, Fig~\ref{Fig:showcase} could well represent that in certain situations performance brought by increasing usable resources might be more significant then increasing concurrency. This is especially true when facing a memory-bound problem. 

% Yet the question remains that whether equating kernel and function is an appropriate design. Too illustrate it, kernel is a concept in execution model yet function is a concept in programming model. Messing these tow concept together might limit the potential of performance of the hardware. More specifically, many kernel fusion related research (\lingqi{note to self: find cite}) proves that sequences of simple kernel functions would cause insufficient resource usage.

% Another disadvantage is that after the life time of a single kernel, all on-chip resources will be wiped out. As Section~\ref{sec:resource} analyzed, these resources can potentially benefit performance by simply use them to cache data that would otherwise need to be either reload or recompute again in future kernel functions. 

% Admittedly, kernel also works as an implicit logic barrier to ensure the order of sequence of logical kernel functions. Yet the latest CUDA APIs for cooperative group can perfectly replace this implicit barrier with negligible performance difference~\cite{zhang2020study}. In fact. these new APIs open a possibility for new Execution Model that free kernel from the concept of "function". This new Execution Model can further expose nontrivial hardware features to programmers for better performance. 
Thereafter, we proposed PERsistent Kernels (PERKS) for iterative solvers on GPUs to improve performance by exposing the large capacity of register files and shared memory for advanced optimization. We mainly focus on iterative solvers, as the performance benefit is magnified by time-steps. Yet this method can be generalized to any situations when leveraging on-chip resources is necessary between functions.
%Thereafter, we proposed PERsistent Kernels (PERKS) as an execution model for iterative solvers on GPUs to improve 
%data locality performance by taking advantage of the large capacity of register files and shared memory. 
% \lingqi{Make it more generalize}
As Figure~\ref{fig:exemodel} illustrates, in PERKS we move the time stepping loop from the host to the device, and use grid synchronization as the device-wide barrier at each time step. We then use the register files and shared memory to reduce traffic to the device memory by caching the domain (or a subset from it) in-between time steps. 

Considering the trends of increasing resources as mentioned in Section~\ref{sec:trend}, the potential performance benefit brought by PERKS will also increase as time goes by. 


% \lingqi{note to self: add CG}
%Despite any blocking method utilized, temporal and location dependency exist between adjacent blocks. 

% We choose to work on stencil because the temporal and spatial dependency in stencil 


% Temporal and spatial dependency is consistent 
% in stencil, despite any blocking methods applied. 

% \end{comment}
\color{black}


==> 03_5performance_model_NOT_USE.tex <==

\section{Performance Analysis}\label{sec:simplepermodel}
%\lingqi{QUESTION: seems like peak performance not as important as concurrency analysis}


%\lingqi{Question: we need peak and conc}
%\chen{show the purpose of the performance model at the first sentences including why the perf. model is needed in this paper.}
%\begin{itemize}[leftmargin=3mm]
%\revision{\chen{In this section, we build a performance model to show the theoretical peak performance of PERK. Also, we can analyze the impact of different parameters on the performance of PERK. Hence, we can qualify the implementation quality by comparing our performance with the projected peak results.}

In this section, \revisiona{we conduct analysis to answer the following questions.}
% we propose a performance model that serves the following purposes.

First, \revisiona{\textbf{how to quantify the quality of our implementations?}} We propose a projection of achievable performance that we compare with measured results to detect abnormal behavior or implementation shortcomings. We relied on this projection in the analysis of our PERKS implementation quality (Section~\ref{sec:peakperform}).
%{\item\lingqi{Provide simple model to project performance of PERKS (Section~\ref{sec:projectionmodel} or Equation~\ref{eqt:projectionLarge})} \wahib{@Lingqi@:this point is similar to the previous point, so please merge.}}
%\item Identifying limitations of caching schemes and shortcomings of caching policies (Section~QQ).\lingqi{I don't know what to do with it}

Second, \revisiona{\textbf{is oversubscription necessary?}} We identify the bounds on reducing concurrency before dropping performance and use concurrency to explain potential optimizations for further performance improvement (Section~\ref{sec:conan}). 
% the feasibility of PERKS in practice, 

\revisiona{\textbf{We emphasize that:}} we use the analysis to understand the quality of our implementation and address its implication on performance.
{\revisiona{However,} the concurrency analysis is not a requirement for porting kernels to PERKS;  In contrast, end-users wishing to port the kernel to PERKS need only to satisfy the concurrency requirements by setting the device occupancy\footnote{\revision{Occupancy in CUDA is the ratio of active warps to the maximum number of warps supported on a given device. Occupancy can be controlled, manually or by auto-tuning~\cite{kerneltuner,shende2006tau,adhianto2010hpctoolkit} by changing the grid and thread block sizes (subject to constraints of resources).}} to minimum occupancy while maintaining performance \revisiona{(See\ref{sec:enduser})}. }
%\revision{
%We use these analyses to understand the feasibility of PERKS in practice and address its performance concern. 
% End-user readers can refer to Section~\ref{sec:enduser}.
%}
%\item Identifying the bounds on reducing concurrency before dropping performance (Section~MM).
%\item Using concurrency to explain potential optimizations for further performance improvement (Section~\ref{sec:perconcurrency}). 
%\item Analyzing the trade-off between the registers required for maintaining the desirable concurrency in the kernels and registers designated for caching (Section~\ref{sec:regtradeoff}).

%\color{blue}
%The purpose of this section lists as follow:
%\begin{itemize}
%    \item Project the performance before start adapting existing kernel to PERKS \item Judge how optimize the PERKS kernel is. 
%    \item Use concurrency to explain the potential way for further performance optimization
%    \item analyze the trade of between more concurrency and more register for cache.
%\end{itemize}

% \lingqi{might need to optimize}
% \lingqi{Note to self: add plugin to this section}
% \textbf{Premise}


%concurrency $C$ that combines
%{code}
% that usually not strictly equal to $P$
\subsection{Overview}
%\wahib{Note to self: remove parameter $M$ and adjust accordingly.}
This performance \revisiona{analysis} relies on three performance attributes: a) measured performance $\mathbb{M}$ of our PERKS implementation, b) the projected peak performance $\mathbb{P}$ achievable on a given GPU,  and c) the efficiency function $\mathfrak{E()}$ describing the efficiency of the given kernel running on the device.
%\revision{gap} between $\mathbb{P}$ and $\mathbb{M}$. 
More specifically, $\mathfrak{E()}$ is a function of the concurrency exposed by the software $\mathbb{C}_{sw}$ and the concurrency required by the hardware $\mathbb{C}_{hw}$. The relation of measured performance to projected peak performance becomes:
%Eff(C_{code},C_{hw})  
%\color{blue}
\begin{equation}\footnotesize
   \mathbb{M}  =  \mathbb{P}\times \mathfrak{E(} \revision{\mathbb{C}_{sw}},\mathbb{C}_{hw}\mathfrak{)}
    \label{eqt:basic}
\end{equation}
%Section~\ref{sec:peakperform}
We discuss projected peak performance in the following section. A detailed discussion of the efficiency and concurrency functions is in Section~\ref{sec:perconcurrency}.


\subsection{Projecting Peak Achievable Performance}\label{sec:peakperform}
We rely on the FOM (Figure Of Merit) as the performance metric in this analysis. In stencils, we use the giga-cells updated per second (GCells/s)~\cite{DBLP:conf/cgo/MatsumuraZWEM20,chen2019versatile}. Given the memory-bound nature of the conjugate gradient solver, we directly use sustained memory bandwidth as a metric, following other works on conjugate gradient~\cite{anzt2020ginkgo}. Due to space limitations, this section mainly focuses on stencils to explain the performance analysis. Without loss of generality, the analysis is applicable to other cases (ex: conjugate gradients) by adjusting the performance metric and code concurrency accordingly.

We use a simple performance model inspired by the roofline model~\cite{ofenbeck2014applying,kim2011performance}. The model's utility is to project the upper bound on performance based on the reduction of global memory traffic. This model, in turn, helps us in this paper to identify performance gaps in our PERKS implementation and later inspect the reasons for those gaps (e.g., register spilling). 



% \subsubsection{Baseline}
% To show that the baseline implementation is enough optimized, the peak performance for baseline is analyzed in this subsection. By assuming that the bottleneck is global memory bandwidth, and all memory transactions are coalesced, baseline performance can be computed based on the memory bandwidth. 
In a kernel implemented as PERKS, the bottleneck could either be the global memory bandwidth or the shared memory bandwidth (if the PERKS caching scheme moves the bottleneck to become the shared memory bandwidth). We don't assume the registers to be a bottleneck since we assume that as long as we ensure that no register spilling occurs, we avoid register pressure.

%\wahib{Note to self: revise to reduce and simplify. Use a single case to avoid confusion.}
\begin{comment}

We first consider the case where we either only use global memory or only use shared memory. Assumes to compute a \revision{2D} domain with $D$ comprised of $M\cdot N$ total cells.% with total cell amount $Cell$:
%\begin{equation}\footnotesize
%    \begin{aligned}
%        Cell=D
%    \end{aligned}
%\end{equation}
The memory access per cell is $Apc$. The total memory access amount is $T=Cell\cdot Apc$. 
Latency $L$ can be computed based on memory bandwidth $B$, total cell amount $Cell_{total}$, memory access per cell $Apc$ and type size $S(type)$:
\begin{equation}\footnotesize
    \begin{aligned}
        L=\frac{{Cell\cdot S(type)\cdot Apc}}{{B}} \\ 
    \end{aligned}
    \label{eqt:latency}
\end{equation}
Throughput $Thr$ can be further compute based on Latency $L$:
\begin{equation}\footnotesize
    \begin{aligned}
  Thr=\frac{Cell}{L}  =\frac{B}{S(type)\cdot Apc}
    \end{aligned}
    \label{eqt:throughput}
\end{equation}

{\color{blue}


For example, assume that computing js2d5pt single precision stencil with a100 GPU, in which global memory bandwidth is 1555 GB/s, shared memory bandwidth is 19.5 TB/s ($Freq\cdot band\cdot smx\_amount$). Ideally, only one store and one load operation is necessary for single cell operation. Thus $Apc_{global}=2$. From shared memory perspective, ideally, 1 store and 3 load is necessary per cell for computing js2d5pt. Thereby, $Apc_{sm}=4$.

If global memory is the bottleneck, 
% $Thr_{global}={B_{global}}/{(sizeof(float))\times{2})}=194.38 GCells/s$,
$Thr_{global}=194.4 GCells/s$, based on Equation~\ref{eqt:throughput}. 
The measured performance for our baseline implementation is $137.6 GCells/s$ (70.8\% of theory). 

If shared memory is the bottleneck, based on Equation~\ref{eqt:throughput}, 
% $Thr_{sm}={B_{sm}}/{(sizeof(float))\times{4}}=1.22 TCells/s$. 
$Thr_{sm}=1.22 TCells/s$. 
The measured performance for PERKS when whole domain is cached is $566 GCells/s$ (46.4\% of theory).
}
	
\end{comment}
%This depends on implementations. 
% \subsubsection{PERKS}
%In situations of PERKS, that use shared memory and registers to cache portion of domain.

We initially do not account for the memory accesses to global memory originating from the boundary threads in each thread block, e.g., halo region in stencil, and confine our analysis to the dependency in cached region. We then expand our analysis to consider those unavoidable global memory accesses (Equation~\ref{eqt:perkhalo}).%\wahib{Note to self: add pointer to where we account for the accesses to global memory.} 

%To simplify the analysis, we firstly dismiss the dependency in cached region that require memory access to global memory, e.g. halo region in stencil. 

We assume a total domain of size $\mathbb{D}$ bytes, the cached portion to be $\mathbb{D}_{cache}$ bytes, and the uncached portion to be {\footnotesize$\mathbb{D}_{uncache}=\mathbb{D}-\mathbb{D}_{cache}$} bytes. The cached portion of the domain data would be divided between registers and shared memory (since we cache in both registers and shared memory): {\footnotesize$\mathbb{D}_{cache}=\mathbb{D}^{sm}_{cache}+\mathbb{D}^{reg}_{cache}$}. For $N$ time steps, \revision{a}ssuming the number of bytes stored to global memory in each time step is $\mathbb{S}_{gm}$ and the number of bytes loaded is $\mathbb{L}_{gm}$, the total global memory bytes accessed $\mathbb{A}_{gm}$ becomes:
%\begin{equation}\footnotesize
%    \mathbb{L}_{global}(i)= 
%\begin{cases}
%    \mathbb{D}_{total},& \text{if } i= 0\\
%    \mathbb{D}_{global}, & \text{otherwise}
%\end{cases}
%\end{equation}
%\begin{equation}\footnotesize
%    \mathbb{S}_{global}(i)= 
%\begin{cases}
%    \mathbb{D}_{total},& \text{if } i= n-1\\
%    \mathbb{D}_{global}, & \text{otherwise}
%\end{cases}
%\end{equation}
\begin{equation}\footnotesize
\begin{aligned}
    %\mathbb{A}^{gm}(\mathbb{D})&=\sum_{i=0}^{n-1}(\mathbb{L}^{gm}(i)+\mathbb{S}^{gm}(i))\\
    %&=2\cdot n\cdot \mathbb{D}_{uncache} + 2\cdot  \mathbb{D}_{cache}
    %\mathbb{A}_{gm}(\mathbb{D})&=N\cdot(\mathbb{L}_{gm}+\mathbb{S}_{gm})\\
    %&=2\cdot N\cdot \mathbb{D}_{uncache} + 2\cdot  \mathbb{D}_{cache}
    \mathbb{A}_{gm}(\mathbb{D})=N\cdot(\mathbb{L}_{gm}+\mathbb{S}_{gm})
    &=2\cdot N\cdot \mathbb{D}_{uncache} + 2\cdot  \mathbb{D}_{cache}    
%    \\
%    &\stackrel{\text{n is large enough}}{\approx} 2\cdot n\cdot \mathbb{D}_{global}
\end{aligned}
\end{equation}


In the case when the kernel is bounded by global memory bandwidth, i.e., the volume of cached data does not move the bottleneck from global memory to shared memory, for the global memory bandwidth of $\mathbb{B}_{gm}$ and data type size of $\mathfrak{S}(type)$, the time $\mathbb{T}_{gm}(\mathbb{D})$ for accessing the global memory becomes:%can be computed base on Equation~\ref{eqt:time}:

\begin{equation}\footnotesize
    \begin{aligned}
        %\mathbb{T}_{gm}(\mathbb{D})=\frac{{\mathbb{A}_{gm}(\mathbb{D})\cdot \mathfrak{S}(type)}}{{\mathbb{B}_{gm}}}
                \mathbb{T}_{gm}(\mathbb{D})={{\mathbb{A}_{gm}(\mathbb{D})\cdot \mathfrak{S}(type)}}/{{\mathbb{B}_{gm}}}
    \end{aligned}
    \label{eqt:time_gm}
\end{equation}

In the case when the kernel is bounded by shared memory bandwidth, i.e., the volume of data cached in shared memory moves the bottleneck to be the shared memory bandwidth, the total shared memory (in bytes) accessed $\mathbb{A}_{sm}$ becomes: %we assume the algorithm that we plan to apply PERKS be $\mathbb{ALG}$. PERKS won't influence the shared memory access amount of $\mathbb{ALG}$ per time step, which can be assumed as $\mathbb{A}^{sm}(\mathbb{ALG})$. 
%But some additional memory access within cached with shared memory region $\mathbb{A}^{sm}(\mathbb{D}^{sm}_{cache})$ exists if caching data in shared memory. Similar to global memory access we can get: 

\begin{comment}
\begin{equation}\footnotesize
    \mathbb{L}_i(sm)= 
\begin{cases}
    0,& \text{if } i= 0\\
    \mathbb{D}_{sm}, & \text{otherwise}
\end{cases}image.png
\end{equation}
\begin{equation}\footnotesize
    \mathbb{S}_i(sm)= 
\begin{cases}
    0,& \text{if } i= n-1\\
    \mathbb{D}_{sm}, & \text{otherwise}
\end{cases}
\end{equation}
\end{comment}

\begin{equation}\footnotesize
\begin{aligned}
    %\mathbb{A}_{sm}(\mathbb{D}_{cache}^{sm})&=N\cdot(\mathbb{L}_{sm}+\mathbb{S}_{sm})\\
    %				&=2\cdot (N-1)\cdot \mathbb{D}_{cache}^{sm}
    \mathbb{A}_{sm}(\mathbb{D}_{cache}^{sm})=N\cdot(\mathbb{L}_{sm}+\mathbb{S}_{sm})
    				=2\cdot (N-1)\cdot \mathbb{D}_{cache}^{sm}    				
    %\mathbb{A}^{sm}(\mathbb{D}_{cache})&=\sum_{i=0}^{n-1}(\mathbb{L}^{sm}(i)+\mathbb{S}^{sm}(i))\\
    %				&=2\cdot (n-1)\cdot \mathbb{D}^{sm}_{cache}
\end{aligned}
\end{equation}


%Additionally, given that the global memory bandwidth is $\mathbb{B}^{sm}$ and the data type size is $\mathfrak{S}(type)$, the time $\mathbb{T}$ for accessing the global memory can be computed base on Equation~\ref{eqt:time}:
Assuming $\mathbb{A}_{sm}(\mathbb{KERNEL})$ to be the shared memory originally used by the kernel, e.g., shared memory used in the baseline implementation of a stencil kernel to improve the locality, and $\mathbb{B}_{sm}$ to be the shared memory bandwidth, the time $\mathbb{T}_{sm}(\mathbb{D})$ for accessing the shared memory becomes:

\begin{equation}\footnotesize
    \begin{aligned}
        %\mathbb{T}_{sm}(\mathbb{D}_{cache}^{sm})=\frac{{(\mathbb{A}_{sm}(\mathbb{D}_{cache}^{sm})+\mathbb{A}_{sm}(\mathbb{KERNEL}))\cdot \mathfrak{S}(type)}}{{\mathbb{B}_{sm}}}
        \mathbb{T}_{sm}(\mathbb{D}_{cache}^{sm})=\{{{(\mathbb{A}_{sm}(\mathbb{D}_{cache}^{sm})+\mathbb{A}_{sm}(\mathbb{KERNEL}))\cdot \mathfrak{S}(type)}}\}/{{\mathbb{B}_{sm}}}
    \end{aligned}
    \label{eqt:time_sm}
\end{equation}


%The time $\mathbb{T}_{domain}$ for accessing the domain, Assuming perfect overlapping, in PERKS is:
%
%\begin{equation}\footnotesize
%    \begin{aligned}
%     \mathbb{T}_{domain}=\max(\mathbb{T}_{global},\mathbb{T}_{{sm}}
%    \end{aligned}
%    \label{eqt:maxlat}
%\end{equation}

Next, we consider the unavoidable global memory accesses necessary to resolve the neighborhood dependencies in $\mathbb{D}_{cache}$, e.g., the halo region of stencils. In the cached portion of the domain, the halo region requires global memory accesses to resolve the dependencies. Assuming the global memory accesses, in bytes, for the halo region of the data computed by the boundary threads in thread blocks that are in the cached portion of the domain to be $\mathbb{A}_{gm}(\mathfrak{H}(\mathbb{D}_{cache}))$, the time for accessing those halo region $\mathbb{T}_{gm}(\mathfrak{H}(\mathbb{D}_{cache}))$ would be:

\begin{equation}\footnotesize
    \begin{aligned}
    % \mathbb{T}_{gm}(\mathfrak{H}(\mathbb{D}_{cache}))=\frac{\mathbb{A}(\mathfrak{H}(\mathbb{D}_{cache}))\cdot \mathfrak{S}(type)}{\mathbb{B}_{gm}}
          \mathbb{T}_{gm}(\mathfrak{H}(\mathbb{D}_{cache}))={\mathbb{A}(\mathfrak{H}(\mathbb{D}_{cache}))\cdot \mathfrak{S}(type)}/{\mathbb{B}_{gm}}
    \end{aligned}
    \label{eqt:perkhalo}
\end{equation}
The projected best-case total time required for the PERKS kernel may be written as:

\begin{equation}\footnotesize
    \begin{aligned}
     \mathbb{T}_{PERKS}=\max(\mathbb{T}_{gm}(\mathbb{D})+\mathbb{T}_{gm}(\mathfrak{H}(\mathbb{D}_{cache})),\mathbb{T}_{{sm}})
    \end{aligned}
    \label{eqt:maxlat}
\end{equation}

Accordingly, the projected peak performance ($\mathbb{P}$ in Equation~\ref{eqt:basic}) for the $N$ time steps can be expressed as:

\begin{equation}\footnotesize
    \begin{aligned}
     %\mathbb{P}=\frac{\mathbb{D} \cdot N}{\mathbb{T}_{PERKS}}
     \mathbb{P}={\mathbb{D} \cdot N}/{\mathbb{T}_{PERKS}}
     %\mathbb{P}_{PERKS}=\frac{\mathbb{D} \cdot n}{\mathbb{T}_{PERKS}}
    \end{aligned}
    \label{eqt:maxpeak}
\end{equation}


To further illustrate how this performance analysis works, we give two examples while computing $N=1000$ time-steps of a single precision 2D 5-point Jacobi stencil on A100. 

We use the domain size $\mathbb{D}=3072^2$ as an example of a large domain size; the total cache-able region is $\mathbb{D}_{cache}=3072\cdot2448$ leading to $\mathbb{T}_{gm}(\mathbb{D})=9900.70$ us. The total number of bytes for the halo accesses is $\mathbb{A}(\mathfrak{H}(\mathbb{D}_{cache}))=1000\cdot2\cdot 216\cdot(136\cdot2+256\cdot2)$. Thus 
% $\mathbb{T}^{gm}(\mathfrak{H}(\mathbb{D}_{cache}))=870.35$ us. 
 $\mathbb{T}^{gm}(\mathfrak{H}(\mathbb{D}_{cache}))= 871.22$ us. 
% So $\mathbb{P}_{PERKS}=3072^2\cdot 1000/\mathbb{T}_{PERKS}=876.16$ GCells/s, 
So $\mathbb{P}_{PERKS}=3072^2\cdot 1000/\mathbb{T}_{PERKS}= 876.09$ GCells/s, 
the measured performance is $444.19$ GCells/s ($50.70\%$ of $\mathbb{P}$; in the following sections we elaborate on the analysis of concurrency and its impact on the gap between measured and projected peak).

We use the domain size $\mathbb{D}=3072\cdot2448$ as an example of small domain/ size, i.e.,  when the whole domain can be cached. In our baseline implementation used $\mathbb{A}_{sm}(\mathbb{KERNEL})=\mathbb{D}\cdot 1000 \cdot 4$ bytes of shared memory. The shared memory cached portion is $\mathbb{D}_{cache}=3072\cdot1152$, so $\mathbb{A}^{sm}(\mathbb{D}_{cache})=3072\cdot1152\cdot(999)\cdot2$. We get $\mathbb{T}_{sm}=7.6$ ms and $\mathbb{P}=\mathbb{D}\cdot 1000/\mathbb{T}_{PERKS}=986.38$ GCells/s, the measured performance is $609.30$ GCells/s (61.77\% of $\mathbb{P}$).


%\subsubsection{Large Domain/Input Size}\label{sec:modelLarge}

%{\color{blue}In the majority of situations, 
%% the total memory required for the domain/input $V_{total}$ is far larger than the cacheable portion $V_{cache}$. 
%even after transforming to PERKS, the solver remains bounded by global memory bandwidth ($L_{domain}=L_{global}$). }
%% (assuming perfect overlap of memory with compute, as is the assumption in the roofline model). 
%
%% {\color{blue} In this situation the upper-bound on $P$ we project is directly related to the number of memory transactions after saved and the global memory throughput $Thr_{mem}$. 
%
%
%% }
%
%% {\color{blue} In the situation of conjugate gradient, we directly use memory bandwidth as throughput to represent performance}
%
%% In this situation the upper-bound on speedup we project is directly related to the number of memory transactions saved. 
%Assuming that all memory transactions are coalesced, the amount of memory accesses 
%%(in Bytes)
%is proportional to the number of memory transactions. {\color{blue} Assume that original domain size is $D_{total}$, the saved memory access is $D_{cache}$. Additionally based on Equation~\ref{eqt:latency} and Equation~\ref{eqt:throughput}, the upper-bound on Performance is: }
%
%{\color{blue}
%\begin{equation}\footnotesize
%    \begin{aligned}
%   Thr_{PERKS}=\frac{D_{total}}{D_{total}-D_{cache}+D_{halo}}\times{Thr_{global}}
%    \end{aligned}
%    \label{eqt:perkspeed}
%\end{equation}
%}
%
%{\color{blue}
%To illustrate it, still assume that computing js2d5pt single precision stencil in $3072\times3072$ (36 MB) domain with A100 GPU. The total cache-able region is $3072\times2448$ (28.69 MB). The total halo region is $216\times(136\times2+256\times2)$ (0.65 MB). $Thr_{global}=194.38$. Thus, $Thr_{PERKS}=36/(36-28.69+0.65)*194.38=879.11$, the measured performance is 444.55 GCells/s. 
%
%}

\begin{comment}
It is worth mentioning that $V_{halo}$ is largely negligible in this situation, so for the further analysis, we dismiss this part and get:
\begin{equation}\footnotesize
    \begin{aligned}
   Thr_{PERKS} \approx\frac{D_{total}}{D_{total}-D_{cache}}\times{Thr_{global}}
    \end{aligned}
    \label{eqt:perkslarge}
\end{equation}
Let $Per_{cache}=D_{cache}/D_{total}$, we can further get:
\begin{equation}\footnotesize
    \begin{aligned}
   Thr_{PERKS} \approx\frac{1}{1-Per_{cache}}\times{Thr_{global}}
    \end{aligned}
    \label{eqt:perkslargepercent}
\end{equation}


\subsubsection{Small Domain/Input Size}\label{sec:smdom}
%\lingqi{I think the bottleneck is moved to sm, yet we considered reg in equation~\ref{eqt:perkreg}}
When the domain size is small enough to be mostly or entirely cachable {\color{blue}($L_{domain}=L_{sm}$)}. 
{
\color{blue}
The $Thr_{PERKS}$ in this situation is: 
\begin{equation}\footnotesize
    \begin{aligned}
     Thr_{{PERKS}}=\frac{D_{{total}}}{L_{sm}+L_{halo}}
    \end{aligned}
\end{equation}

To further illustrate it, take computing single precision js2d5pt a domain size of $1024\times7344$ as an example: 

\textbf{Computing $L_{sm}$ based on Equation~\ref{eqt:smlatency}}:$A_{add}$ highly relies on implementation. In our js2d5pt single precision implementation, cached domain per block is $136\times256$. Shared memory access for computation is $136\times256\times4$. Within the domain, $64\times256$ is stored in shared memory. The boundary shared memory access amount is $(256\times2+136\times2)\times2$. This means additional $12.89\%$ of additional shared memory access. There by, total latency for shared memory is $L_{sm}=6.97\times10^{-6}s$

\textbf{Computing $L_{halo}$ based one Equation~\ref{eqt:perkhalo}}: Though halo region might be resided in L2 cache, there is no guarantee. The following discussion only assumes that halo region is in global memory. The tiling per thread block (TB) is $256\times136$, which means halo region per TB is $(256+136)\times 2$. Total thread block amount is $216$. The total halo region amount is $216\times(256+136)\times 2$. With one read one write per iteration. $L_{halo}=8.71\times10^{-7}s$. 

Thus, $L_{sm}+L_{halo}=7.84\times10^{-6}$; $Thr_{PERKS}=959GCells/s$. The measured result is $566GCells/s$ (59\% of theory).


% $B_{sm}=19.49TB/s$.



}
\end{comment}
% For example, assuming only the use of 80\% of the shared memory in V100 to compute a single precision js2d5pt stencil. In this situation, $halo=1$ and the thread block cached range would be $138\times138$ in each thread block. The shared memory access time in a thread block is: $V_{sm}=140\times140\times6$ (5 loads and 1 store). Global memory access time per thread block is: $L_{mem}=138\times138\times2$ (1 load 1 store). According to Jia et. al\cite{jia2018dissecting}, $B_{sm}=13800\ GB/s$ and $B_{mem}=900\ GB/s$, and hence $L_{sm}=8.52\ ns$. In this situation, and since $L_{sm}>L_{halo}>L_{reg}$, the projected upper-bound on speedup is: $Speedup_{small}=\tfrac{(L_{mem})}{L_{sm}}=\tfrac{52.32}{8.52} = 6.14$x. The actual measured speedup for single precision js2d5pt stencil with a small domain implemented as PERKS on V100 is $5.66$x.

% Yet even if most of the data is cached in shared memory or registers, there is still traffic to the global memory to resolve the dependency of threads at the boundary of each thread block. {\color{blue}The latency for accessing the domain portion cached in shared memory $L_{{sm}}$ is determined by total shared memory access volume $V_{{sm}}$ and shared memory throughput $Thr_{{sm}}$: 

% \begin{equation}\footnotesize
%     \begin{aligned}
%      L_{{sm}}=\frac{V_{{sm}}}{Thr_{{sm}}}
%     \end{aligned}
%     \label{eqt:perksm}
% \end{equation}

% The latency for accessing the domain portion cached in registers $L_{{reg}}$ depends on the total registers accesses $V_{{reg}}$ and registers access bandwidth $Thr_{{reg}}$: 

% \begin{equation}\footnotesize
%     \begin{aligned}
%      L_{{reg}}=\frac{V_{{reg}}}{Thr_{{reg}}}
%     \end{aligned}
%     \label{eqt:perkreg}
% \end{equation}

% The time for accessing the halo region in global memory is:
% \begin{equation}\footnotesize
%     \begin{aligned}
%      L_{halo}=\frac{V_{halo}}{Thr_{mem}}
%     \end{aligned}
%     \label{eqt:perkhalo}
% \end{equation}
% Assuming perfect overlapping, the time for accessing the domain in PERKS would be:
% \begin{equation}\footnotesize
%     \begin{aligned}
%      L_{small}=MAX(L_{halo},L_{{sm}},L_{{reg}})
%     \end{aligned}
%     \label{eqt:maxlat}
% \end{equation}
% Based on this, the upper-bound on PERKS performance can then projected to be:
% \begin{equation}\footnotesize
%     \begin{aligned}
%      Thr_{PERKS}=\frac{D_{mem}}{L_{small}}
%     \end{aligned}
%     \label{eqt:maxcomp}
% \end{equation}
% }

\begin{comment}
Assuming the time to access the global memory in a non-PERKS implementation to be $time_{mem}$, the upper-bound on speedup can then projected to be:
\begin{equation}\footnotesize
    \begin{aligned}
     Speedup_{small}=\frac{time_{mem}}{time_{small}}
    \end{aligned}
    \label{eqt:maxcomp2}
\end{equation}
\end{comment}
% \lingqi{note to self, go further details if have time for benchmarking }
%\wahib{Note to self: stopped here}
% \lingqi{@wahib: Some space in shared memory is preserved for computation use, use the remained space for cache, personally prefer "cache" instead of "compute" to represent this situation.}




\begin{comment}
\subsection{Empirical Projection Model}\label{sec:projectionmodel}
% \lingqi{note to self: stop here}
% The goal of this section is to build a simple model to give anticipation for the potential performance achievements when moving an implementation to PERKS. This simple model starts with a simple Premise:

\textbf{Assumption:} PEKRS do not change the efficiency of any baseline implementation. If parallel parameters equals to each other, $Eff_{PERKS}=Eff_{ori}$. With this and according to Equation~\ref{eqt:basic}, we can deduce that:
\begin{equation}\footnotesize
    M_{PERKS}=M_{ori} \times \frac{P_{PERKS}}{P_{ori}}
    \label{eqt:projection}
\end{equation}

Additionally, in large domain/input size, with Equation~\ref{eqt:perkslargepercent}, we can get:

\begin{equation}\footnotesize
\begin{aligned}
    M_{PERKS}&=M_{ori} \times \frac{1}{1-Per_{cache}}
\end{aligned}
\label{eqt:projectionLarge}
\end{equation}

In js2d5pt implementation, we set thread block=256. In baseline, the default thread block per stream multiprocessor ($TB/SM$) is 8. Yet, PERKS put much pressure in register and the max $TB/SM$ is 2. We measured different $TB/SM$ settings for baseline and PERKS and put them in Table~\ref{tab:projection}. We also use Equation~\ref{eqt:projectionLarge} to project the performance based on the percentage of region cached and put the result in the same Table. 

\begin{table}[t]
    \centering\small
    \caption{Single precision $3702\times3702$ js2d5pt stencil in A100, performance of baseline, PERKS and the performance projection}
    \begin{tabular}{|c|c|c|c|c|c|}
    \hline
        \multirow{2}{*}{$\tfrac{TB}{SM}$}  & Baseline & $Per_{cache}$ & Projection & PERKS&Accuracy\\
          & GCells/s && GCells/s & GCells/s&\\\hline
        1 & 94.87   & 77.34\%\tablefootnote{Slightly smaller than tb/sm=2 due to compiler under-optimization} & 418.73& 357.79& 85.44\%\\
        2 & 133.41  & 79.69\% & 656.78& 444.55& 67.69\%\\ 
        8 & 137.65  & -       & - & -&-\\\hline
    \end{tabular}
    \label{tab:projection}
\end{table}


% Admittedly, while implementing PERKS, loops and data structures that maintain register and shared array would put pressure on register usage and thus decrease the concurrent max thread amount per stream multiprocessor (SM). It is practical to project performance base on: 1) fewer threads per SM and 2) PERKS not able to use all register resources for cache. 

% Another drawback of this model is that in the situation when using PERKS in small domain, bottleneck might move from global memory to on-chip resources, the premise might be break. Yet, because the most of the code and implementation stays unmodified, this empirical projection model would still give prediction with acceptable errors. 

% \lingqi{Need to additionally have an evaluation to show the register usage situation. How many registers really be available.}
According to Table~\ref{tab:projection}, the Projection Model's accuracy is generally more than 50\%, which is enough to satisfy the model's goal to anticipate the potential performance benefit of applying PERKS without the knowledge of achieving high performance with low occupancy~\cite{volkov2010better}. Additional efforts to tune code with concurrency analysis could gain further performance. 
\end{comment}
%\color{blue}
%\lingqi{note to self: stop here}
\subsection{Concurrency and Micro-benchmarks}\label{sec:perconcurrency}
% \lingqi{note to self: stop here}
%\lingqi{note to self: rethink how to describe concurrency per thread}
%\lingqi{note to self: What is the concurrency used in this paper}
Reducing device occupancy increases the availability of resources to be used for caching in PERKS (as illustrated earlier in Figure~\ref{Fig:showcase}). On the contrary, reducing occupancy can lead to lower device utilization. To effectively implement PERKS, one has to reduce the occupancy as much as possible without scarifying performance. Inspired by the findings of Volkov~\cite{volkov2010better}, we assume that the efficiency function $\mathfrak{E}$ reaches its peak point when the code provides enough concurrency to saturate the device (irrespective of the occupancy):
\begin{equation}\footnotesize
    \mathfrak{E}(\mathbb{C}_{sw},\mathbb{C}_{hw})=100\%, \text{if } \forall \mathbb{C}_{sw}\geq \mathbb{C}_{hw}
\end{equation}

%The efficiency function $\mathfrak{E}()$ in this paper is used heuristically to ensure that PERKS won't harm performance. General cases when $\exists \mathbb{C}_{sw} < \mathbb{C}_{hw}$ is beyond the topic of this paper. 

Where $\mathbb{C}_{sw}(\mathbb{OP})$ is the minimum number of concurrently executable instructions of the operation $\mathbb{OP}$ exposed by the launched kernel, and $\mathbb{C}_{hw}(\mathbb{OP})$ is the maximum numbers of instructions of the operation $\mathbb{OP}$ that the device is capable of handling concurrently. Because this paper mainly focuses on memory bound applications, the $\mathbb{OP}$ referred to in this paper are limited to data access operations, i.e. global memory load/store $\mathbb{C}(\mathbb{GM})$, shared memory load/store $\mathbb{C}(\mathbb{SM})$, and L2 cache load/store $\mathbb{C}(\mathbb{L}2)$. 

%Specifically, $\mathbb{C}_{sw}(\mathbb{OP})$ denotes the max unblocking operations $\mathbb{OP}$ in software $sw$; $\mathbb{C}_{hw}(\mathbb{OP})$ denotes the minimal the operations $\mathbb{OP}$ that necessary to saturate a given device $hw$. Device level concurrency usually really large, we use stream multiprocessor level concurrency $\mathbb{C}_{sw}^{SMX}$ and $\mathbb{C}_{hw}^{SMX}$ for most of followning discussion. Because this paper mainly focus on memory bound applications, the $\mathbb{OP}$ referred in this paper is limited to memory access related, i.e. global memory access $\mathbb{C}(\mathbb{GM})$, shared memory access $\mathbb{C}(\mathbb{SM})$, and L2 cache access $\mathbb{C}(\mathbb{L}2)$. 



%When $\exists\mathbb{C}_{code}(\mathbb{OPT})<\mathbb{C}_{code}(\mathbb{OPT})$, the $\mathbb{OPT}$ could not saturate the device, the $\mathbb{M}$ would be far away from $\mathbb{P}$
\subsubsection{Measuring $\mathbb{C}_{sw}^{SMX}$} $\mathbb{C}_{sw}^{SMX}(\mathbb{OP})$, the kernel concurrency at the streaming multi-processor (SMX) level, can be computed based on the concurrency exposed by the threads of a thread block $\mathbb{C}_{sw}^{TB}(\mathbb{OP})$ and number of concurrently running thread blocks per stream multiprocessor {\footnotesize$TB/SMX$}:  {\footnotesize$\mathbb{C}_{sw}^{SMX}(\mathbb{OP})=\mathbb{C}_{sw}^{TB}(\mathbb{OP})\cdot TB/SMX$}.

%As an example, we use the code example in Fig~\ref{fig:ccrcyexmaple} to deduce the code concurrency of global memory load and stores $\mathbb{C}^{SMX}_{sw}(\mathbb{GM})$ in a single Stream Multiprocessor to be: $\mathbb{C}^{SMX}_{sw}(\mathbb{GM})=\mathbb{C}^{TB}_{sw}(\mathbb{GM})=256\cdot 2 = 2048$ load and store operations for type float. Note that the number of operations in this example is then adjusted to accounts for the effect of coalesced access on the actual number of operations (or transactions).

%  \begin{comment}
%  \begin{figure}
% \centering
% \begin{lstlisting}[language=C,gobble=2]
%  blocks = 80; thread/block = 256; block/SMX = 1;
%  __global__ void Kernel(float*A,float*B,...)
%  {...
%    A[(256*bid)+tid] = B[(256*bid)+tid] * tid;
%  }
% \end{lstlisting}
% \caption{\label{fig:ccrcyexmaple} Example for concurrency counting in a CUDA kernel.}
% \end{figure}
% \end{comment}
 
\subsubsection{Measuring $\mathbb{C}_{hw}$} According to Little's Law~\cite{Little1961APF}, the hardware concurrency $\mathbb{C}_{hw}$ can be determined by the throughput $\mathbb{THR}$ and latency $\mathbb{L}$\cite{volkov2010better}: 
\begin{equation}\footnotesize
    \mathbb{C}_{hw}(\mathbb{OP})=\mathbb{THR(OP)} \cdot \mathbb{L(OP)}
\end{equation}

The throughput $\mathbb{THR}$ for different data access operations are available in Nvidia online documents~\cite{nvidia2019programming,amperewhite}. We measure the latency $\mathbb{L}$ with commonly used microbenchmarks~\cite{wong2010demystifying,mei2014benchmarking,zhang2017understanding} (The latency measurements are collected in the AD/AE appendix). %Throughput and latency of relevant operations on A100 and V100 are summarized in Table~\ref{tab:concurrency}. 

\begin{comment}
	Latency of shared memory and L2 Cache can be tested with microbenchmark provided by previous research~\cite{wong2010demystifying,mei2014benchmarking}. But these works\cite{wong2010demystifying,mei2014benchmarking} test global memory latency with a metrics of cycle, which do not reflect its latency in second due to dynamic frequency. We thereby combine Mei etc.'s~\cite{mei2014benchmarking} microbenchmark Zhang etc's research~\cite{zhang2017understanding} to test $L_{global}$ with CPU clock. The alternative measurement is to manually set frequency to be static and use the existing microbenchmark and latency in cycle and deduce its latency in second from the frequency. However, we found that the deduced latency various as the frequency various, which might due to that latency of some operation, that involved in global memory access, might various as the GPU frequency various. So the CPU measured global memory latency with default dynamic frequency setting is reported in this paper. $Thr$, $L$ and $C$ of memory in A100 and V100 is gathered in Table~\ref{tab:concurrencysm}, Table~\ref{tab:concurrencyl2} and Table ~\ref{tab:concurrencygm}. 
\end{comment}

\begin{comment}
\begin{table}[t]
	\caption{Throughput and latency of relevant operations on A100 and V100 GPUs}
    \centering
	\begin{tabular}{|c|c|c|}
	\hline
	 & A100&V100\\\hline
	\multicolumn{3}{|c|}{ Shared memory}\\\hline
	$\mathbb{THR}(\mathbb{SM})(B/cycle) $&128&128\\
	$\mathbb{L}(\mathbb{SM})(cycle)$ &28&26\\
	$\mathbb{C}^{SMX}_{hw}(\mathbb{SM}) (B)$ &3584&3328\\\hline
	\multicolumn{3}{|c|}{Global memory}\\\hline
	$\mathbb{THR}(\mathbb{GM})(GB/s) $ & 1555   & 900\\
	$\mathbb{L}(\mathbb{GM})(ns)$      & 403.28 & 286.17\\
	 $\mathbb{C}_{hw}(\mathbb{GM})(B)$& 627101 & 257553\\
	$\mathbb{C}^{SMX}_{hw}(\mathbb{GM})(B)$  & 5807   & 3220\\\hline	
	
	\multicolumn{3}{|c|}{L2 Cache}\\\hline
	$\mathbb{THR}(\mathbb{L}2)(B/cycle) $ & 5120   & 2048\\
	$\mathbb{L}(\mathbb{L}2)(cycle)$      & 218/384 & 200\\
	$\mathbb{C}_{hw}(\mathbb{L}2)(B)$& 1541120 & 409600\\
	$\mathbb{C}^{SMX}_{hw}(\mathbb{L}2)(B)$ & 14270   & 5120\\\hline	
	\end{tabular}
	\label{tab:concurrency}
\end{table} 
\end{comment}

\begin{comment}
\todo{use a single table, it can be two rows, e.g. V100, A100}
\begin{table}[t]
	\caption{Throughput and latency of relevant operations on A100 and V100 GPUs}
    \centering
     
    \begin{subtable} [h]{0.47\textwidth}
    \centering
    \caption{Shared memory}
    \begin{tabular}{|c|c|c|c|}
    \hline
          & $\mathbb{THR}$  & $\mathbb{L}$  & $\mathbb{C}^{SMX}_{hw}(\mathbb{SM})$ \\
          &  (B/cycle) & (cycle) & (B)\\\hline
        {A100} & 128 & 28 & 3584 \\\hline
        {V100} & 128 & 26 & 3328 \\\hline
    \end{tabular}
    \label{tab:concurrencysm}
    \end{subtable}

	\begin{subtable}[h]{0.47\textwidth}
	\centering
    \caption{Global memory}
    \begin{tabular}{|c|c|c|c|c|}
    \hline
         & $\mathbb{THR}$ & $\mathbb{L}$  & $\mathbb{C}_{hw}(\mathbb{GM})$ & $\mathbb{C}^{SMX}_{hw}(\mathbb{GM})$ \\
         & (GB/s) & (ns) &(B) & (B) \\\hline
        {A100}  & 1555 & 403.28 & 627101& 5807 \\\hline
        {V100}  & 900  & 286.17 & 257553 & 3220 \\\hline
    \end{tabular}
    \label{tab:concurrencygm}
    \end{subtable}
    
    \begin{subtable} [h]{0.47\textwidth}
    \centering
    \caption{L2 Cache}
    \begin{tabular}{|c|c|c|c|c|}
    \hline
         & $\mathbb{THR}$  & $\mathbb{L}$ & $\mathbb{C}_{hw}(\mathbb{L}2)$ & $\mathbb{C}^{SMX}_{hw}(\mathbb{L}2)$ \\
         & (B/cycle) & (cycle) & (B) & (B)\\\hline
        {A100\tablefootnote{A100 has two segments of L2 cache. While the average latency of each segment may vary, we treat them as a homogeneous L2 for simplicity} } 
            & 5120 & 218/384 & 1541120 & 14270 \\\hline
        {V100} & 2048 & 200 & 409600  & 5120 \\\hline
    \end{tabular}
    \label{tab:concurrencyl2}
    \end{subtable}
    \label{tab:concurrencysummary}
\end{table}
\end{comment}

%Easy to notice that if Fig~\ref{fig:ccrcyexmaple} runs in A100, we have $\mathbb{C}_{code}(gm)>\mathbb{C}_{hw}(gm)$. The measured bandwidth of this code is $1015.98$ GB/s ($65.33\%$ of global memory bandwidth). Experiments also shows that in this situation increasing thread block numbers won't further influence performance. 


\subsection{Concurrency Analysis}
\label{sec:conan}

%%The main benefit of performance model is that it could guide optimizations when un-reasonable slowdown is observed. In PERKS performance model is also necessary to ensure that applying PERKS don't harm performance. 

%Even though in this research we haven't encountered, we anticipate 2 scenarios that PERKS might harm performance: 1). The original kernel $\mathbb{KERNEL}$ has high register pressure that any modification might introduce register spill or already suffer from register spill issue, or 2). The $\mathbb{KERNEL}$ is under-optimized that need to rely on large amount of concurrently running threads to ensure performance. 

%Solving first issue is not the purpose of this research, readers can refer to existing register optimizations~\cite{Rawat:2018:AIR:3291656.3291718,Rawat:2018:ROS:3200691.3178500}; yet the second issue can be resolve by using concurrency analysis to guide code optimization. 

% \subsubsection{Use concurrency analysis to reduce thread blocks per stream multiprocessor $TB/SMX$ to its minimum}
In this section, we briefly describe how we analyze the concurrency to reduce the occupancy of the original kernel in order to release resources for caching while sustaining performance. We conduct a static analysis to extract the data movement operations in the kernel. Note that we account for any barriers in the original kernels that could impact the concurrency of operations, i.e., we do not combine operators/instructions from before and after the barrier when we count the operators. Finally, we apply a simple model to identify the least occupancy we could drop to before the concurrency starts to drop. For example, we did a static analysis of a single precision 2D 5-point Jacobi stencil kernel to conduct a concurrency analysis. It is worth mentioning that the baseline kernel we use is fairly complex since it is highly optimized by using shared memory to reduce traffic to global memory to its minimum~\cite{maruyama2014optimizing}. The results summarized in Table~\ref{tab:concurrencyanalysis} show that for this kernel, we could reduce the original occupancy to ${1/4}^{th}$ while maintaining performance.

% $\mathbb{C}_{sw=2d5pt,TB/SM=1}^{SMX}(\mathbb{GM})=18512$B$>\mathbb{C}_{hw=A100}^{SMX}(\mathbb{GM})$. Also $\mathbb{C}_{sw=2d5pt,TB/SM=1}^{SMX}(\mathbb{SM})>10320$B$>\mathbb{C}_{hw=A100}^{SMX}(\mathbb{SM})$

% \footnote{In this implementation, loading from global memory to shared memory happens before the computation starts.}
To understand the gap between the projected upper-bound on achievable performance and the measured performance ($94.75/138.29=68.52\%$), we inspect the efficiency function $\mathfrak{E()}$. The number of concurrent global memory accesses and shared memory accesses in the 2D 5-point Jacobi stencil kernel are enough to saturate A100 when TB/SMX=1. Accordingly, we get $\mathfrak{E}_(\mathbb{C}_{sw=j2d5pt,TB/SM\geq1},\mathbb{C}_{hw=A100})=1$,which would indicate that the observed gap in performance is not due to a drop in concurrency we did not model. While this confirms the effectiveness of the concurrency analysis (i.e., since the concurrency analysis resonates with the empirical measurements in Table~\ref{tab:concurrencyanalysis}), it does not uncover the gap between measured and projected peak achievable. Further investigative profiling revealed that the concurrency for accesses in L2 cache, not global memory, is impacted by reducing occupancy on A100 in specific to the level that affects performance notably. More particularly, access to global memory for the halo region garners a high L2 cache hit rate. This effectively means that higher concurrency is necessary to saturate the L2 cache when hit rates are high. To confirm, we manually doubled the concurrency $\mathbb{C}^{TB}_{sw}$: the performance increased to 123.94 GCells/s with TB/SMX=1 (from $68.52\%$ up to $89.6\%$). 
% (as empirical benchmarking in Table~\ref{tab:concurrency} confirms)




%So, \textbf{no necessary to launch thousands of threads to saturate device. An alternative solution is to launch fewer threads with more unblocked operations.}

%The guess is that this larger desire for L2 cache concurrency might due to the 2 slice design of A100 chip. 
%We also put the experiment of running with $\mathbb{D}=3072^2$ in the same table. 


\begin{table}[t]
    \centering
    \caption{Concurrency analysis of global memory accesses of a single precision 2D-5point Jacobi stencil kernel running on A100 (1000 time-steps on $3072^2$ domain)}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{?c?c|c|c|c|c?}
        \tbhline
            \multirow{2}{*}{$\tfrac{TB}{SMX}$}  & Used Reg. & Unused Reg. & GM Load & GM Store & Measured\\
              & /SMX  &/SMX    & op/SMX & op/SMX  & GCells/s\\\tbhline
            \textit{1} & 32KB  & 224KB  & 2580 & 2048 & 94.75\\
            \textit{2} & 64KB   & 192KB & 5160 & 4096 & 133.24\\
            \textit{8} & 256KB  & 0KB   & 20640 & 16384 & 138.29\\\tbhline
        \end{tabular}
    }
    \label{tab:concurrencyanalysis}
\end{table}





%This issue could be alleviated with concurrency analysis. 

%In situations that amount of registers used $\mathbb{ALG}$ is small, like low order stencil, 

%\lingqi{note to self: summarize the register added from baseline to perks} 
%When applying PERKS more registers would be consumed. 

%Low order stencil, not a issue.

%How about higher order stencil?

%\subsubsection{Concurrency to guide optimization}
%2 blk/sm or more ILP
%\subsection{Lessons}

%\subsection{STOP HERE}
\begin{comment}
Specifically, if dealing with single precision data in A100, with $size(float)=4B$. In order to saturate global memory bandwidth, one can either launch 1024 threads with each thread accesses global memory 2 times (or 1.42 times) unblockedly; or launch 256 threads with each thread accesses global memory 6 times (or 5.67 times). In other words,\textbf{ no necessary to launch thousands of threads to saturate device. An alternative solution is to launch fewer threads with more unblocked operations. }





\subsection{Trade off between registers for performance and registers for cache}\label{sec:regtradeoff}
Increasing concurrency inside code ($C_{code}$) is either done by using more threads, or provide more unblocked operations inside code. Both method consumes registers for performance. More registers used for performance means fewer registers remained for cache, which decrease the potencial performance of PERKS as can be implied by Equation~\ref{eqt:projectionLarge}. This paradox can by solved by Equation~\ref{eqt:concurrencyrequirement}, which implies that after $C_{code}>C_{hw}$ additional $C_{code}$ do not influence performance. So a heuristic approach is to find a point where $C_{code} \gtrapprox C_{hw}$ and use all the remained resources to cache data. 


The baseline js2d5pt code used in this section is global memory bandwidth bottleneck, we mark its global memory access operation count per SMX in Table~\ref{tab:concurrencyanalysis}. In stencil computation, read data from global memory includes halo regions that possibly comes from L2 cache. So $C_{read}\gtrapprox C_{L2 Cache}$ need to be saturated. While storing data only involve global memory. So $C_{write}\gtrapprox C_{global}$ need to be guaranteed. $C_{global}=1452 float$; ${C_{L2 Cache}=3567 float}$. According to Table~\ref{tab:concurrencyanalysis}, All $C_{write}>C_{global}$; Most $C_{read}>C_{L2 Cache}$ except $C_{read}|TB/SM=1$. This explains that 1) nearly no performance different for $TB/SMX>=2$, because the device is saturated; and 2) performance drop significantly when $TB/SMX=1$ because the L2 cache is under utilized. 



Though further sacrificing device saturation ($C_{code}<C_{hw}$) to spare more registers for cache might also increase performance, this performance feature is hard to model. The simplest advice for this situation is to refer to the Projection Model in Section~\ref{sec:projectionmodel}. 

% Also, under the assumption that compiler is optimized enough to separate remained registers, within certain small domain size, more registers for cache that 

% \footnote{ }


% In situation that after transfer from baseline to PERKS, code concurrency might decrease due to register pressure, which lead to fewer concurrently running threads, additional optimization would be perform to increase concurrency from implementation level. 

% \lingqi{When add additionally tune process, might be even closer to the peak performance.}



% On the other hand, for 3d13pt. the thread block cached range would be: $22\times22\times{22}$. In this situation:

% $region_{total_{sm}}=26^3\times14\times80$(13 load 1 store, in 80 stream multiprocessors)

% $time_{sm}=815ns<time_{mem_{halo}}=1442ns$

% we can expect a performance of: 

% $Speed=\tfrac{(region_{total})}{time}=\tfrac{22^3\times 80}{time_{total}}=931 GCells/s$. 

% Yet these anticipated peak performances are difficult to achieve in real code. 
% \end{comment}
% \begin{comment}
\end{comment}
\begin{comment}
\subsubsection{Tiled PERKS}\label{sec:perktilemodel}
%\lingqi{@Wahib: I think it is better to consist with PERKS, or are there any reason for use PERK? not sure if is mistake, would mark}
%Tiled PERK only valid when $time_{{sm}}=time_{total}$, or, the bottleneck not global memory bandwidth. This situation is true in most of 2d stencil solvers.


%consequences of time step $i_t$ mainly influence performance. On one hand, $i_t$ should be large enough to saturate the stream multiprocessor. In this situation $speed_{tiled}$ is proportion to $i_t$.
% \begin{comment}
\begin{equation}\footnotesize
    \begin{aligned}
     time_{tiled}(i_t)=time_{small}\times i_t+time_{mem}
    \end{aligned}
    \label{eqt:haloconsider}
\end{equation}
\begin{equation}\footnotesize
    \begin{aligned}
     speed_{tiled}(i_t)=\tfrac{region_{total}\times i_t}{ time_{small}\times i_t+time_{mem}}
    \end{aligned}
    \label{eqt:haloconsider2}
\end{equation}

%Additionally, we can get:

\begin{equation}\footnotesize
    \begin{aligned}
        speed_{tiled}(i_t)=\lim_{i_t \to \infty}speed_{small}
    \end{aligned}
    \label{eqt:tilesmall}
\end{equation}

% speed=\tfrac{region_{total}\times i_t}{ time_{small}\times i_t+time_{mem}}=\lim_{i_t \to  \infty}\frac{region_{total}}{time_{small}}=speed_{small}
%But, on the other hand $i_t$ is proportion to the HALO size, increasing the HALO region and decreasing the VALID region ($region_{VALID}$), thus increase the valid computation time. Let $p_{VALID}=\tfrac{region_{VALID}}{region_{total}}=\tfrac{region_{total}-region_{HALO}}{region_{total}}$

\begin{equation}\footnotesize
    \begin{aligned}
     time_{valid}=\tfrac{time}{p_{VALID}} 
    \end{aligned}
    \label{eqt:haloconsider}
\end{equation}
Because $speed=\frac{region_{total}}{time}$. It is possible to further get:
\begin{equation}\footnotesize
    \begin{aligned}
     speed_{valid}= speed_{tiled}(i_t)\times p_{VALID}
    %  speed_{small}\times{region_{VALID}} 
    \end{aligned}
    \label{eqt:haloconsider2}
\end{equation}
% \end{comment}

As Figure~\ref{fig:perttile} shows, there are $T$ temporal blocking time steps for each tile. For $time_{global}$ being the time for loading/storing from/to global memory every $T$ steps, $time_{load}$ being the time for accessing the tile (including halo) in shared memory in one time step, and $N$ being the total number of time steps in the simulation, the time per tile based on data accesses can be written as:
\begin{equation}\footnotesize
    \begin{aligned}
%     time_{tiled}=time_{load}\times T + time_{global}\times\tfrac{N}{T}
time_{tiled}=time_{load}\times N + time_{global}\times\tfrac{N}{T}
    \end{aligned}
    \label{eqt:haloconsider}
\end{equation}

% \end{comment}

% \begin{comment}
The ratio of the valid region to the total region $\tfrac{region_{valid}}{region_{total}}$ reduces the speedup, since the redundant computation of the halo region means additional redundant work inflates the amount of work. Assuming the time to access the global memory in a non-PERK implementation to be $time_{mem}$, the projected upper-bound on speedup (for $T$ time steps) then becomes:
\begin{equation}\footnotesize
    \begin{aligned}
     Speedup_{tiled}=\tfrac{time_{mem}}{time_{tiled}}\times\tfrac{region_{valid}}{region_{total}}
    %  speed_{small}\times{region_{valid}} 
    \end{aligned}
    \label{eqt:haloconsider2}
\end{equation}

%For simplicity, we assume that: $ speed_{tiled}(i_t) \approx speed(small)$. We can get $speed_{valid}=speed(small)\times p_{VALID}$

For example, we compute a single precision js2d5pt stencil with temporal blocking of $100$ steps $T=100$ on V100. The total cacheable domain is $1224\times1224$ with $halo=1$, and the total halo region $T*2*halo=200$. The valid region would be:  $region_{valid}=(1224-200)^2$ and the ratio of the valid region to the total region would be $((1224-200)/1224)^2=0.7$. The projected upper-bound on speedup is: $Speedup_{tiled}=\tfrac{time_{mem}}{time_{tiled}}\times0.7 = \tfrac{122.17}{14.93}\times0.7 = 5.72$x. The actual measured speedup for single precision js2d5pt stencil with tiled PERKS implementation on V100 is $4.91$x.
% \end{comment}
	

The upper limit of Tiled PERKS is bounded by speedup of smaller domains from the previous subsection: $Speedup_{small}$. Yet the ratio of the valid region to the total region $\tfrac{region_{valid}}{region_{total}}$ reduces the speedup, since the redundant computation of the halo region means additional redundant work inflates the total amount of work. Assuming the time to access the global memory in a non-PERK implementation to be $time_{mem}$, the projected upper-bound on speedup (for $T$ time steps) then becomes:
\begin{equation}\footnotesize
    \begin{aligned}
     Speedup_{tiled}=\tfrac{time_{mem}}{time_{tiled}}\times\tfrac{region_{valid}}{region_{total}}
    %  speed_{small}\times{region_{valid}} 
    \end{aligned}
    \label{eqt:haloconsider3}
\end{equation}

For example, we compute a single precision js2d5pt stencil with temporal blocking of $100$ steps $T=100$. The total cacheable domain is $2048\times2560$ with $halo=1$; and the total halo region $T*2*halo=200$. The valid region would be:  $region_{valid}=(2048-200)\times(2560-200)$ and the ratio of the valid region to the total region would be $((2048-200)\times(2560-200)/2048/2560)^2=0.83$. 
The projected upper-bound on speedup is: $speedup_{tiled}=Speedup_{small}\times0.83 = 5.66(measured)\times0.83 = 4.70$x 
The actual measured value for single precision js2d5pt stencil with tiled PERKS implementation on V100 is $3.68$x.

\end{comment}

%Assuming that the tested speed in small domain is $speed_{small}=300GCells/s$. We can get a theoretical speed of $speed=speed_{small}\times p_{VALID}=210GCells

%To further explain it, take 2d5pt in V100 as an example. Assume that $i_t=100$. The total cacheable domain is: $1224\times1224$. The $HALO=i_t*2*halo=200$. The valid region would be:  $region_{VALID}=(1224-200)^2$ and $p_{VALID}=((1224-200)/1224)^2=70.00\%$. Assuming that the tested speed in small domain is $speed_{small}=300GCells/s$. We can get a theoretical speed of $speed=speed_{small}\times p_{VALID}=210GCells$. 

% \lingqi{note to self: add reference after analysis section is done}

% In this situation, $i_t$ should be large enough to saturate device, 

% \begin{equation}\footnotesize
%     \begin{aligned}
%      max(time_{{comp}},time_{mem_{halo}},time_{{sm}})
%     \end{aligned}
%     \label{eqt:maxcomp}
% \end{equation}


% \wahib{@Lingqi: one more thing about the performance model, I think it should include a small part about the tiled PERKs and halo region.}

%\lingqi{@Wahib: I found that I did not subtract the boundary halo of whole domain while processing the result of Tiled PERKS. This produce a slightly higher than normal speedup and make it hard to do analysis in this section. I corrected the result and recompile part of this section}



%for solvers that are very optimized to use all registers, 
%\textbf{PERKS on GPUs from other vendors:} PERKS are not necessarily limited to CUDA; AMD GPUs can also benefit from PERKS given that AMD has a device-wide barrier primitive similar to the one in CUDA (ROCm documentation says they do not support any Cooperative Groups Functions)


%: a) can be used in cases where a kernel is standalone (CITE) or a smaller time steps exit (CITE), b) fuse before using a PERK, c) argue that a similar limitation on temporal blocking exists, yet temporal blocking is widely used



%While this focus in this paper is on GPUs, there is an opportunity to expand the PERKS method to other architectures. For instance, one could implement a PERKS-like kernel on a CPU by manually, or automatically, altering the register reuse decided by the compiler to cache portions of the output of each time step to be used in as input in the following time step.



%\wahib{Note to self: if we don't broaden the assumption that PERKS can work on CPU, remove the following paragraph since it is not relevant for GPUs.}
%\textbf{Symmetry of Loads and Stores:} In this analysis we assume symmetry between the load and store operations. In processor where the load and store operations are asymmetric w.r.t. latency and throughput (ex: Fujitsu A64FX~\cite{yoshida2018fujitsu}), one would need to first determine the effect of asymmetry on performance. For iterative stencils, if the load operation is the bottleneck, then caching any data in region of interest is preferable. For conjugate gradient solver, because matrix $A$ is usually relatively large and involves only one load operation per element, the bottleneck would be the load operation. In this situation, the priority for caching vector $x$ would be drop, and the priority would likely become: $r>Ap|p>others$ $r>others$ and $r>Ap=p>others$ respectively for dense matrix, general sparse matrix, and diagonal sparse matrix.


%\wahib{Note to self: Generality w.r.t. operation in the kernel}
%\wahib{Note to self: Usability w.r.t. distributed computing: comm/comp overlap and use PERK for the interior, or with communication-avoiding Kylov methods~\cite{DBLP:conf/sc/IdomuraIAI20}}


%\wahib{note to self: there are no guarantees that the compiler releases all the registers after the compute portion is finished. For solvers that are very optimized to use all registers, imperfect register reuse by the compiler could result in fewer registers being available for caching and leaves only shared memory can be used in caching.}
%\wahib{Note to self: emphasize that the PERKS is not necessarily limited to CUDA; AMD GPUs can also benefit from PERKS given that AMD has a device-wide barrier primitive that is similar to CUDa (name that feature and cite it in ROCm)}

% PERKS mainly deal with situations that global memory bandwidth is the bottleneck. And PERKS can benefit performance if the program has the schema that load data from global memory compute and store to global memory 





% \wahib{This subsubsection should move to the implementation section, since it is specific to CUDA.}
% \lingqi{note to self: move this subsubsection}

% Other Limitations that might want to mention
% \begin{itemize}
%     \item global memory bandwidth problem
%     \item code have already express enough concurrency. 
%     \item If the bottleneck is shared memory bandwidth, performance might be bad
%     \item PERKS tent to use more registers as 
% \end{itemize}
% Another issue is that
%\lingqi{note to self: make sure that the performance mark be consistent }
%\lingqi{note to self: find a name for shared memory implementation}


% \end{comment}
\color{black}

% \revision
% {
% % We want to emphasize that Section~\ref{sec:peakperform} 
% \subsection{Summarize}
% In this Section, we present the Peak Achievable Performance we used to ensure the quality of our implementation (Section~\ref{sec:peakperform}). We prove that over-subscription and greedily consuming all resources are unnecessary by using Concurrency Analysis (Section~\ref{sec:conan}). Yet both are only necessary for squeezing performance. 

% Practically, a programmer can simply rely on auto tuning tools (ex: Kernel Tuner~\cite{kerneltuner}) to identify the minimal occupancy of an iterative memory-bound kernel and use the remaining on-chip resources to cache data.
% % As 

% % Given an iterative application that reaches memory bottleneck, programmers can simply rely on auto tuning tools (ex: Kernel Tuner~\cite{kerneltuner}) to identify the minimal occupancy

% % The purpose of Section~\ref{sec:perconcurrency} and Section~\ref{sec:conan} is mainly to prove the unnecessity of over-subscription and greedily consuming all resources. Practically, programmers can either follow the track we proposed, or simply rely on auto tuning tools (ex: Kernel Tuner~\cite{kerneltuner}) to identify the minimal occupancy. Ideally, optimizing solvers for higher performance in lower occupancy could gain further performance by applying PERKS. 

% % In this section, we propose a performance model that serves the following purposes. First, we propose a projection of achievable performance that we compare with measured results to detect abnormal behavior or implementation shortcomings. We relied on this projection in the analysis of our PERKS implementation quality (Section~\ref{sec:peakperform}).
% %{\item\lingqi{Provide simple model to project performance of PERKS (Section~\ref{sec:projectionmodel} or Equation~\ref{eqt:projectionLarge})} \wahib{@Lingqi@:this point is similar to the previous point, so please merge.}}
% %\item Identifying limitations of caching schemes and shortcomings of caching policies (Section~QQ).\lingqi{I don't know what to do with it}
% % Second, we identify the bounds on reducing concurrency before dropping performance and use concurrency to explain potential optimizations for further performance improvement (Section~\ref{sec:conan}). 


% }



==> 04_05whyperksworks.tex <==

\section{How and Why PERKS is Effective}\label{sec:simplepermodel}

This section includes an analysis of the effectiveness of PERKS in a practical setting. The analysis in this section is based on the latest Nvidia GPUs. Nonetheless, the analysis can be expanded to other architectures with relative ease. 
\revisiona{We begin with a practical bound analysis (Section~\ref{sec:practicalbound}). Next, we explain why PERKS is effective by analyzing the influence of domain size that is cached (Section~\ref{sec:howworks}). Finally, we discuss how PERKS is effective in identifying the potential efficiency loss (Section~\ref{sec:whyworks}).}
% We first explain how to effectively reduce concurrency in a regression-free manner to improve the performance of PERKS (Sections~\ref{sec:perconcurrency}). 
%We then discuss how the transformation to PERKS becomes effective by analyzing the practical bound on performance gain when PERKS is applied (Section~\ref{sec:howperksreduces}). 
% \revisiona{We then discuss how the transformation to PERKS is effective by analyzing the practical bound on performance before and after PERKS is applied (Section~\ref{sec:howperksreduces}).}
%Finally, we further explain why PERKS are feasible in the latest generations of GPUs (Section~\ref{sec:whyperks}). 
\begin{comment}
{
\subsection{Concurrency}\label{sec:apdperconcurrency}

{To effectively improve performance with PERKS, it is desirable to reduce the occupancy as much as possible \revisionb{\textbf{without scarifying performance}}.} Inspired by the findings of Volkov~\cite{volkov2010better}, we assume that the efficiency function $\mathfrak{E}$ reaches its peak point when the code provides enough concurrency to saturate the device (irrespective of the occupancy):
\begin{equation}\footnotesize
    \mathfrak{E}(\mathbb{C}_{sw},\mathbb{C}_{hw})=100\%, \text{if } \forall \mathbb{C}_{sw}\geq \mathbb{C}_{hw}
\end{equation}

Where $\mathbb{C}_{sw}(\mathbb{OP})$ is the minimum number of concurrently executable instructions of the operation $\mathbb{OP}$ exposed by the launched kernel, and $\mathbb{C}_{hw}(\mathbb{OP})$ is the maximum numbers of instructions of the operation $\mathbb{OP}$ that the device is capable of handling concurrently. Because this paper mainly focuses on memory bound applications, the $\mathbb{OP}$ referred to in this paper are limited to data access operations, i.e. global memory load/store $\mathbb{C}(\mathbb{GM})$, shared memory load/store $\mathbb{C}(\mathbb{SM})$, and L2 cache load/store $\mathbb{C}(\mathbb{L}2)$. 


\subsubsection{Measuring $\mathbb{C}_{sw}^{SM}$} $\mathbb{C}_{sw}^{SM}(\mathbb{OP})$, the kernel concurrency at the streaming multi-processor (SM) level, can be computed based on the concurrency exposed by the threads of a thread block $\mathbb{C}_{sw}^{TB}(\mathbb{OP})$ and number of concurrently running thread blocks per stream multiprocessor {\footnotesize$TB/SM$}:  {\footnotesize$\mathbb{C}_{sw}^{SM}(\mathbb{OP})=\mathbb{C}_{sw}^{TB}(\mathbb{OP})\cdot TB/SM$}.

\subsubsection{Measuring $\mathbb{C}_{hw}$} According to Little's Law~\cite{Little1961APF}, the hardware concurrency $\mathbb{C}_{hw}$ can be determined by the throughput $\mathbb{THR}$ and latency $\mathbb{L}$\cite{volkov2010better}: 
\begin{equation}\footnotesize
    \mathbb{C}_{hw}(\mathbb{OP})=\mathbb{THR(OP)} \cdot \mathbb{L(OP)}
\end{equation}

The throughput $\mathbb{THR}$ for different data access operations are available in the official documentation of Nvidia GPUs~\cite{nvidia2019programming,amperewhite}. We measure the latency $\mathbb{L}$ with commonly used microbenchmarks~\cite{wong2010demystifying,mei2014benchmarking,zhang2017understanding} (The latency measurements are collected in the AD/AE appendix).


\subsection{Concurrency Analysis}

In this section, we briefly describe how we analyze the concurrency to reduce the occupancy of the original kernel in order to release resources for caching while sustaining performance. We conduct a static analysis to extract the data movement operations in the kernel. Note that we account for any barriers in the original kernels that could impact the concurrency of operations, i.e., we do not combine operators/instructions from before and after the barrier when we count the operators. Finally, we apply a simple model to identify the least occupancy we could drop to before the concurrency starts to drop. For example, we did a static analysis of a single precision 2D 5-point Jacobi stencil kernel to conduct a concurrency analysis. It is worth mentioning that the baseline kernel we use is fairly complex since it is highly optimized by using shared memory to reduce traffic to global memory to its minimum~\cite{maruyama2014optimizing}. The results summarized in Table~\ref{tab:concurrencyanalysis} show that for this kernel, we could reduce the original occupancy to ${1/4}^{th}$ while maintaining performance.


To understand the gap between the projected upper-bound on achievable performance and the measured performance ($94.75/138.29=68.52\%$), we inspect the efficiency function $\mathfrak{E()}$. The number of concurrent global memory accesses and shared memory accesses in the 2D 5-point Jacobi stencil kernel are enough to saturate A100 when TB/SM=1. Accordingly, we get $\mathfrak{E}_(\mathbb{C}_{sw=j2d5pt,TB/SM\geq1},\mathbb{C}_{hw=A100})=1$,which would indicate that the observed gap in performance is not due to a drop in concurrency we did not model. While this confirms the effectiveness of the concurrency analysis (i.e., since the concurrency analysis resonates with the empirical measurements in Table~\ref{tab:concurrencyanalysis}), it does not uncover the gap between measured and projected peak achievable. Further investigative profiling revealed that the concurrency for accesses in L2 cache, not global memory, is impacted by reducing occupancy on A100 in specific to the level that affects performance notably. More particularly, access to global memory for the halo region garners a high L2 cache hit rate. This effectively means that higher concurrency is necessary to saturate the L2 cache when hit rates are high. To confirm, we manually doubled the concurrency $\mathbb{C}^{TB}_{sw}$: the performance increased to 123.94 GCells/s with TB/SM=1 (from $68.52\%$ up to $89.6\%$). 


\begin{table}[t]
    \centering
    \caption{Concurrency analysis of global memory accesses of a single precision 2D-5point Jacobi stencil kernel running on A100 (1000 time-steps on $3072^2$ domain)}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{?c?c|c|c|c|c?}
        \tbhline
            \multirow{2}{*}{$\tfrac{TB}{SM}$}  & Used Reg. & Unused Reg. & GM Load & GM Store & Measured\\
              & /SM  &/SM    & op/SM & op/SM  & GCells/s\\\tbhline
            \textit{1} & 32KB  & 224KB  & 2580 & 2048 & 94.75\\
            \textit{2} & 64KB   & 192KB & 5160 & 4096 & 133.24\\
            \textit{8} & 256KB  & 0KB   & 20640 & 16384 & 138.29\\\tbhline
        \end{tabular}
    }
    \label{tab:concurrencyanalysis}
\end{table}




}
\end{comment}

\begin{comment}
{
\subsection{How: Sustaining Performance at Low Concurrency to Free Resources}\label{sec:perconcurrency}

In PERKS, low occupancy is desirable since this releases on-chip resources (scratchpad memory and registers) to be used for caching more data. Yet, low occupancy should not be done in a manner that drops the performance. Volkov et al.~\cite{volkov2010better} explored methods to achieve high performance with low occupancy. Specifically, Volkov et al. reported that performance is not only dictated by Thread Level Parallelism (TLP). We use {\footnotesize$\mathbb{C}_{sw}(\mathbb{OP})$} to represent the parallelism exposed by the kernel, where {\footnotesize$\mathbb{C}_{sw}(\mathbb{OP})$} is the minimum number of concurrently executable instructions of the operation {\footnotesize$\mathbb{OP}$} exposed by the launched kernel. 

The kernel saturates the device only when the minimal concurrency exposed by the kernel is higher than the max concurrency supported by the hardware ({\footnotesize$\mathbb{C}_{hw}$}). 

The hardware concurrency is dictated by {\footnotesize$\mathbb{C}_{hw}$} by throughput {\footnotesize$\mathbb{THR}$} and latency {\footnotesize$\mathbb{L}$}~\cite{volkov2010better}, according to Little's Law~\cite{Little1961APF}: 
\begin{equation}\footnotesize
    \mathbb{C}_{hw}=\mathbb{THR} \cdot \mathbb{L}
\end{equation}
The throughput {\footnotesize$\mathbb{THR}$} for different data access operations are available in the official documentation of Nvidia GPUs~\cite{nvidia2019programming,amperewhite}. We measure latency {\footnotesize$\mathbb{L}$} with commonly used microbenchmarks~\cite{wong2010demystifying,mei2014benchmarking,zhang2017understanding}.% (The latency measurements we collected are reported in detail in the supplementary material). 

We only summarize the concurrency findings due to the space limit.
% (details are in the supplementary material). 
For global memory access operations at the SM level, relying only on TLP requires minimal occupancy (for {\footnotesize$\mathbb{C}_{sw}\geq \mathbb{C}_{hw}$}) of $31.25\%$ (P100), $25\%$ (V100), and $37.5\%$ (A100) to fully saturate the memory bandwidth. Reducing the number of threads launched to meet this minimal occupancy releases the on-chip resources to be used for caching in PERKS. In addition, it is worth mentioning that many well-tuned kernels usually rely more on Instruction Level Parallelism (ILP) to drive concurrency, which means that even lower occupancy can be tolerated (e.g.~\cite{kronbichler2019multigrid,zachariadis2020accelerating,swirydowicz2019acceleration,merrill2016merge}).
\end{comment}
\begin{comment}
\subsection{Concurrency Analysis: single precision 2D 5-point Jacobi stencil as a case study}
\label{sec:2d5ptana}
% \begin{comment}
\begin{table}[t]
	\caption{\revisiona{Hardware concurrency of memory access for double precision values per stream multiprocessors (SM) on P100, V100, and A100 GPUs}}
% \scriptsize
    \centering
	\begin{tabular}{|c|c|c|c|}
	\hline
	 & \textbf{P100}&\textbf{V100}&\textbf{A100}\\\hline
% 	\multicolumn{4}{|c|}{\textbf{Global memory}}\\\hline
	\textbf{$\mathbb{THR}$/SM(GB/s)}~\cite{amperewhite}       & 13    & 12       & 15 \\
	\textbf{$\mathbb{L}$ (ns)}                & 384   & 288       & 407 \\
	\textbf{$\mathbb{C}_{hw}$/SM (B)}      & 4992  & 3456      & 6105   \\
    % $\mathbb{C}^{SM}_{hw}(Double)$ & 624   & 432       & 764   \\
  \textbf{ Min Occupancy($ILP=1$)}  \tablefootnote{Min Occupancy is deduced by assuming that only using TLP for parallelism, and assuming that thread block size is 128}                 & 31.25\%  & 25\%  & 37.5\%     \\\hline	
	\end{tabular}
	\label{tab:lowoccupancy}
% 	{\footnotesize * Min Occupancy is deduced by assuming that only using TLP for parallelism}
\end{table} 
% \end{comment}
% \end{comment}




{
%%The main benefit of performance model is that it could guide optimizations when un-reasonable slowdown is observed. In PERKS performance model is also necessary to ensure that applying PERKS don't harm performance. 

%Even though in this research we haven't encountered, we anticipate 2 scenarios that PERKS might harm performance: 1). The original kernel $\mathbb{KERNEL}$ has high register pressure that any modification might introduce register spill or already suffer from register spill issue, or 2). The $\mathbb{KERNEL}$ is under-optimized that need to rely on large amount of concurrently running threads to ensure performance. 

%Solving first issue is not the purpose of this research, readers can refer to existing register optimizations~\cite{Rawat:2018:AIR:3291656.3291718,Rawat:2018:ROS:3200691.3178500}; yet the second issue can be resolve by using concurrency analysis to guide code optimization. 

% \subsubsection{Use concurrency analysis to reduce thread blocks per stream multiprocessor $TB/SM$ to its minimum}
In this section, we briefly describe how we analyze concurrency to reduce the occupancy of the original kernel in order to release resources for caching while sustaining performance. \revisionb{We use single precision 2D 5-point Jacobi stencil kernel as an example. It is worth mentioning that the baseline kernel we use is fairly complex, since it is highly optimized by using shared memory to reduce traffic to global memory to its minimum~\cite{maruyama2014optimizing}. 

\textbf{Basic measurement.} We profile the kernel to figure out the minimal occupancy we could reduce before performance starts to drop. The results are summarized in Table~\ref{tab:concurrencyanalysis}. The results show that for this kernel, we could reduce the original occupancy to ${1/4}^{th}$ (with {\footnotesize$TB/SM=2$}) while maintaining performance (we could clearly observe a performance drop from {\footnotesize$TB/SM=2$} to {\footnotesize$TB/SM=1$}). \textbf{Important to note that, at this point, we have already released $75\%$ of registers and $87\%$ of shared memory for cache without harming performance and without any modification of the kernel implementation.}

\textbf{Advanced measurement.} We conduct a static analysis to extract the data movement operations in the kernel. Note that we account for any barriers in the original kernels that could impact the concurrency of operation, i.e., we do not combine operators/instructions from before and after the barrier when we count the operators. We further inspect the efficiency function {\footnotesize$\mathfrak{E()}$} on each critical operation. The result shows that the concurrency for accesses in L2 cache, not global memory, is impacted by reducing occupancy on A100 specific to the level that notably affects performance. In particular, access to global memory for the halo region garners a high L2 cache hit rate. This effectively means that higher concurrency is necessary to saturate the L2 cache when hit rates are high. We thus follow Volkov's method~\cite{volkov2010better} to increase concurrency by doubling the ILP. The performance increased to $123.94$ GCells/s with {\footnotesize$TB/SM=1$}. This process released $87.5\%$ of registers and $89\%$ of shared memory.
% \revisionb{\st{To confirm, we manually doubled the concurrency $\mathbb{C}^{TB}_{sw}$: the performance increased to 123.94 GCells/s with TB/SM=1 (from $68.52\%$ up to $89.6\%$). 
} 

% To understand the gap between the projected upper-bound on achievable performance and the measured performance ($94.75/138.29=68.52\%$), we inspect the efficiency function $\mathfrak{E()}$. The number of concurrent global memory accesses and shared memory accesses in the 2D 5-point Jacobi stencil kernel are enough to saturate A100 when TB/SM=1. Accordingly, we get $\mathfrak{E}_(\mathbb{C}_{sw=j2d5pt,TB/SM\geq1},\mathbb{C}_{hw=A100})=1$,which would indicate that the observed gap in performance is not due to a drop in concurrency we did not model. While this confirms the effectiveness of the concurrency analysis (i.e., since the concurrency analysis resonates with the empirical measurements in Table~\ref{tab:concurrencyanalysismain}), it does not uncover the gap between measured and projected peak achievable. Further investigative profiling revealed that the concurrency for accesses in L2 cache, not global memory, is impacted by reducing occupancy on A100 in specific to the level that affects performance notably. More particularly, access to global memory for the halo region garners a high L2 cache hit rate. This effectively means that higher concurrency is necessary to saturate the L2 cache when hit rates are high. 
% \revisionb{\st{To confirm, we manually doubled the concurrency $\mathbb{C}^{TB}_{sw}$: the performance increased to 123.94 GCells/s with TB/SM=1 (from $68.52\%$ up to $89.6\%$).}}

% (as empirical benchmarking in Table~\ref{tab:concurrency} confirms)




%So, \textbf{no necessary to launch thousands of threads to saturate device. An alternative solution is to launch fewer threads with more unblocked operations.}

%The guess is that this larger desire for L2 cache concurrency might due to the 2 slice design of A100 chip. 
%We also put the experiment of running with $\mathbb{D}=3072^2$ in the same table. 


\begin{table}[t]
    \centering
    \caption{\revisionb{Performance analysis of different thread block per treaming multiprocessor ($\tfrac{TB}{SM}$) in a single precision 2D-5point Jacobi stencil kernel running on A100 with 256 threads per thread block (1000 time-steps on $3072^2$ domain).}}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{?c?c|c|c|c|c|c|c?}
        \tbhline
            \multirow{2}{*}{$\tfrac{TB}{SM}$}  & Used  & Unused  & Used  & Unused   & Perf\\
              & Reg./SM  &Reg./SM & sm/SM  &sm/SM      & GCells/s\\\tbhline
            \textit{1} & 32KB  & 224KB  & 10 KB & 154 KB & 94.75\\
            \textit{2} & 64KB   & 192KB & 20 KB & 144 KB  & 133.24\\
            \textit{8} & 256KB  & 0KB   & 81 KB & 83 KB  & 138.29\\\tbhline
        \end{tabular}
    }
    \label{tab:concurrencyanalysismain}
\end{table}

% \begin{comment}
\begin{table}[t]
    \centering
    \caption{Concurrency analysis of global memory accesses of a single precision 2D-5point Jacobi stencil kernel running on A100 (1000 time-steps on $3072^2$ domain)}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{?c?c|c|c|c|c|c|c?}
        \tbhline
            \multirow{2}{*}{$\tfrac{TB}{SM}$}  & Used  & Unused  & Used  & Unused  & GM Load & GM Store & Perf\\
              & Reg./SM  &Reg./SM & sm/SM  &sm/SM    & op/SM & op/SM  & GCells/s\\\tbhline
            \textit{1} & 32KB  & 224KB  & 10 KB & 154 KB& 2580 & 2048 & 94.75\\
            \textit{2} & 64KB   & 192KB & 20 KB & 144 KB & 5160 & 4096 & 133.24\\
            \textit{8} & 256KB  & 0KB   & 81 KB & 83 KB & 20640 & 16384 & 138.29\\\tbhline
        \end{tabular}
    }
    \label{tab:concurrencyanalysismain}
\end{table}
% \end{comment}

}

\subsection{How PERKS is effective}\label{sec:howperks}

What PERKS different from traditional GPU programming is it uses chip-wide synchronization to replace kernel launch (as implicit barrier) and then caches data with on-chip resources. In this section, we quantificationally analyze the trade-off between saving memory traffic and the overhead of chip-wide synchronization with a thought experiment. 

\textbf{Scenario} A constant data that needed to be reloaded one time upon each kernel launch (e.g., the matrix in conjugate gradient solver). 

\textbf{Assumption} Able to use $50\%$ of shared memory for cache. 

\textbf{Revenue of PERKS ({\footnotesize$\mathbb{R}$})} The memory traffic saved would be the ({\footnotesize$\mathbb{R}$}) of applying PERKS. Based on Nvidia's document~\cite{nvidiaa100} we could deduce that {\footnotesize$\mathbb{M}(\text{Cache 50\% Shared Memory})=$} $2.55$ ns (P100), $4.37$ ns (V100), and $5.83$ ns (A100).

\textbf{Cost of PERKS ({\footnotesize$\mathbb{C}$})} \todo{@Wahib: It is also OK to remove the COST part. We could stop at the overhead is the same level.} The cost of applying PERKS is to use chip-wide synchronization to replace kernel launch. Though we assume that the overhead of chip-wide synchronization ({\footnotesize$\mathbb{O}(explicit\ barrier)$}) is the same as the overhead of kernel launch ({\footnotesize$\mathbb{O}(implicit\ barrier)$}), we can deduce the upper bound of such cost ({\footnotesize$\mathbb{C}=\mathbb{O}(explicit\ barrier)-\mathbb{O}(implicit\ barrier)$}). Based on Zhang etc.'s research~\cite{zhang2020study}: {\footnotesize$\mathbb{C}(PERKS)\leq$} 2.5 ns ({\footnotesize$\tfrac{TB}{SM}\leq2$}). 

\textbf{Profit of PERKS ({\footnotesize$\mathbb{P}=\mathbb{R}-\mathbb{C}$})} {\footnotesize$\mathbb{P}(\text{Cache 50\% Shared Memory})\geq$} $0.05$ ns (P100), $1.87$ ns (V100), and $3.33$ ns (A100), per time step. A more significant amount of time step would amplify this performance benefit. 
% The performance benefit would be amplified as the amount of time step increases.  

% This is a simplified analysis that dismissed many factors, e.g. possibility of using register for cache, and situations that data be reused more then one times. 
% \begin{comment}


\begin{table}[t]
    \centering
    \caption{\revisiona{The memory related parameters of the latest Nvidia GPUs\cite{nvidiaa100} and the anticipated time for loading data to fill 50\% of shared memory}}% SM is Steam Multiprocessor}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{?l?c|c|c?}\tbhline
    \textbf{Feature}    & \textbf{P100} & \textbf{V100}  & \textbf{A100}  \\\hline
    \textbf{Shared memory}~\tablefootnote{\emph{Shared memory} is a configurable portion of L1 cache that can be used as a user-managed scratchpad memory} 
    & 3.5 MB & 7.5 MB & 17.29 MB \\
    \textbf{Register files} &14 MB &20MB&27MB\\
    \textbf{L2 cache }    & 4 MB & 6 MB  & 40 MB  \\
    \textbf{Memory bandwidth}    & 720 GB/s & 900 GB/s  & 1555 GB/s  \\\hline
    \textbf{Time }    
    &   &  &  \\
    \textbf{(Fill $50\%$ shared memory)}    
    &  2.55 ns & 4.37 ns & 5.83 ns \\\hline
    % \textbf{Time}    &   &  & \\
    % \textbf{(Fill $50\%$ of register files)}    &  10.19 ns & 11.65 ns & 9.10 ns \\\hline
    \end{tabular}
    \label{tab:gpu_loadsmltc}
    }
\end{table}
% \end{comment}
% As a comparison, considering the domain of $8192^2$ in double precision 2D stencil domain size used in previous research. The total domain size is 

% Also, worth mentioning that we can use the large register files in the latest GPUs, and we haven't considered the scenario when unnecessary storing data also happens (e.g., stencil) (memory transactions doubled). In these situations, an even more significant amount of memory traffics could be saved by applying PERKS. For example, in double precision 2D 5-point Jacobian stencil in A100, a total size of 20.25 MB space can be cached, saving $27.31$ ns per time step. 




% And this potential would be even more significant in the situation of iterative solvers when the memory traffics is reduced amplify as the number of iteration increases. 

\color{black}
% \end{comment}

\end{comment}
\begin{comment}
\subsection{Concurrency Analysis}
\label{sec:conan}

In this section, we briefly describe how we analyze the concurrency to reduce the occupancy of the original kernel in order to release resources for caching while sustaining performance. We conduct a static analysis to extract the data movement operations in the kernel. Note that we account for any barriers in the original kernels that could impact the concurrency of operations, i.e., we do not combine operators/instructions from before and after the barrier when we count the operators. Finally, we apply a simple model to identify the least occupancy we could drop to before the concurrency starts to drop. For example, we did a static analysis of a single precision 2D 5-point Jacobi stencil kernel to conduct a concurrency analysis. It is worth mentioning that the baseline kernel we use is fairly complex since it is highly optimized by using shared memory to reduce traffic to global memory to its minimum~\cite{maruyama2014optimizing}. The results summarized in Table~\ref{tab:concurrencyanalysis} show that for this kernel, we could reduce the original occupancy to ${1/4}^{th}$ while maintaining performance.


To understand the gap between the projected upper-bound on achievable performance and the measured performance ($94.75/138.29=68.52\%$), we inspect the efficiency function $\mathfrak{E()}$. The number of concurrent global memory accesses and shared memory accesses in the 2D 5-point Jacobi stencil kernel are enough to saturate A100 when TB/SM=2. Accordingly, we get $\mathfrak{E}_(\mathbb{C}_{sw=j2d5pt,TB/SM\geq2},\mathbb{C}_{hw=A100})=1$,which confirms the effectiveness of the concurrency analysis (i.e., since the concurrency analysis resonates with the empirical measurements in Table~\ref{tab:concurrencyanalysis}). Further \revisiona{investigation} revealed that the concurrency for accesses in L2 cache, not global memory, is impacted by reducing occupancy on A100 in specific to the level that affects performance notably. More particularly, access to global memory for the halo region garners a high L2 cache hit rate. This effectively means that higher concurrency is necessary to saturate the L2 cache when hit rates are high. To confirm, we manually doubled the concurrency $\mathbb{C}^{TB}_{sw}$: the performance increased to 123.94 GCells/s with TB/SM=1 (from $68.52\%$ up to $89.6\%$). 

\begin{table}[t]
    \centering
    \caption{Concurrency analysis of global memory accesses of a single precision 2D-5point Jacobi stencil kernel running on A100 (1000 time-steps on $3072^2$ domain)}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{?c?c|c|c|c|c?}
        \tbhline
            \multirow{2}{*}{$\tfrac{TB}{SM}$}  & Used Reg. & Unused Reg. & GM Load & GM Store & Measured\\
              & /SM  &/SM    & op/SM & op/SM  & GCells/s\\\tbhline
            \textit{1} & 32KB  & 224KB  & 2580 & 2048 & 94.75\\
            \textit{2} & 64KB   & 192KB & 5160 & 4096 & 133.24\\
            \textit{8} & 256KB  & 0KB   & 20640 & 16384 & 138.29\\\tbhline
        \end{tabular}
    }
    \label{tab:concurrencyanalysis}
\end{table}

\end{comment}

% \subsection{Why: Potential Performance Gain in PERKS}\label{sec:howperksreduces}
% \subsection{Why: \revisiona{PERKS don't influence efficiency}}\label{sec:practicalbound}
\subsection{\revisiona{Practical Bound}}\label{sec:practicalbound}

% \revisiona{Intuitively, the more data cached the higher speedup PERKS provide. However, in iterative solvers like stencil, inter thread block communication might still remained in the cached portion of domain. We use a practical bound on the performance gain in PERKS to assess the performance gain of cache over the overhead of handling dependence.}

A practical bound on the performance is useful to assess the
%quality of PERKS implementation 
\revisiona{efficiency of an implementation}
and to identify adverse effects of unforeseen pressure on resources.
We rely on the FOM (Figure of Merit) as a performance metric in this analysis. In stencils, we use the giga-cells updated per second (GCells/s)~\cite{DBLP:conf/cgo/MatsumuraZWEM20,chen2019versatile}. Given the memory-bound nature of the conjugate gradient solver, we directly use sustained memory bandwidth as a metric, following other works on conjugate gradient that use the same metric~\cite{anzt2020ginkgo}. Due to space limitations, this section mainly focuses on stencils to explain performance analysis. Without loss of generality, the analysis is applicable to other cases (ex: conjugate gradients) by adjusting the performance metric and code concurrency accordingly.



We use a simple, yet effective, model inspired by the roofline model~\cite{ofenbeck2014applying,kim2011performance}. The model's utility is to project the upper bound on performance gain based on the reduction of global memory traffic. 

%\revision{Before and after} a kernel implemented as PERKS,
When only a portion of the domain is cached, the bottleneck is the global memory bandwidth. In this analysis, we do not consider the case when the PERKS caching moves the bottleneck to become the shared memory bandwidth, which is usually the case when the domain is fully cached. We do not assume the registers to be a bottleneck since we assume that as long as we ensure that no register spilling occurs, we avoid adverse register pressure.
%the bottleneck would be either the global memory bandwidth or the shared memory bandwidth (if the PERKS caching scheme moves the bottleneck to become the shared memory bandwidth, which is usually the case when the domain is fully cached). We don't assume the registers to be a bottleneck since we assume that as long as we ensure that no register spilling occurs, we avoid adverse register pressure.

We initially do not account for the memory accesses to global memory originating from the boundary threads in each thread block, e.g., halo region in stencil, and confine our analysis to the dependency in cached region. We then expand our analysis later in the section to consider those unavoidable global memory accesses (Equation~\ref{eqt:mainperkhalo}).

We assume a total domain of size {\footnotesize$\mathbb{D}$} bytes, the cached portion to be {\footnotesize$\mathbb{D}_{cache}$} bytes, and the uncached portion to be {\footnotesize$\mathbb{D}_{uncache}=\mathbb{D}-\mathbb{D}_{cache}$} bytes. The cached portion of domain data would be divided between registers and shared memory (since we cache in both registers and shared memory): {\footnotesize$\mathbb{D}_{cache}=\mathbb{D}^{sm}_{cache}+\mathbb{D}^{reg}_{cache}$}. For $N$ time steps, assuming that the number of bytes stored to global memory in each time step is $\mathbb{S}_{gm}$ and the number of bytes loaded is $\mathbb{L}_{gm}$, the total global memory bytes accessed $\mathbb{A}_{gm}$ becomes:

\begin{equation}\footnotesize
\begin{aligned}
    \mathbb{A}_{gm}(\mathbb{D})=N\cdot(\mathbb{L}_{gm}+\mathbb{S}_{gm})
    &=2\cdot N\cdot \mathbb{D}_{uncache} + 2\cdot  \mathbb{D}_{cache}    
\end{aligned}
\end{equation}


% In the case when the kernel is bounded by global memory bandwidth, i.e., the volume of cached data does not move the bottleneck from global memory to shared memory, 
For the global memory bandwidth of {\footnotesize$\mathbb{B}_{gm}$} and the size of the data type of {\footnotesize$\mathfrak{S}(type)$}, the time {\footnotesize$\mathbb{T}_{gm}(\mathbb{D})$} for accessing the global memory becomes:
\begin{equation}\footnotesize
    \begin{aligned}
                \mathbb{T}_{gm}(\mathbb{D})={{\mathbb{A}_{gm}(\mathbb{D})\cdot \mathfrak{S}(type)}}/{{\mathbb{B}_{gm}}}
    \end{aligned}
    \label{eqt:time_gm}
\end{equation}

% In the case when the kernel is bounded by shared memory bandwidth, i.e., the volume of data cached in shared memory moves the bottleneck to be the shared memory bandwidth, the total shared memory (in bytes) accessed $\mathbb{A}_{sm}$ becomes: 

% \begin{equation}\footnotesize
% \begin{aligned}
%     \mathbb{A}_{sm}(\mathbb{D}_{cache}^{sm})=N\cdot(\mathbb{L}_{sm}+\mathbb{S}_{sm})=2\cdot (N-1)\cdot \mathbb{D}_{cache}^{sm}    		
% \end{aligned}
% \end{equation}
% Assuming {\footnotesize$\mathbb{A}_{sm}(\mathbb{KNEL})$} to be the shared memory originally used by the kernel, e.g., shared memory used in the baseline implementation of a stencil kernel to improve the locality, and $\mathbb{B}_{sm}$ to be the shared memory bandwidth, the time {\footnotesize$\mathbb{T}_{sm}(\mathbb{D})$} for accessing the shared memory becomes:
% \begin{equation}\footnotesize
%     \begin{aligned}
%         \mathbb{T}_{sm}(\mathbb{D}_{cache}^{sm})=\{{{(\mathbb{A}_{sm}(\mathbb{D}_{cache}^{sm})+\mathbb{A}_{sm}(\mathbb{KNEL}))\cdot \mathfrak{S}(type)}}\}/{{\mathbb{B}_{sm}}}
%     \end{aligned}
%     \label{eqt:time_sm}
% \end{equation}

Next, we consider the unavoidable global memory accesses necessary to resolve the neighborhood dependencies in {\footnotesize$\mathbb{D}_{cache}$}, e.g., the halo region of stencils. In the cached portion of the domain, the halo region requires global memory accesses to resolve the dependencies. Assuming the global memory accesses, in bytes, for the halo region of the data computed by the boundary threads in thread blocks that are in the cached portion of the domain to be {\footnotesize$\mathbb{A}_{gm}(\mathfrak{H}(\mathbb{D}_{cache}))$}, the time for accessing those halo region {\footnotesize$\mathbb{T}_{gm}(\mathfrak{H}(\mathbb{D}_{cache}))$} would be:
\begin{equation}\footnotesize
    \begin{aligned}
          \mathbb{T}_{gm}(\mathfrak{H}(\mathbb{D}_{cache}))={\mathbb{A}(\mathfrak{H}(\mathbb{D}_{cache}))\cdot \mathfrak{S}(type)}/{\mathbb{B}_{gm}}
    \end{aligned}
    \label{eqt:mainperkhalo}
\end{equation}
The best-case bound on the total time required for the PERKS kernel may be written as:
\begin{equation}\footnotesize
    \begin{aligned}
    %  \mathbb{T}_{PERKS}=\max(\mathbb{T}_{gm}(\mathbb{D})+\mathbb{T}_{gm}(\mathfrak{H}(\mathbb{D}_{cache})),\mathbb{T}_{{sm}})
     \mathbb{T}_{PERKS}=\mathbb{T}_{gm}(\mathbb{D})+\mathbb{T}_{gm}(\mathfrak{H}(\mathbb{D}_{cache}))
    \end{aligned}
    \label{eqt:maxlat}
\end{equation}
Accordingly, the projected bound on performance gain ($\mathbb{P}$) for the $N$ time steps can be expressed as:
\begin{equation}\footnotesize
    \begin{aligned}
     \mathbb{P}={\mathbb{D} \cdot N}/{\mathbb{T}_{PERKS}}
    \end{aligned}
    \label{eqt:maxpeak}
\end{equation}



% \todo{change to double precision}

To further illustrate how this performance analysis works, 
we give a examples while computing $N=1000$ time-steps of a double precision 2D 5-point Jacobi stencil on A100. We use the domain size {$\mathbb{D}=3072^2$} as an example. 

\revisiona{We can get the practical bound of the kernel before applying PERKS by assuming that the total cacheable region is $0$. In this case, we have: $\mathbb{T}_{SHM}(\mathbb{D})=97.10$ ms. So, {$\mathbb{P}_{SHM}=3072^2\cdot 1000/\mathbb{T}_{SHM}= 97.18$ GCells/s. The measured result is $77.30$ GCells/s ($79.54\%$ of the upper bound)}.}

The total cacheable region is {$\mathbb{D}_{cache}=3072\times1512$} leading to {$\mathbb{T}_{gm}(\mathbb{D})=49.36$ ms}. The total number of bytes for the halo accesses is {$\mathbb{A}(\mathfrak{H}(\mathbb{D}_{cache}))=1000\cdot2\cdot 108\cdot(168\cdot2+256\cdot2)$}. Thus $\mathbb{T}_{gm}(\mathfrak{H}(\mathbb{D}_{cache}))= 50.30$ ms. So {$\mathbb{P}_{PERKS}=3072^2\cdot 1000/\mathbb{T}_{PERKS}= 187.62$ GCells/s} would be the practical bound on performance gain. The measured result is $112.04$ GCells.s ($59.72\%$ of the upper bound).

\revisiona{So, in this specific case, transporting to PERKS loses $25\%$ of efficiency. }

% In the supplementary material, we elaborate on the analysis of concurrency and its impact on the gap between measured and bound on performance gain.

\begin{comment}
We use the domain size {$\mathbb{D}=3072^2$} as an example of a partially cached domain; the total cache-able region is {$\mathbb{D}_{cache}=3072\cdot2448$} leading to {$\mathbb{T}_{gm}(\mathbb{D})=9900.70$ us}. The total number of bytes for the halo accesses is {$\mathbb{A}(\mathfrak{H}(\mathbb{D}_{cache}))=1000\cdot2\cdot 216\cdot(136\cdot2+256\cdot2)$}. Thus $\mathbb{T}_{gm}(\mathfrak{H}(\mathbb{D}_{cache}))= 871.22$ us. So {$\mathbb{P}_{PERKS}=3072^2\cdot 1000/\mathbb{T}_{PERKS}= 876.09$ GCells/s} would be the practical bound on performance gain. In the supplementary material, we elaborate on the analysis of concurrency and its impact on the gap between measured and bound on performance gain.
\end{comment}
\begin{comment}
\subsection{{Why PERKS is Feasible in the latest Nvidia GPUs}}\label{sec:whyperks}

This section summarizes the three hardware development in GPUs that make PERKS feasible now.

First, a fewer amount of warps is required for CUDA runtime to hide the latency effectively, since the latency of most compute, data, and control operations dropped signficnatnly in recent generations of GPUs~\cite{jia2018dissecting}. We discussed the sufficiency of low occupancy in Section~\ref{sec:perconcurrency}. 

Second, a new explicit device-wide synchronization API released in CUDA 9.0 (2017) provides the possibility to reuse on-chip resources between device-wide barriers with lower overhead (Section~\ref{sec:backsync}). The overhead is further reduced in the newer GPU generations~\cite{amperewhite}.

Third, as reported by Nvidia developer guides~\cite{nvidiaa100}, on-chip resources have increased from 17.5 MB in P100 (2016) to 44.29 MB in A100 (2020) ($2.53$x larger in 4 years). This provides a further benefit for PERKS since it increases the capacity for caching. %The cost of 
\end{comment}

% \begin{comment}

\revisiona
{

\subsection{How PERKS Effectively Speedup Base Kernel}\label{sec:howworks}
Based on the analysis in Section~\ref{sec:practicalbound}, we observed that the overhead of halo access only takes $1.9\%$ of the total runtime. If we assume that the overhead of handling dependency is negligible, based on Equation~\ref{eqt:maxlat}, we have:

\begin{equation}\footnotesize
    \begin{aligned}
     \mathbb{T}_{PERKS}\approx(\mathbb{T}_{gm}(\mathbb{D}))
    \end{aligned}
\end{equation}

Accordingly, we have the following:
\begin{equation}\footnotesize
\begin{aligned}
    \mathbb{P}_{PERKS+basekernel}&\approx \mathbb{P}_{basekernel} \times \frac{\mathbb{D}}{\mathbb{D}-\mathbb{D}_{cache}}
\end{aligned}
\label{eqt:projectionLarge}
\end{equation}
% \todo{change to double precision}
For example, in the implementation of a single-precision 2D 5-point Jacobian stencil at a domain size of $3072^2$, we set the thread block = 256. In the baseline kernel (SHM), we measured that the kernel achieved a peak performance of $77.30$. After porting the kernel to PERKS, we can cache $49.22\%$ of the domain. So {${\mathbb{D}}/{(\mathbb{D}-\mathbb{D}_{cache})}=$}$1.97$x. The measured speedup is $1.47$x ($74.6\%$ of the model, as we lose about $25\%$ efficiency in this case).

\subsection{Why PERKS is Effective, a Statistics Perspective}\label{sec:whyworks}
We observe a certain level of inefficiency while analyzing the result with the practical bound. We can assume that the efficiency of an implementing PERKS is $eff$. We can add this to Equation~\ref{eqt:projectionLarge}, and, the speedup to be:  
\begin{equation}\footnotesize
\begin{aligned}
    Speedup =  eff\times\frac{\mathbb{D}}{\mathbb{D}-\mathbb{D}_{cache}}
\end{aligned}
\label{eqt:speedup}
\end{equation}

In stencil implementations, on average, we achieved $70.22\%$ efficiency in the SHM kernel and $69.52\%$ efficiency in the PERKS (SHM) kernel. So $eff=99.00\%$. So, we need, on average, $1.00\%$ of the domain to be cached to obtain a speedup. In stencil implementations, we, on average, cache $30.76\%$ of the domain. So we expect that PERKS consistently speedup SHM. 
}


\begin{comment}


Yet, after transforming the code to PERKS, the max $TB/SM$ is 2. We measured different $TB/SM$ settings for baseline and PERKS and put them in Table~\ref{tab:projection}. We also use Equation~\ref{eqt:projectionLarge} to project the performance based on the percentage of region cached and put the result in the same Table. 

\begin{table}[t]
    \centering\small
    \caption{Single precision $3702\times3702$ 2D 5-point Jacobian stencil in A100, performance of SM-OPT, PERKS, and the relationship between speedup and the cached proportion.}
    \begin{tabular}{|c|c|c|c|c|c|}
    \hline
        \multirow{2}{*}{$\tfrac{TB}{SM}$}  & SM-OPT & \multirow{2}{*}{$\tfrac{\mathbb{D}_{cache}}{\mathbb{D}}$} &  \multirow{2}{*}{$\tfrac{\mathbb{D}}{\mathbb{D}-\mathbb{D}_{cache}}$} & PERKS  & PERKS\\
          & GCells/s &&  &GCells/s&Speedup\\\hline
        1 & 94.87   & 77.34\% & 4.41   & 357.79& 3.77\\
        2 & 133.41  & 79.69\% & 4.92   & 444.55& 3.33\\ 
        8 & 137.65  & -       & - & -&-\\\hline
    \end{tabular}
    \label{tab:projection}
\end{table}

According to Table~\ref{tab:projection}, the Projection Model's accuracy is generally more than 67\%. So, this model can anticipate the potential speedup of applying PERKS without the knowledge of concurrency~\cite{volkov2010better}. 

\end{comment}

==> Apendixes/x00_summarizePERKS.tex <==
\section{{Why PERKS is Feasible in the latest Nvidia GPUs}}\label{sec:whyperks}

This section summarizes the three hardware development in GPUs that make PERKS feasible now. First, a fewer amount of warps is required for CUDA runtime to hide the latency effectively, since the latency of most compute, data, and control operations dropped significantly in recent generations of GPUs~\cite{jia2018dissecting}. We discussed the sufficiency of low occupancy in Section~\ref{sec:perconcurrency}. 

%Also, we can find traces in literature. On one side, the CUDA programming guide~\cite{nvidia2019programming} shows a trend of reducing throughput per stream multiprocessor. On the other hand, if we compare the latency result in existing microbenchmarks~\cite{wong2010demystifying,jia2018dissecting} we can also observe a reduction in instruction latency. Both trends result in a lower hardware concurrency per stream multiprocessor in newer generation GPUs. 

Second, a new explicit device-wide synchronization API released in CUDA 9.0 (2017) provides the possibility to reuse on-chip resources between device-wide barriers with lower overhead (Section~\ref{sec:backsync}). The overhead is further reduced in the newer GPU generations~\cite{amperewhite}.

Third, as reported by Nvidia developer guides~\cite{nvidiaa100}, on-chip resources have increased from 17.5 MB in P100 (2016) to 44.29 MB in A100 (2020) ($2.53$x larger in 4 years). This further benefits PERKS since it increases the capacity for caching. 

% Zhang etc.~\cite{zhang2020study} did a comprehensive research on this and showed that the difference in overhead between explicit device-wide synchronization and implicit device-wide synchronization is largely negligible. 

\begin{table}[t]
    \centering
    \caption{The memory related parameters of the latest Nvidia GPUs\cite{nvidiaa100}}% SM is Steam Multiprocessor}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{?l?c|c|c?}\tbhline
    \textbf{Feature}    & \textbf{P100} & \textbf{V100}  & \textbf{A100}  \\\hline
    \textbf{Shared memory}~\tablefootnote{\emph{Shared memory} is a configurable portion of L1 cache that can be used as a user-managed scratchpad memory} 
    & 3.5 MB & 7.5 MB & 17.29 MB \\
    \textbf{Register files} &14 MB &20MB&27MB\\
    \textbf{L2 cache }    & 4 MB & 6 MB  & 40 MB  \\
    \textbf{Memory bandwidth}    & 720 GB/s & 900 GB/s  & 1555 GB/s  \\\hline
    % \textbf{Time}    &   &  & \\
    % \textbf{(Fill $50\%$ of register files)}    &  10.19 ns & 11.65 ns & 9.10 ns \\\hline
    \end{tabular}
    \label{tab:gpu_loadsmltc}
    }
\end{table}

==> Apendixes/x01_considerations.tex <==
\section{PERKS and CUDA Considerations}
\subsection{Restrictions of Synchronization APIs}
PERKS highly relies on cooperative groups related APIs (supported since CUDA 9.0~\cite{nvidia2021api}). Currently, the API does not allow over-subscription, i.e., one needs to explicitly assign workload to blocks and threads to expose enough parallelism to the device. However, it is worth mentioning that this API does not limit the flexibility, as different kernels can still run concurrently in a single GPU, as long as they as a whole doesn't exceed the hardware limitation.

\subsection{New Features in Nvidia Ampere}
The Nvidia Ampere generation of GPUs introduced two new features that have the potential to improve the performance of PERKS. Namely, asynchronous copy for shared memory and L2 cache residency control~\cite{nvidiaa100}. When testing asynchronous copy to cache in PERKS, we did not observe noticeable performance difference. For L2 cache residency control, we experimented with setting the input and halo region to be persistent. We observed $8\%$ slowdown and no change in performance, respectively. Accordingly, we do not use those new features in our PERKS implementations.

\subsection{Register pressure in PERKS} 
One concern with PERKS is that kernels might run into register pressure if the compiler is not optimally reusing registers for different time steps, potentially affecting concurrency and penalizing performance. To illustrate this issue, take a high register-pressure 2D 25-point double precision Jacobi stencil as an example. The shared memory optimized baseline version (SM-OPT) uses $78$ registers per thread, yet the PERKS version uses $112$ registers\footnote{We gathered the number of registers used by finding the maximum number of registers available as cache before spilling with "\_\_launch\_bounds\_\_" instruction. Register spilled can be indicated by '-Xptxas "-v -dlcm=cg"' flag.}. Similar behavior is also observed in other stencil benchmarks. Reducing the occupancy while maintaining the concurrency --as mentioned in the previous section-- reduces the impact of this compiler's inefficiency in register reuse in all the benchmarks we report in the results section. In the above example, at worst, $48$ registers among the maximum available $178$ registers per thread could not be used for caching data; it neither harms concurrency nor triggers register spilling. 

\begin{table}[t]
    \centering
    \caption{Register information of single precision 2d5pt and double precision 2ds25pt}
    \begin{tabular}{|c|c|c|}
    \hline
        TYPE & 2d5pt(f)  & 2ds25pt(d)  \\\hline
        SM-OPT            & 32  & 78 \\
        PERKS(SM-OPT)                    & 32  & 112\\
        PERKS(SM-OPT) with $D_{cache}^{sm}$& 32  & 126\\\hline
    \end{tabular}
    \label{tab:registeranalysis}
\end{table}



==> Apendixes/x02_ResultsDetails.tex <==
\section{Caching}
\subsection{Caching Policy}\label{sec:cachepolicy}

A caching policy is required to determine which portion of the domain (or data) to cache. When the entire domain (or data) can fit in register files and shared memory used for caching, the entire algorithm can run from the cache (this is particularly useful in the cases of strong scaling where per node domain size becomes smaller as the number of nodes grows). When only a fraction of the domain can be cached, a policy is required to select the data to prioritize for caching. In the following sections, we elaborate on the caching policy.

\subsubsection{Considerations for dependency between threads Blocks} 
Algorithms that do not require dependency between the thread blocks can use the cache space most efficiently because all the load and store transactions to global memory can be eliminated. The dependencies within the thread block are resolved by using either the shared memory or shuffle operations.

In iterative solvers, there is often neighbor dependency (ex: a stencil kernel where a cell update relies on values computed in neighboring threads). In such a case, caching the results of the threads at the interior of the CUDA thread blocks eliminates the stores and loads from global memory. The threads at the boundary of threads blocks would, however, continue to store and load from global memory (since the shared memory scope is the thread block). When the capacity of cache is large enough, w.r.t. the domain size to be cached, the performance drawback would be negligible. 

\subsubsection{Identifying which data gets priority to be cached}

In many cases, the capacity of register files and shared memory is limited, i.e., it is impossible to cache the entire domain/input. In cases where all the domain/input array elements are accessed at the same frequency, one could assume it is unnecessary to use a cache policy that prioritizes specific parts of the domain/input. However, this is not always true.

Take iterative stencil as an example. The data managed by the threads at the boundary of the thread block is stored to main memory to be accessed by the neighboring threads blocks in the following iterations; caching those boundary elements saves one load operation. On the other hand, data at the interior of the thread block is not involved in inter thread block dependency; caching saves one load and one store operation. Finally, data in the halo region is updated at each time step; there is no benefit in caching the layers in the halo region. To conclude, the priority in caching yielding the highest reuse would be: {\footnotesize $Data_{no\_inter\_TB\_dependency}>Data_{inter\_TB\_dependency}$}, i.e., the priority is to cache the data of the interior threads of the thread block, followed by the data of the threads at the boundary of the thread block, and no caching for the halo region.

For other iterative solvers, such as conjugate gradient, there are different data arrays that could be potentially cached, unlike a single domain array in stencils. The cacheable variables and usage per array element for the conjugate gradient solver are as follows: a) one load and no stores for the matrix {$\mathbf{A}$}, and b) three loads and one store for the residual vector {$\mathbf{r}$}. So by assuming that each operation accesses data in a coalesced access pattern, it would be more effective to cache vector {$\mathbf{r}$}. As a result, the ideal cache priority is {\footnotesize$\mathbf{r}>\mathbf{A}$}.

To summarize, while PERKS does not touch on the compute part of the original kernel, attention should be given to identifying the ideal caching policy for each solver implemented as PERKS. That being said, one could assume this step can be automated by using a dedicated profile-guided utility (or even sampling from the profiler directly) to aid the user in swiftly identifying an ideal caching policy, based on the access patterns and frequency of access of data arrays in the solver.


\subsection{Detailed Results}
\subsubsection{Where to Cache: Shared Mem., Registers, or Both?}

\label{sec:caching:where}
The intuition is that using both shared memory and registers would always be better (more cache-able space). The results show that this is usually the case. There can, however, be exceptions. For instance, in our observations, we see that for higher order stencils, using shared memory and registers is often not the ideal choice (presumably due to arising register pressure).

\subsubsection{What to Cache?}
\label{sec:what:cache}
We highlight important observations when varying the data to cache in the conjugate gradient solver. First, the implicit cache policy ($IMP$) achieves a geometric mean of $3.63$x and $1.21$x over Ginkgo for dataset sizes both within and (surprisingly) when exceeding L2 cache, respectively. This means \textbf{PERKS can gain speedup before applying any explicit caching policy} by getting hits in the L2 cache. Second, the speedup difference between caching the vector ($VEC$) or not is usually insignificant for most situations. This is likely because the vectors are generally not large enough to consume all available cache resources. Third, as expected, the general tendency is that the more PERKS caches, the more speedup there is. So we generally get the highest speedup with caching the matrix ($MAT$) or caching both the vector and matrix ($MIX$). The exception is in the case of single precision when the dataset sizes exceed L2 cache: we still get speedup from $MAT$ and $MIX$, though not the highest speedup. 
\subsubsection{What Should the End-user Do?}
\label{sec:summary:cache}
In summary, the cache location analysis for stencil and the cache policy analysis for conjugate gradient (which is a fairly complex solver) shows that a simple greedy approach of targeting the largest data arrays in as many caching resources as possible gives mostly the best performance. While there can be outliers, the simple greedy policy is, in most cases, effective enough, and also simple for end-users (since they only need to identify the arrays generating the most traffic).


\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{FIG/stencilheatmap.pdf}
\caption{Heatmap of speedup over non-PERKS baseline (SM-OPT) when caching data in different locations, for different stencils.}
\label{Fig:stheatmap}
\end{figure}

\begin{figure}[t]
\centering
\textcolor{white}
{
\frame
{\includegraphics[width=\linewidth]{FIG/cgheatmap.pdf}}}
\caption{ Heatmap of speedup over Ginkgo~\cite{anzt2020ginkgo} when using different caching policies in the conjugate gradient solver (iterative method to solve $Ax=b$).
}
\label{Fig:cgpolicy}
\end{figure}

==> Apendixes/x03_performanceanalysis.tex <==
\section{Performance Analysis}\label{appendix}

First, We propose a projection of achievable performance that we compare with measured results to detect abnormal behavior or implementation shortcomings. We relied on this projection to analyze our PERKS implementation quality (Section~\ref{sec:peakperform}).

Second, We identify the bounds on reducing concurrency before dropping performance and use concurrency to explain potential optimizations for further performance improvement (Section~\ref{sec:apdconan}). 

\textbf{We emphasize that:} we use the analysis to understand the quality of our implementation and address its implication on performance. However, the concurrency analysis is not a requirement for porting kernels to PERKS;  In contrast, end-users wishing to port the kernel to PERKS need only to satisfy the concurrency requirements by setting the device occupancy to minimum occupancy while maintaining performance (Section~\ref{sec:enduser}). 

Finally, we also provide an empirical performance model for end-users in the large domain, which projects the speedup before applying PERKS without the knowledge of concurrency analysis (Section~\ref{sec:empmodel}). 


\subsection{Overview}
This performance analysis relies on three performance attributes: a) measured performance $\mathbb{M}$ of our PERKS implementation, b) the projected peak performance $\mathbb{P}$ achievable on a given GPU,  and c) the efficiency function $\mathfrak{E()}$ describing the efficiency of the given kernel running on the device.
More specifically, $\mathfrak{E()}$ is a function of the concurrency exposed by the software $\mathbb{C}_{sw}$ and the concurrency required by the hardware $\mathbb{C}_{hw}$. The relation of measured performance to projected peak performance becomes:
\begin{equation}\footnotesize
   \mathbb{M}  =  \mathbb{P}\times \mathfrak{E(} \mathbb{C}_{sw},\mathbb{C}_{hw}\mathfrak{)}
    \label{eqt:basic}
\end{equation}
We discuss projected peak performance in the following section. A detailed discussion of the efficiency and concurrency functions is in Section~\ref{sec:apdperconcurrency}.


\subsection{Projecting Peak Achievable Performance}\label{sec:peakperform}
Details can be referred to Section~\ref{sec:howperksreduces}.
\begin{comment}

We rely on the FOM (Figure Of Merit) as the performance metric in this analysis. In stencils, we use the giga-cells updated per second (GCells/s)~\cite{DBLP:conf/cgo/MatsumuraZWEM20,chen2019versatile}. Given the memory-bound nature of the conjugate gradient solver, we directly use sustained memory bandwidth as a metric, following other works on conjugate gradient~\cite{anzt2020ginkgo}. Due to space limitations, this section mainly focuses on stencils to explain the performance analysis. Without loss of generality, the analysis is applicable to other cases (ex: conjugate gradients) by adjusting the performance metric and code concurrency accordingly.

We use a simple performance model inspired by the roofline model~\cite{ofenbeck2014applying,kim2011performance}. The model's utility is to project the upper bound on performance based on the reduction of global memory traffic. This model, in turn, helps us in this paper to identify performance gaps in our PERKS implementation and later inspect the reasons for those gaps (e.g., register spilling). 


In a kernel implemented as PERKS, the bottleneck could either be the global memory bandwidth or the shared memory bandwidth (if the PERKS caching scheme moves the bottleneck to become the shared memory bandwidth). We don't assume the registers to be a bottleneck since we assume that as long as we ensure that no register spilling occurs, we avoid register pressure.


We initially do not account for the memory accesses to global memory originating from the boundary threads in each thread block, e.g., halo region in stencil, and confine our analysis to the dependency in cached region. We then expand our analysis to consider those unavoidable global memory accesses (Equation~\ref{eqt:perkhalo}).

We assume a total domain of size $\mathbb{D}$ bytes, the cached portion to be $\mathbb{D}_{cache}$ bytes, and the uncached portion to be {\footnotesize$\mathbb{D}_{uncache}=\mathbb{D}-\mathbb{D}_{cache}$} bytes. The cached portion of the domain data would be divided between registers and shared memory (since we cache in both registers and shared memory): {\footnotesize$\mathbb{D}_{cache}=\mathbb{D}^{sm}_{cache}+\mathbb{D}^{reg}_{cache}$}. For $N$ time steps, assuming the number of bytes stored to global memory in each time step is $\mathbb{S}_{gm}$ and the number of bytes loaded is $\mathbb{L}_{gm}$, the total global memory bytes accessed $\mathbb{A}_{gm}$ becomes:
\begin{equation}\footnotesize
\begin{aligned}
    \mathbb{A}_{gm}(\mathbb{D})=N\cdot(\mathbb{L}_{gm}+\mathbb{S}_{gm})
    &=2\cdot N\cdot \mathbb{D}_{uncache} + 2\cdot  \mathbb{D}_{cache}    
\end{aligned}
\end{equation}


In the case when the kernel is bounded by global memory bandwidth, i.e., the volume of cached data does not move the bottleneck from global memory to shared memory, for the global memory bandwidth of $\mathbb{B}_{gm}$ and data type size of $\mathfrak{S}(type)$, the time $\mathbb{T}_{gm}(\mathbb{D})$ for accessing the global memory becomes:

\begin{equation}\footnotesize
    \begin{aligned}
                \mathbb{T}_{gm}(\mathbb{D})={{\mathbb{A}_{gm}(\mathbb{D})\cdot \mathfrak{S}(type)}}/{{\mathbb{B}_{gm}}}
    \end{aligned}
    \label{eqt:time_gm}
\end{equation}

In the case when the kernel is bounded by shared memory bandwidth, i.e., the volume of data cached in shared memory moves the bottleneck to be the shared memory bandwidth, the total shared memory (in bytes) accessed $\mathbb{A}_{sm}$ becomes: 

\begin{equation}\footnotesize
\begin{aligned}
    \mathbb{A}_{sm}(\mathbb{D}_{cache}^{sm})=N\cdot(\mathbb{L}_{sm}+\mathbb{S}_{sm})
    				=2\cdot (N-1)\cdot \mathbb{D}_{cache}^{sm}    				
\end{aligned}
\end{equation}


Assuming $\mathbb{A}_{sm}(\mathbb{KERNEL})$ to be the shared memory originally used by the kernel, e.g., shared memory used in the baseline implementation of a stencil kernel to improve the locality, and $\mathbb{B}_{sm}$ to be the shared memory bandwidth, the time $\mathbb{T}_{sm}(\mathbb{D})$ for accessing the shared memory becomes:

\begin{equation}\footnotesize
    \begin{aligned}
        \mathbb{T}_{sm}(\mathbb{D}_{cache}^{sm})=\{{{(\mathbb{A}_{sm}(\mathbb{D}_{cache}^{sm})+\mathbb{A}_{sm}(\mathbb{KERNEL}))\cdot \mathfrak{S}(type)}}\}/{{\mathbb{B}_{sm}}}
    \end{aligned}
    \label{eqt:time_sm}
\end{equation}


Next, we consider the unavoidable global memory accesses necessary to resolve the neighborhood dependencies in $\mathbb{D}_{cache}$, e.g., the halo region of stencils. In the cached portion of the domain, the halo region requires global memory accesses to resolve the dependencies. Assuming the global memory accesses, in bytes, for the halo region of the data computed by the boundary threads in thread blocks that are in the cached portion of the domain to be $\mathbb{A}_{gm}(\mathfrak{H}(\mathbb{D}_{cache}))$, the time for accessing those halo region $\mathbb{T}_{gm}(\mathfrak{H}(\mathbb{D}_{cache}))$ would be:

\begin{equation}\footnotesize
    \begin{aligned}
          \mathbb{T}_{gm}(\mathfrak{H}(\mathbb{D}_{cache}))={\mathbb{A}(\mathfrak{H}(\mathbb{D}_{cache}))\cdot \mathfrak{S}(type)}/{\mathbb{B}_{gm}}
    \end{aligned}
    \label{eqt:perkhalo}
\end{equation}
The projected best-case total time required for the PERKS kernel may be written as:

\begin{equation}\footnotesize
    \begin{aligned}
     \mathbb{T}_{PERKS}=\max(\mathbb{T}_{gm}(\mathbb{D})+\mathbb{T}_{gm}(\mathfrak{H}(\mathbb{D}_{cache})),\mathbb{T}_{{sm}})
    \end{aligned}
    \label{eqt:maxlat}
\end{equation}

Accordingly, the projected peak performance ($\mathbb{P}$ in Equation~\ref{eqt:basic}) for the $N$ time steps can be expressed as:

\begin{equation}\footnotesize
    \begin{aligned}
     \mathbb{P}={\mathbb{D} \cdot N}/{\mathbb{T}_{PERKS}}
    \end{aligned}
    \label{eqt:maxpeak}
\end{equation}


To further illustrate how this performance analysis works, we give two examples while computing $N=1000$ time-steps of a single precision 2D 5-point Jacobi stencil on A100. 

We use the domain size $\mathbb{D}=3072^2$ as an example of a large domain size; the total cache-able region is $\mathbb{D}_{cache}=3072\cdot2448$ leading to $\mathbb{T}_{gm}(\mathbb{D})=9900.70$ us. The total number of bytes for the halo accesses is $\mathbb{A}(\mathfrak{H}(\mathbb{D}_{cache}))=1000\cdot2\cdot 216\cdot(136\cdot2+256\cdot2)$. Thus $\mathbb{T}^{gm}(\mathfrak{H}(\mathbb{D}_{cache}))= 871.22$ us. So $\mathbb{P}_{PERKS}=3072^2\cdot 1000/\mathbb{T}_{PERKS}= 876.09$ GCells/s, 
the measured performance is $444.19$ GCells/s ($50.70\%$ of $\mathbb{P}$; in the following sections we elaborate on the analysis of concurrency and its impact on the gap between measured and projected peak).

We use the domain size $\mathbb{D}=3072\cdot2448$ as an example of small domain/ size, i.e.,  when the whole domain can be cached. In our baseline implementation used $\mathbb{A}_{sm}(\mathbb{KERNEL})=\mathbb{D}\cdot 1000 \cdot 4$ bytes of shared memory. The shared memory cached portion is $\mathbb{D}_{cache}=3072\cdot1152$, so $\mathbb{A}^{sm}(\mathbb{D}_{cache})=3072\cdot1152\cdot(999)\cdot2$. We get $\mathbb{T}_{sm}=7.6$ ms and $\mathbb{P}=\mathbb{D}\cdot 1000/\mathbb{T}_{PERKS}=986.38$ GCells/s, the measured performance is $609.30$ GCells/s (61.77\% of $\mathbb{P}$).
\end{comment}

\subsection{{Quality of the implementation}}

The roofline-like model we propose suffers from the same limitations of the roofline model, e.g., it has an implicit assumption of perfect overlap of compute and memory accesses. Additionally, inaccuracies can arise from the L2 concurrency issues we discussed in Section~\ref{sec:perconcurrency}. The projected peak performance is effective in serving the purposes of identifying unanticipated performance gaps and guiding our occupancy reduction. That being said, it is important to note that projected peak performance showed is taken as an indicator of the bound on performance improvement and not as accurate performance prediction. %In large-domain stencils, we observed $64\%$ ($36\%\sim85\%$) of the projected peak. In the small-domain stencils, we observe $59\%$ ($34\%\sim97\%$) of the projected peak. 

%The roofline-like model we proposed reveals the achievable performance. It can help us understand the implementation quality. 
In large-domain stencils, we achieved $64\%$ ($36\%\sim84\%$) of the projected peak. In the small-domain stencils, we achieved $59\%$ ($34\%\sim108\%$) of the projected peak. The $100+\%$ performance likely comes from L2 cache that we didn't include in the model.

\subsection{Concurrency and Micro-benchmarks}\label{sec:apdperconcurrency}
Reducing device occupancy increases the availability of resources to be used for caching in PERKS (as illustrated earlier in Figure~\ref{Fig:showcase}). On the contrary, reducing occupancy can lead to lower device utilization. To effectively implement PERKS, one has to reduce the occupancy as much as possible without scarifying performance. Inspired by the findings of Volkov~\cite{volkov2010better}, we assume that the efficiency function $\mathfrak{E}$ reaches its peak point when the code provides enough concurrency to saturate the device (irrespective of the occupancy):
\begin{equation}\footnotesize
    \mathfrak{E}(\mathbb{C}_{sw},\mathbb{C}_{hw})=100\%, \text{if } \forall \mathbb{C}_{sw}\geq \mathbb{C}_{hw}
    \label{eqt:efficiency}
\end{equation}

Where $\mathbb{C}_{sw}(\mathbb{OP})$ is the minimum number of concurrently executable instructions of the operation $\mathbb{OP}$ exposed by the launched kernel, and $\mathbb{C}_{hw}(\mathbb{OP})$ is the maximum numbers of instructions of the operation $\mathbb{OP}$ that the device is capable of handling concurrently. Because this paper mainly focuses on memory-bound applications, the $\mathbb{OP}$ referred to in this paper are limited to data access operations, i.e. global memory load/store $\mathbb{C}(\mathbb{GM})$, shared memory load/store $\mathbb{C}(\mathbb{SM})$, and L2 cache load/store $\mathbb{C}(\mathbb{L}2)$. 


\subsubsection{Measuring $\mathbb{C}_{sw}^{SMX}$} $\mathbb{C}_{sw}^{SMX}(\mathbb{OP})$, the kernel concurrency at the streaming multi-processor (SMX) level, can be computed based on the concurrency exposed by the threads of a thread block $\mathbb{C}_{sw}^{TB}(\mathbb{OP})$ and number of concurrently running thread blocks per stream multiprocessor {\footnotesize$TB/SMX$}:  {\footnotesize$\mathbb{C}_{sw}^{SMX}(\mathbb{OP})=\mathbb{C}_{sw}^{TB}(\mathbb{OP})\cdot TB/SMX$}.

 
\subsubsection{Measuring $\mathbb{C}_{hw}$} According to Little's Law~\cite{Little1961APF}, the hardware concurrency $\mathbb{C}_{hw}$ can be determined by the throughput $\mathbb{THR}$ and latency $\mathbb{L}$\cite{volkov2010better}: 
\begin{equation}\footnotesize
    \mathbb{C}_{hw}(\mathbb{OP})=\mathbb{THR(OP)} \cdot \mathbb{L(OP)}
\end{equation}

The throughput $\mathbb{THR}$ for different data access operations are available in Nvidia online documents~\cite{nvidia2019programming,amperewhite}. We measure the latency $\mathbb{L}$ with commonly used microbenchmarks~\cite{wong2010demystifying,mei2014benchmarking,zhang2017understanding}. Table~\ref{tab:concurrency} shows the detailed results in V100 and P100. We can further induce the minimal concurrency necessary for accessing global memory. The detailed results are displayed in Table~\ref{tab:lowoccupancy}.

\begin{comment}
	Latency of shared memory and L2 Cache can be tested with microbenchmark provided by previous research~\cite{wong2010demystifying,mei2014benchmarking}. But these works\cite{wong2010demystifying,mei2014benchmarking} test global memory latency with a metrics of cycle, which do not reflect its latency in second due to dynamic frequency. We thereby combine Mei etc.'s~\cite{mei2014benchmarking} microbenchmark Zhang etc's research~\cite{zhang2017understanding} to test $L_{global}$ with CPU clock. The alternative measurement is to manually set frequency to be static and use the existing microbenchmark and latency in cycle and deduce its latency in second from the frequency. However, we found that the latency varies as the frequency varies; the latency of some operation involved in global memory access can be affected by the GPU uncore frequency. The CPU measured global memory latency with default dynamic frequency setting is reported in this paper. $Thr$, $L$ and $C$ of memory in A100 and V100 is gathered in Table~\ref{tab:concurrencysm}, Table~\ref{tab:concurrencyl2} and Table ~\ref{tab:concurrencygm}. 
\end{comment}

% \begin{comment}
\begin{table}[t]
	\caption{Throughput and latency of relevant operations on A100 and V100 GPUs}
    \centering
	\begin{tabular}{|c|c|c|}
	\hline
	 & A100&V100\\\hline
	\multicolumn{3}{|c|}{ Shared memory}\\\hline
	$\mathbb{THR}(\mathbb{SM})(B/cycle) $&128&128\\
	$\mathbb{L}(\mathbb{SM})(cycle)$ &28&26\\
	$\mathbb{C}^{SMX}_{hw}(\mathbb{SM}) (B)$ &3584&3328\\\hline
	\multicolumn{3}{|c|}{Global memory}\\\hline
	$\mathbb{THR}(\mathbb{GM})(GB/s) $ & 1555   & 900\\
	$\mathbb{L}(\mathbb{GM})(ns)$      & 403.28 & 286.17\\
	 $\mathbb{C}_{hw}(\mathbb{GM})(B)$& 627101 & 257553\\
	$\mathbb{C}^{SMX}_{hw}(\mathbb{GM})(B)$  & 5807   & 3220\\\hline	
	
	\multicolumn{3}{|c|}{L2 Cache}\\\hline
	$\mathbb{THR}(\mathbb{L}2)(B/cycle) $ & 5120   & 2048\\
	$\mathbb{L}(\mathbb{L}2)(cycle)$      & 218/384 & 200\\
	$\mathbb{C}_{hw}(\mathbb{L}2)(B)$& 1541120 & 409600\\
	$\mathbb{C}^{SMX}_{hw}(\mathbb{L}2)(B)$ & 14270   & 5120\\\hline	
	\end{tabular}
	\label{tab:concurrency}
\end{table} 
% 
\begin{comment}
\begin{table}[t]
	\caption{Hardware concurrency of memory access for double precision values per stream multiprocessors (SMX) on P100, V100, and A100 GPUs}
% \scriptsize
    \centering
	\begin{tabular}{|c|c|c|}
	\hline
	&\textbf{V100}&\textbf{A100}\\\hline
% 	\multicolumn{4}{|c|}{\textbf{Global memory}}\\\hline
	\textbf{$\mathbb{THR}$/SMX(GB/s)}~\cite{amperewhite}        & 12       & 15 \\
	\textbf{$\mathbb{L}$ (ns)}                & 286       & 403 \\
	\textbf{$\mathbb{C}_{hw}$/SMX (B)}      & 3220      & 5807   \\
    % $\mathbb{C}^{SMX}_{hw}(Double)$ & 624   & 432       & 764   \\
  \textbf{ Min Occupancy($ILP=1$)}  \tablefootnote{Min Occupancy is deduced by assuming that only using TLP for parallelism, and assuming that thread block size is 128}                   & 25\%  & 37.5\%     \\\hline	
	\end{tabular}
	\label{tab:lowoccupancy}
% 	{\footnotesize * Min Occupancy is deduced by assuming that only using TLP for parallelism}
\end{table} 
\end{comment}
% 
\begin{table}[t]
	\caption{Hardware concurrency of memory access for double precision values per stream multiprocessors (SMX) on P100, V100, and A100 GPUs}
% \scriptsize
    \centering
	\begin{tabular}{|c|c|c|c|}
	\hline
	 & \textbf{P100}&\textbf{V100}&\textbf{A100}\\\hline
% 	\multicolumn{4}{|c|}{\textbf{Global memory}}\\\hline
	\textbf{$\mathbb{THR}$/SMX(GB/s)}~\cite{amperewhite}       & 13    & 12       & 15 \\
	\textbf{$\mathbb{L}$ (ns)}                & 384   & 286       & 403 \\
	\textbf{$\mathbb{C}_{hw}$/SMX (B)}      & 4992  & 3220      & 5807   \\
    % $\mathbb{C}^{SMX}_{hw}(Double)$ & 624   & 432       & 764   \\
  \textbf{ Min Occupancy($ILP=1$)}  \tablefootnote{Min Occupancy is deduced by assuming that only using TLP for parallelism, and assuming that thread block size is 128}                 & 31.25\%  & 25\%  & 37.5\%     \\\hline	
	\end{tabular}
	\label{tab:lowoccupancy}
% 	{\footnotesize * Min Occupancy is deduced by assuming that only using TLP for parallelism}
\end{table} 



\subsection{Concurrency Analysis}
\label{sec:apdconan}

In this section, we briefly describe how we analyze the concurrency to reduce the occupancy of the original kernel in order to release resources for caching while sustaining performance. We conduct a static analysis to extract the data movement operations in the kernel. Note that we account for any barriers in the original kernels that could impact the concurrency of operations, i.e., we do not combine operators/instructions from before and after the barrier when we count the operators. Finally, we apply efficient function $\mathfrak{E()}$ (Equation~\ref{eqt:efficiency}) to identify the least occupancy we could drop to before the concurrency starts to drop. 

For example, we did a static analysis of a single precision 2D 5-point Jacobi stencil kernel to conduct a concurrency analysis. It is worth mentioning that the baseline kernel we use is fairly complex since it is highly optimized by using shared memory to reduce traffic to global memory to its minimum~\cite{maruyama2014optimizing}. The results are summarized in Table~\ref{tab:concurrencyanalysis}. It shows that for this kernel, we could reduce the original occupancy to ${1/4}^{th}$ while maintaining performance.

To understand the gap between the projected upper-bound on achievable performance and the measured performance ($94.75/138.29=68.52\%$), we inspect the efficiency function $\mathfrak{E()}$. The results revealed that the concurrency for accesses in L2 cache, not global memory, is impacted by reducing occupancy on A100 in specific to the level that affects performance notably. More particularly, access to global memory for the halo region garners a high L2 cache hit rate. This effectively means that higher concurrency is necessary to saturate the L2 cache when hit rates are high. To confirm, we manually doubled the concurrency $\mathbb{C}^{TB}_{sw}$: the performance increased to 123.94 GCells/s with TB/SMX=1 (from $68.52\%$ up to $89.6\%$). 


\begin{table}[t]
    \centering
    \caption{Concurrency analysis of global memory accesses of a single precision 2D-5point Jacobi stencil kernel running on A100 (1000 time-steps on $3072^2$ domain)}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{?c?c|c|c|c|c?}
        \tbhline
            \multirow{2}{*}{$\tfrac{TB}{SMX}$}  & Used Reg. & Unused Reg. & GM Load & GM Store & Measured\\
              & /SMX  &/SMX    & op/SMX & op/SMX  & GCells/s\\\tbhline
            \textit{1} & 32KB  & 224KB  & 2580 & 2048 & 94.75\\
            \textit{2} & 64KB   & 192KB & 5160 & 4096 & 133.24\\
            \textit{8} & 256KB  & 0KB   & 20640 & 16384 & 138.29\\\tbhline
        \end{tabular}
    }
    \label{tab:concurrencyanalysis}
\end{table}




\subsection{Empirical Performance Model}\label{sec:empmodel}

Based on the performance analysis, we further deduce an empirical performance model for end-user. This model can help decide whether to apply PERKS without the knowledge of performance analysis. 

\textbf{Assumption:} PERKS does not change the efficiency of any implementations. If parallel parameters are equal to each other, $\mathfrak{E}_{PERKS}=\mathfrak{E}_{ori}$. According to Equation~\ref{eqt:basic}, we can deduce that:

\begin{equation}\footnotesize
    \mathbb{M}_{PERKS}=\mathbb{M}_{ori} \times \frac{\mathbb{P}_{PERKS}}{\mathbb{P}_{ori}}
    \label{eqt:projection}
\end{equation}

Additionally, in large domain/input size, assuming that the overhead of handling dependency is negligible, we can get:

\begin{equation}\footnotesize
\begin{aligned}
    \mathbb{M}_{PERKS}&=\mathbb{M}_{ori} \times \frac{1}{1-Per_{cache}}
\end{aligned}
\label{eqt:projectionLarge}
\end{equation}

For example, in 2D 5-point Jacobian stencil implementation, we set thread block=256. In baseline (SM-OPT), the default thread block per stream multiprocessor ($TB/SM$) is 8. Yet, after transforming the code to PERKS, the max $TB/SM$ is 2. We measured different $TB/SM$ settings for baseline and PERKS and put them in Table~\ref{tab:projection}. We also use Equation~\ref{eqt:projectionLarge} to project the performance based on the percentage of region cached and put the result in the same Table. 

\begin{table}[t]
    \centering\small
    \caption{Single precision $3702\times3702$ 2D 5-point Jacobian stencil in A100, performance of SM-OPT, PERKS and the performance projection}
    \begin{tabular}{|c|c|c|c|c|c|}
    \hline
        \multirow{2}{*}{$\tfrac{TB}{SM}$}  & SM-OPT & $Per_{cache}$ & Projection & PERKS&Accuracy\\
          & GCells/s && GCells/s & GCells/s&\\\hline
        1 & 94.87   & 77.34\%
        & 418.73& 357.79& 85.44\%\\
        2 & 133.41  & 79.69\% & 656.78& 444.55& 67.69\%\\ 
        8 & 137.65  & -       & - & -&-\\\hline
    \end{tabular}
    \label{tab:projection}
\end{table}

According to Table~\ref{tab:projection}, the Projection Model's accuracy is generally more than 67\%. So, this model can anticipate the potential speedup of applying PERKS without the knowledge of concurrency~\cite{volkov2010better}. 



==> Apendixes/x04_samplecodes.tex <==

\section{Source code of PERKS-based 3d7pt stencil}
The PERKS-based 3d 7-pt stencil kernel is presented in this section. 


\begin{lstlisting}[language=C,rulecolor=\color{black}, basicstyle=\tiny, caption=PERKS-based 3D 7-pt stencil with switch of source/ destination from/ to global memory/ shared memory/ register,captionpos=t]
template<class REAL, int halo, int LOCAL_ITEM_PER_THREAD, int BLOCKDIM, int LOCAL_TILE_X,int SM_SIZE_Z, int REG_SIZE_Z,
          int REG_CACHESIZE_Z=1,          
          bool loadfrmcache=false, bool storetocache=false,
          bool isloadfrmreg=false, bool isstoretoreg=false,
          int REGY_SIZE=REG_Y_SIZE_MOD, int REGX_SIZE=2*halo+1>
__device__ void __forceinline__ process_one_layer (REAL * __restrict__ input, REAL * __restrict__ output, 
        REAL* smbuffer_buffer_ptr[SM_SIZE_Z],REAL r_smbuffer[REG_SIZE_Z][LOCAL_ITEM_PER_THREAD],int global_z, int p_y, int p_x,int width_z, int width_y, int width_x,int ps_y, int ps_x, int sm_width_x,int cpbase_y, int cpend_y, int index_y,int tid_x, int tid_y,stencilParaList,REAL* sm_space=NULL, int frmcachesmid_z=0, int tocachesmid_z=0,REAL  r_space[REG_CACHESIZE_Z][LOCAL_ITEM_PER_THREAD]=NULL, int frmcacheregid_z=0, int tocacheregid_z=0,REAL* boundary_buffer=NULL, int boundary_buffer_index_z=0, const int boundary_east_step=0, const int boundary_west_step=0,const int boundary_north_step=0, const int boundary_south_step=0,const int boundary_step_yz=0)
{
  #define LOCAL_TILE_Y (LOCAL_ITEM_PER_THREAD*BLOCKDIM/LOCAL_TILE_X)
  #define gdim_y (BLOCKDIM/LOCAL_TILE_X)

  if(!loadfrmcache)
  {
    global2sm<REAL, halo, halo, 1, halo+1+isBOX, halo+isBOX, LOCAL_ITEM_PER_THREAD, gdim_y, false, true>(input, smbuffer_buffer_ptr,   p_x, p_y, global_z, width_x, width_y, width_z,  sm_width_x, ps_x, ps_y, LOCAL_TILE_X,tid_x,tid_y);
  }
  else
  {
    _Pragma("unroll")
    for(int l_y=0; l_y<LOCAL_ITEM_PER_THREAD; l_y++)
    {
      int local_y=l_y+LOCAL_ITEM_PER_THREAD*tid_y;

      if(!isloadfrmreg)
      {
        smbuffer_buffer_ptr[halo+isBOX][(local_y+ps_y)*sm_width_x+ps_x+tid_x] = sm_space[frmcachesmid_z*LOCAL_TILE_X*LOCAL_TILE_Y+(local_y-0)*LOCAL_TILE_X+tid_x];
      }
      else
      {
        smbuffer_buffer_ptr[halo+isBOX][(local_y+ps_y)*sm_width_x+ps_x+tid_x] = r_space[frmcacheregid_z][l_y];
      }
    }
    // middle frm sm or reg. halo need special care
    for(int l_y=tid_x-isBOX; l_y<LOCAL_TILE_Y+isBOX; l_y+=LOCAL_TILE_X)
    {
      #pragma unroll
      for(int l_x=tid_y; l_x<halo; l_x+=LOCAL_TILE_Y/LOCAL_ITEM_PER_THREAD)
      {
        //east
        smbuffer_buffer_ptr[halo+isBOX][(l_y+0+ps_y)*sm_width_x+ps_x+l_x+LOCAL_TILE_X] = boundary_buffer[boundary_east_step + (boundary_buffer_index_z) * (LOCAL_TILE_Y+2*isBOX)*halo  + (l_y+isBOX) + l_x * (LOCAL_TILE_Y+2*isBOX)];
        //west
        smbuffer_buffer_ptr[halo+isBOX][(l_y+0+ps_y)*sm_width_x+ps_x-halo+l_x]  = boundary_buffer[boundary_west_step + (boundary_buffer_index_z) * (LOCAL_TILE_Y+2*isBOX)*halo  + (l_y+isBOX) + l_x * (LOCAL_TILE_Y+2*isBOX)];
      }
    }
    //north south
    {
      int l_x=tid_x;
      #pragma unroll
      for(int l_y=tid_y; l_y<halo; l_y+=BLOCKDIM/LOCAL_TILE_X)
      {
        //north
        smbuffer_buffer_ptr[halo+isBOX][(l_y+LOCAL_TILE_Y+ps_y)*sm_width_x+ps_x+l_x] = boundary_buffer[boundary_north_step + (boundary_buffer_index_z) * (LOCAL_TILE_X)*halo  + (l_x) + l_y * (LOCAL_TILE_X)];
        
        //south
        smbuffer_buffer_ptr[halo+isBOX][(l_y-halo+ps_y)*sm_width_x+ps_x+l_x]  = boundary_buffer[boundary_south_step + (boundary_buffer_index_z) * (LOCAL_TILE_X)*halo  + (l_x) + l_y * (LOCAL_TILE_X)];
      }
    }
    __syncthreads();
  }

  //sm2reg
  sm2regs<REAL, LOCAL_ITEM_PER_THREAD, 1+2*halo, 1+halo, halo, 0, halo*2,  LOCAL_ITEM_PER_THREAD, 1>(smbuffer_buffer_ptr, r_smbuffer, ps_y+index_y, ps_x,  sm_width_x, tid_x);

  REAL sum[LOCAL_ITEM_PER_THREAD];
  _Pragma("unroll")
  for(int l_y=0; l_y<LOCAL_ITEM_PER_THREAD; l_y++)
  {
    sum[l_y]=0;
  }
  //main computation
  computation<REAL,LOCAL_ITEM_PER_THREAD,halo,REG_Y_SIZE_MOD>( sum,  smbuffer_buffer_ptr, ps_y+index_y,  sm_width_x, tid_x+ps_x,  r_smbuffer, stencilParaInput);

  __syncthreads();
  if(!storetocache)
  {
    reg2global3d<REAL, LOCAL_ITEM_PER_THREAD>(sum, output, global_z, width_z,p_y+index_y, width_y, p_x, width_x,  tid_x);
  }  
  else
  { 
    if(!isstoretoreg)
    {
      int z_ind=(tocachesmid_z)*LOCAL_TILE_X*LOCAL_TILE_Y;
      _Pragma("unroll")
      for(int l_y=0; l_y<LOCAL_ITEM_PER_THREAD; l_y++)
      {
        int local_y=l_y+index_y;
        sm_space[z_ind+(local_y-0)*LOCAL_TILE_X+tid_x]  = sum[l_y];
      }
    }
    else
    {
      _Pragma("unroll")
      for(int l_y=0; l_y<LOCAL_ITEM_PER_THREAD; l_y++)
      {
        r_space[tocacheregid_z][l_y]=sum[l_y];
      }
    }
  }
  REAL* tmp = smbuffer_buffer_ptr[0];
  // smswap 
  _Pragma("unroll")
  for(int hl=1; hl<halo+1+isBOX; hl++)
  {
    smbuffer_buffer_ptr[hl-1]=smbuffer_buffer_ptr[hl];
  }
  smbuffer_buffer_ptr[halo+isBOX]=tmp;
  regsself3d<REAL,REG_SIZE_Z,LOCAL_ITEM_PER_THREAD>(r_smbuffer);

  #undef LOCAL_TILE_Y
  #undef gdim_y
}
\end{lstlisting}
\begin{lstlisting}[language=C,rulecolor=\color{black}, basicstyle=\tiny, caption=3D 7-pt stencil computation function,captionpos=t]
#define stencilParaT const REAL center=-1.67f;const REAL west[1]={0.162f};const REAL east[1]={0.161f}; const REAL north[1]={0.163f}; const REAL south[1]={0.164f}; const REAL bottom[1]={0.166f}; const REAL top[1]={0.165f};
template<class REAL, int RESULT_SIZE, int halo, int REGY_SIZE,  int REGZ_SIZE=2*halo+1, int REGX_SIZE=2*halo+1, int REG_BASE=halo, int SMZ_SIZE=halo+1+halo>
#define isBOX (0)
#define stencilParaList const REAL west[HALO],const REAL east[HALO],const REAL north[HALO],const REAL south[HALO],const REAL top[HALO], const REAL bottom[HALO], const REAL center
#define stencilParaInput  west,east,north,south,top,bottom,center
#define REG_Y_SIZE_MOD (LOCAL_ITEM_PER_THREAD)
__device__ void __forceinline__ computation(REAL result[RESULT_SIZE],REAL* sm_ptr[SMZ_SIZE], int sm_y_base, int sm_width, int sm_x_ind,REAL reg_ptr[REGZ_SIZE][RESULT_SIZE], stencilParaList)
{
    _Pragma("unroll")
    for(int l_y=0; l_y<RESULT_SIZE; l_y++)
    {
      _Pragma("unroll")
      for(int hl=0; hl<halo; hl++)
      {
        result[l_y]+=west[hl]*
              sm_ptr[0][sm_width*(l_y+sm_y_base) + sm_x_ind-1-hl];
        result[l_y]+=east[hl]*
          sm_ptr[0][sm_width*(l_y+sm_y_base) + sm_x_ind+1+hl];
        result[l_y]+=north[hl]*
          sm_ptr[0][sm_width*(l_y+sm_y_base+1+hl) + sm_x_ind];
        result[l_y]+=south[hl]*
          sm_ptr[0][sm_width*(l_y+sm_y_base-1-hl) + sm_x_ind];
        result[l_y]+=bottom[hl]*reg_ptr[REG_BASE-1-hl][l_y];
        result[l_y]+=top[hl]*reg_ptr[REG_BASE+1+hl][l_y];
      }
    }
    _Pragma("unroll")
    for(int l_y=0; l_y<RESULT_SIZE; l_y++)
    {
        result[l_y]+=center*reg_ptr[REG_BASE][l_y];
    }
}
\end{lstlisting}


\begin{lstlisting}[language=C,rulecolor=\color{black}, basicstyle=\tiny, caption=supplimentary function,captionpos=t]
template<class REAL, int halo, bool isInit=false, bool sync=true>
__device__ void __forceinline__ global2sm(REAL* src, REAL* sm_buffer, 
                                              int size, 
                                              int global_y_base, int global_y_size,
                                              int global_x_base, int global_x_size,
                                              int sm_y_base, int sm_x_base, int sm_width,
                                              int tid)
{
  //fill shared memory buffer
  _Pragma("unroll")
  for(int l_y=0; l_y<size; l_y++)
  {
    int l_global_y;
    if(isInit)
    {
      l_global_y=(MAX(global_y_base+l_y,0));
    }
    else
    {
      l_global_y=(MIN(global_y_base+l_y,global_y_size-1));
      l_global_y=(MAX(l_global_y,0));
    }
    #define  dst_ind (l_y+sm_y_base)*sm_width
      sm_buffer[dst_ind-halo+tid+sm_x_base]=src[l_global_y * global_x_size + MAX(global_x_base-halo+tid,0)];
      if(halo>0)
      {
        if(tid<halo*2)
        {  
          sm_buffer[dst_ind-halo+tid+blockDim.x+sm_x_base]=src[(l_global_y) * global_x_size + MIN(-halo+tid+blockDim.x+global_x_base, global_x_size-1)];
        }
      }

  }
  if(sync==true)
  {  
    __syncthreads();
  }
  #undef dst_ind
}
template<class REAL, int halo, int BASE_Z, int SIZE_Z, int SMSIZE, int SM_BASE_Z=BASE_Z,  int LOCAL_ITEM_PER_THREAD, int gdim_y, bool isInit=false, bool sync=true>
__device__ void __forceinline__ global2sm(REAL *src, REAL* smbuffer_buffer_ptr[SMSIZE],
                                          int gbase_x, int gbase_y, int gbase_z,
                                          int width_x, int width_y, int width_z,
                                          int sm_width_x, int sm_base_x,
                                          int sm_base_y,
                                          int tile_x, int tid_x, int tid_y)
{
  _Pragma("unroll")
  for(int l_z=0; l_z<SIZE_Z; l_z++)
  {
    int l_global_z;
    if(!isInit)
    {
        l_global_z = (MIN(gbase_z+l_z+BASE_Z,width_z-1));
    }
    else
    {
       l_global_z = (MAX(gbase_z+l_z+BASE_Z,0));
    }
    #pragma unroll
    for(int i=0; i<LOCAL_ITEM_PER_THREAD; i++)
    {
      int l_y=i+tid_y*LOCAL_ITEM_PER_THREAD-halo;
      int l_global_y = (MIN(gbase_y+l_y,width_y-1));
        l_global_y = (MAX(l_global_y,0));
        smbuffer_buffer_ptr[l_z+SM_BASE_Z][sm_width_x*(l_y+sm_base_y) + (tid_x-halo) + sm_base_x]=
            src[l_global_z*width_x*width_y+l_global_y*width_x+
            MAX((gbase_x+tid_x-halo),0)];
      if(tid_x<halo*2)
      {
          smbuffer_buffer_ptr[l_z+SM_BASE_Z][sm_width_x*(l_y+sm_base_y) + tid_x + tile_x-halo+sm_base_x]=
              src[l_global_z*width_x*width_y+l_global_y*width_x+
                MIN(gbase_x+tid_x-halo+tile_x,width_x-1)];
      }
    }
    if(gdim_y>=2*halo)
    {
      {
        if(tid_y<2*halo)
        {
          int l_y=tid_y+gdim_y*LOCAL_ITEM_PER_THREAD-halo;
          int l_global_y = (MIN(gbase_y+l_y,width_y-1));
            l_global_y = (MAX(l_global_y,0));
            smbuffer_buffer_ptr[l_z+SM_BASE_Z][sm_width_x*(l_y+sm_base_y) + (tid_x-halo) + sm_base_x]=
                src[l_global_z*width_x*width_y+l_global_y*width_x+
                MAX((gbase_x+tid_x-halo),0)];
          if(tid_x<halo*2)
          {
              smbuffer_buffer_ptr[l_z+SM_BASE_Z][sm_width_x*(l_y+sm_base_y) + tid_x + tile_x-halo+sm_base_x]=
                  src[l_global_z*width_x*width_y+l_global_y*width_x+
                    MIN(gbase_x+tid_x-halo+tile_x,width_x-1)];
          }
        }
      }
    }
    else if(gdim_y>=2)
    {
      if(tid_y<2)
      {
        #pragma unroll
        for(int i=0; i<halo; i++)
        {
          int l_y=i+2*tid_y+gdim_y*LOCAL_ITEM_PER_THREAD-halo;
          int l_global_y = (MIN(gbase_y+l_y,width_y-1));
            l_global_y = (MAX(l_global_y,0));
            smbuffer_buffer_ptr[l_z+SM_BASE_Z][sm_width_x*(l_y+sm_base_y) + (tid_x-halo) + sm_base_x]=
                src[l_global_z*width_x*width_y+l_global_y*width_x+
                MAX((gbase_x+tid_x-halo),0)];
          if(tid_x<halo*2)
          {
              smbuffer_buffer_ptr[l_z+SM_BASE_Z][sm_width_x*(l_y+sm_base_y) + tid_x + tile_x-halo+sm_base_x]=
                  src[l_global_z*width_x*width_y+l_global_y*width_x+
                    MIN(gbase_x+tid_x-halo+tile_x,width_x-1)];
          }
        }
      }
    }
    else
    {
      if(tid_y==0)
      {
        #pragma unroll
        for(int i=0; i<2*halo; i++)
        {
          int l_y=i+gdim_y*LOCAL_ITEM_PER_THREAD-halo;
          int l_global_y = (MIN(gbase_y+l_y,width_y-1));
            l_global_y = (MAX(l_global_y,0));
            smbuffer_buffer_ptr[l_z+SM_BASE_Z][sm_width_x*(l_y+sm_base_y) + (tid_x-halo) + sm_base_x]=
                src[l_global_z*width_x*width_y+l_global_y*width_x+
                MAX((gbase_x+tid_x-halo),0)];
          if(tid_x<halo*2)
          {
              smbuffer_buffer_ptr[l_z+SM_BASE_Z][sm_width_x*(l_y+sm_base_y) + tid_x + tile_x-halo+sm_base_x]=
                  src[l_global_z*width_x*width_y+l_global_y*width_x+
                    MIN(gbase_x+tid_x-halo+tile_x,width_x-1)];
          }
        }
      }
    }
  }
  if(sync)
  {
    __syncthreads();
  }
}

template<class REAL,int REG_SIZE_Z, int REG_SIZE_Y, 
                        int BASE_Z=0,  int BASE_Y=0, 
                        int SIZE_Z=REG_SIZE_Z, int SIZE_Y=REG_SIZE_Y>
__device__ void __forceinline__ global2regs3d(
  REAL*src, REAL reg_array[REG_SIZE_Z][REG_SIZE_Y],
  int global_z, int width_z,
  int global_y, int width_y,
  int global_x, int width_x,
  int tid_x)
{
  _Pragma("unroll")
  for(int l_y=0; l_y<SIZE_Y; l_y++)
  {
    int l_global_y = (MIN(global_y+l_y+BASE_Y,width_y-1));
    l_global_y = (MAX(l_global_y,0));
    _Pragma("unroll")
    for(int l_z=0; l_z<SIZE_Z ; l_z++)
    {
      int l_global_z = (MIN(global_z+l_z+BASE_Z,width_z-1));
        l_global_z = (MAX(l_global_z,0));
      reg_array[l_z+BASE_Z][l_y+BASE_Y] = src[l_global_z*width_x*width_y+l_global_y*width_x+
            ((global_x+tid_x))];
    }
  }
}
template<class REAL, int SIZE_Z, int SIZE_Y>
__device__ void __forceinline__ regsself3d(
  REAL reg_array[SIZE_Z][SIZE_Y])
{
  _Pragma("unroll")
  for(int l_y=0; l_y<SIZE_Y; l_y++)
  {
    _Pragma("unroll")
    for(int l_z=0; l_z<SIZE_Z ; l_z++)
    { 
      reg_array[l_z][l_y] = reg_array[l_z+1][l_y];
    }
  }
}
template<class REAL, int SIZE_REG, int SIZE=SIZE_REG, int REG_BASE=0>
__device__ void __forceinline__ reg2global3d(
            REAL reg_array[SIZE_REG], REAL*dst,
            int global_z, int width_z,
            int global_y, int width_y,
            int global_x, int width_x,
            int tid_x)
{
  _Pragma("unroll")
  for(int l_y=0; l_y<SIZE; l_y++)
  {
    dst[global_z*width_x*width_y+(global_y+l_y)*width_x+global_x+tid_x]=reg_array[l_y+REG_BASE];
  }
}


\end{lstlisting}
\begin{lstlisting}[language=C,rulecolor=\color{black}, basicstyle=\tiny, caption=PERKS-based full 3D 7-pt stencil kernel including halo region management,captionpos=t]
#define HALO (1)
#define NOCACHE_Z (HALO)
template<class REAL, int halo, 
int LOCAL_ITEM_PER_THREAD, int LOCAL_TILE_X, const int reg_folder_z, bool UseSMCache, int BLOCKDIM=256>
__device__ __forceinline__ void kernel3d_general_inner(REAL * __restrict__ input, REAL * __restrict__ output, int width_z, int width_y, int width_x,REAL* l2_cache_i, REAL* l2_cache_o,  int iteration, int max_sm_flder) 
{
  #define LOCAL_TILE_Y (LOCAL_ITEM_PER_THREAD*BLOCKDIM/LOCAL_TILE_X)
  #define gdim_y (BLOCKDIM/LOCAL_TILE_X)  
  if(!UseSMCache) max_sm_flder=0;
  #define UseRegCache (reg_folder_z!=0)
  const int tile_x_with_halo=LOCAL_TILE_X+2*halo;
  const int tile_y_with_halo=LOCAL_TILE_Y+2*halo;
  stencilParaT;
  extern __shared__ char sm[];
  REAL* sm_rbuffer = (REAL*)sm+1;
  REAL* smbuffer_buffer_ptr[halo+1+isBOX];
  smbuffer_buffer_ptr[0]=sm_rbuffer;
  #pragma unroll
  for(int hl=1; hl<halo+1+isBOX; hl++)
  {
    smbuffer_buffer_ptr[hl]=smbuffer_buffer_ptr[hl-1]+tile_x_with_halo*tile_y_with_halo;
  }
  REAL* sm_space = sm_rbuffer+tile_x_with_halo*tile_y_with_halo*(halo+1+isBOX);
  REAL* boundary_buffer=sm_space+max_sm_flder*LOCAL_TILE_X*(LOCAL_TILE_Y);
  register REAL r_smbuffer[2*halo+1][REG_Y_SIZE_MOD];
  register REAL r_space[reg_folder_z<=0?1:reg_folder_z][LOCAL_ITEM_PER_THREAD];
  /***********************/
  const int tid_x = threadIdx.x%LOCAL_TILE_X;
  const int tid_y = threadIdx.x/LOCAL_TILE_X;
  const int dim_y = LOCAL_TILE_Y/LOCAL_ITEM_PER_THREAD;
  const int cpblocksize_y=(tile_y_with_halo)/dim_y;
  const int cpquotion_y=(tile_y_with_halo)%dim_y;
  const int index_y = LOCAL_ITEM_PER_THREAD*tid_y;
  const int cpbase_y = -halo+tid_y*cpblocksize_y+(tid_y<=cpquotion_y?tid_y:cpquotion_y);
  const int cpend_y = cpbase_y + cpblocksize_y + (tid_y<=cpquotion_y?1:0);
  const int ps_y = halo;
  const int ps_x = halo;
  const int p_x = blockIdx.x * LOCAL_TILE_X;
  const int p_y = blockIdx.y * LOCAL_TILE_Y;
  int blocksize_z=(width_z/gridDim.z);
  int z_quotient = width_z%gridDim.z;
  const int p_z =  blockIdx.z * (blocksize_z) + (blockIdx.z<=z_quotient?blockIdx.z:z_quotient);
  blocksize_z += (blockIdx.z<z_quotient?1:0);
  const int p_z_reg_start=p_z+NOCACHE_Z;
  const int p_z_sm_start=p_z+NOCACHE_Z + reg_folder_z;
  const int p_z_sm_end=p_z_sm_start+max_sm_flder;
  const int p_z_end = p_z + (blocksize_z);
  const int total_folder_z=max_sm_flder+reg_folder_z;
  const int boundary_east_step=0;
  const int boundary_west_step=(LOCAL_TILE_Y+isBOX*2)*(total_folder_z)*halo;
  const int boundary_north_step=boundary_west_step+(LOCAL_TILE_Y+isBOX*2)*(total_folder_z)*halo;
  const int boundary_south_step=boundary_north_step+TILE_X*total_folder_z*halo;
  const int l2_boundary_east_step=0;
  const int l2_boundary_west_step=width_y*halo*gridDim.x*total_folder_z*gridDim.z;
  const int l2_boundary_north_step=l2_boundary_west_step+width_y*halo*gridDim.x*total_folder_z*gridDim.z;
  const int l2_boundary_south_step=l2_boundary_north_step+width_x*halo*gridDim.y*total_folder_z*gridDim.z; 
  const int boundary_step_yz=(LOCAL_TILE_Y+isBOX*2)*total_folder_z;
  _Pragma("unroll")
  for(int cache_z=0; cache_z<reg_folder_z; cache_z++)
  {
    for(int l_y=0; l_y<LOCAL_ITEM_PER_THREAD; l_y++)
    {
      int local_y=l_y+LOCAL_ITEM_PER_THREAD*tid_y;
      r_space[cache_z][l_y]
        = input[(p_z_reg_start + cache_z)*width_x*width_y+(local_y+p_y)*width_x+p_x+tid_x];
    }
  }
  // global 2 sm cache
  for(int cache_z=0; cache_z<max_sm_flder; cache_z++)
  {
    for(int l_y=0; l_y<LOCAL_ITEM_PER_THREAD; l_y++)
    {
      int local_y=l_y+LOCAL_ITEM_PER_THREAD*tid_y;
      sm_space[cache_z*LOCAL_TILE_X*LOCAL_TILE_Y+local_y*LOCAL_TILE_X+tid_x]
        = input[(p_z_sm_start + cache_z)*width_x*width_y+(local_y+p_y)*width_x+p_x+tid_x];
    }
  }
  // boundary
  for(int cache_z=0; cache_z<max_sm_flder+reg_folder_z; cache_z++)
  {
    for(int l_y=threadIdx.x-isBOX; l_y<LOCAL_TILE_Y+isBOX; l_y+=blockDim.x)
    {
      int global_y=MIN(p_y+l_y,width_y-1);
      global_y=MAX(0,global_y);
      #pragma unroll
      for(int l_x=0; l_x<halo; l_x++)
      {
        //east
        int global_x = p_x+LOCAL_TILE_X+l_x;
        global_x = MIN(width_x-1,global_x);
        boundary_buffer[boundary_east_step + cache_z *  (LOCAL_TILE_Y+2*isBOX)*halo + (l_y+isBOX) + l_x * (LOCAL_TILE_Y+2*isBOX)] = input[(p_z+NOCACHE_Z+cache_z)*width_x*width_y+(global_y)*width_x+global_x];
        // //west
        global_x = p_x-halo+l_x;
        global_x = MAX(0,global_x);
        boundary_buffer[boundary_west_step + cache_z *  (LOCAL_TILE_Y+2*isBOX)*halo + (l_y+isBOX) + l_x *  (LOCAL_TILE_Y+2*isBOX)] = input[(p_z+NOCACHE_Z+cache_z)*width_x*width_y+(global_y)*width_x+global_x];
      }
    }
    for(int l_x=threadIdx.x; l_x<TILE_X; l_x+=blockDim.x)
    {
      int global_x = p_x+l_x;
      #pragma unroll
      for(int l_y=0; l_y<halo; l_y++)
      {
        //north
        int global_y = p_y + LOCAL_TILE_Y + l_y;
        global_y=MIN(global_y,width_y-1);
        boundary_buffer[boundary_north_step + cache_z * LOCAL_TILE_X * halo + (l_x) + l_y * LOCAL_TILE_X]= input[(p_z+NOCACHE_Z+cache_z)*width_x*width_y+(global_y)*width_x+global_x];
        //south
        global_y = p_y - halo + l_y;
        global_y=MAX(global_y,0);
        boundary_buffer[boundary_south_step + cache_z * LOCAL_TILE_X * halo + (l_x) + l_y * LOCAL_TILE_X]= input[(p_z+NOCACHE_Z+cache_z)*width_x*width_y+(global_y)*width_x+global_x];
      }
    }
  }
  // int smz_ind=0;
  cg::grid_group gg = cg::this_grid();
  for(int iter=0; iter<iteration; iter++)
  {
    // halo in(global, 0,halo)
    global2regs3d<REAL, 1+2*halo, LOCAL_ITEM_PER_THREAD>
      (input, r_smbuffer, p_z-halo,width_z, p_y+index_y, width_y, p_x, width_x,tid_x);
    global2sm<REAL, halo, -isBOX, halo + isBOX, halo+isBOX+1, 0, true, false> (input, smbuffer_buffer_ptr, p_x, p_y, p_z, width_x, width_y, width_z,tile_x_with_halo, ps_x,cpbase_y, cpend_y, 1,ps_y,LOCAL_TILE_X, tid_x);
    // // // reg->global
    if(UseRegCache)
    {
      _Pragma("unroll")
      for(int global_z=p_z, cache_z_reg=0; global_z<p_z_reg_start; global_z+=1, cache_z_reg++)
      {
        process_one_layer<REAL, halo, LOCAL_ITEM_PER_THREAD, BLOCKDIM, LOCAL_TILE_X, halo+1+isBOX, 2*halo+1,reg_folder_z==0?1:reg_folder_z, true,false, true, false>(input, output, smbuffer_buffer_ptr, r_smbuffer, global_z,  p_y,  p_x, width_z,  width_y,  width_x, ps_y, ps_x, tile_x_with_halo,cpbase_y, cpend_y, index_y,tid_x, tid_y, stencilParaInput,sm_space, 0, 0,r_space, cache_z_reg, 0,boundary_buffer, cache_z_reg, boundary_east_step, boundary_west_step, boundary_north_step, boundary_south_step,boundary_step_yz
        );
      }    
      // // reg->reg                    
      _Pragma("unroll")   
      for(int global_z=p_z_reg_start,cache_z_reg=halo; global_z<p_z_sm_start-halo; global_z+=1,cache_z_reg++)
      {
        process_one_layer<REAL, halo, LOCAL_ITEM_PER_THREAD, BLOCKDIM, LOCAL_TILE_X, halo+1+isBOX, 2*halo+1,reg_folder_z==0?1:reg_folder_z, true,true,true, true> (input, output, smbuffer_buffer_ptr,  r_smbuffer,global_z,  p_y,  p_x,width_z,  width_y,  width_x,ps_y, ps_x, tile_x_with_halo, cpbase_y, cpend_y, index_y,   tid_x, tid_y,stencilParaInput,sm_space, 0, 0,r_space, cache_z_reg,cache_z_reg-halo,boundary_buffer, cache_z_reg, boundary_east_step, boundary_west_step,boundary_north_step,boundary_south_step,boundary_step_yz );
      }
    }
    if((UseRegCache)&&UseSMCache)
    {
      _Pragma("unroll")
      for(int global_z=p_z_sm_start-halo, cache_z=0; global_z<p_z_sm_start; global_z+=1, cache_z++)
      {
        process_one_layer<REAL, halo, LOCAL_ITEM_PER_THREAD, BLOCKDIM, LOCAL_TILE_X, halo+1+isBOX, 2*halo+1,reg_folder_z==0?1:reg_folder_z, true,true,false, true>(input, output,  smbuffer_buffer_ptr, r_smbuffer, global_z,  p_y,  p_x,width_z,  width_y,  width_x,ps_y, ps_x, tile_x_with_halo,cpbase_y, cpend_y, index_y,tid_x, tid_y, stencilParaInput, sm_space, cache_z, 0, r_space, 0, cache_z+reg_folder_z-halo, boundary_buffer, cache_z+reg_folder_z,  boundary_east_step, boundary_west_step, boundary_north_step, boundary_south_step, boundary_step_yz );
      }
    }
    
    if((UseRegCache)&&!UseSMCache)
    {
       // // global -> (reg)
      _Pragma("unroll")
      for(int global_z=p_z_sm_start-halo, cache_z=0, cache_z_reg=reg_folder_z; global_z<p_z_sm_start; global_z+=1, cache_z++,cache_z_reg++)
      {
        process_one_layer<REAL, halo, LOCAL_ITEM_PER_THREAD, BLOCKDIM, LOCAL_TILE_X, halo+1+isBOX, 2*halo+1, reg_folder_z==0?1:reg_folder_z, false,true,false, true>(input, output,  smbuffer_buffer_ptr,  r_smbuffer,global_z,  p_y,  p_x, width_z,  width_y,  width_x,ps_y, ps_x, tile_x_with_halo, cpbase_y, cpend_y, index_y, tid_x, tid_y, stencilParaInput, sm_space, 0, 0,  r_space, 0, cache_z_reg-halo, boundary_buffer, cache_z+reg_folder_z,   boundary_east_step,boundary_west_step, boundary_north_step, boundary_south_step, boundary_step_yz
        );
      }
    }
    //register  boundary 
    //east and west 
    _Pragma("unroll")
    for(int l_z=0; l_z<reg_folder_z; l_z++)
    {
      if(tid_x>=LOCAL_TILE_X-halo)
      {
        int l_x=tid_x-LOCAL_TILE_X+halo;
        for(int l_y=0; l_y<LOCAL_ITEM_PER_THREAD;l_y+=1)
        {
          int local_y=l_y+LOCAL_ITEM_PER_THREAD*tid_y;
          //east
          boundary_buffer[boundary_east_step + (l_z) *  (LOCAL_TILE_Y+2*isBOX)*halo + (local_y+isBOX) + l_x * (LOCAL_TILE_Y+2*isBOX)]=r_space[l_z][l_y];
        }
      }
      if(tid_x<halo)
      {
        int l_x=tid_x;
        for(int l_y=0; l_y<LOCAL_ITEM_PER_THREAD;l_y+=1)
        {
          int local_y=l_y+LOCAL_ITEM_PER_THREAD*tid_y;
          //west
          boundary_buffer[boundary_west_step + (l_z) *  (LOCAL_TILE_Y+2*isBOX)*halo + (local_y+isBOX) + l_x * (LOCAL_TILE_Y+2*isBOX)]=r_space[l_z][l_y];
        }
      }
    }
    //north and south
    _Pragma("unroll")
    for(int l_z=0; l_z<reg_folder_z; l_z++)
    {
      
      int l_x=tid_x;
      #pragma unroll
      for(int l_y=0; l_y<halo; l_y++)
      {
        //south
        if(tid_y==0)
        {
          boundary_buffer[boundary_south_step + (l_z) *  (LOCAL_TILE_X)*halo + (l_x) + l_y * (LOCAL_TILE_X)] = r_space[l_z][l_y];
        }
        //north
        if(tid_y==dim_y-1)
        {
          boundary_buffer[boundary_north_step + (l_z) *  (LOCAL_TILE_X)*halo + (l_x) + (l_y) * (LOCAL_TILE_X)] = r_space[l_z][LOCAL_ITEM_PER_THREAD-halo+ l_y];
        } 
      }
    }
    //no need sync
    if(!UseRegCache&&UseSMCache)
    {
      // sm -> global
      _Pragma("unroll")
      for(int global_z=p_z_sm_start-halo, cache_z=0, cache_z_reg=reg_folder_z; global_z<p_z_sm_start; global_z+=1, cache_z++,cache_z_reg++)
      {
        process_one_layer<REAL, halo, LOCAL_ITEM_PER_THREAD, BLOCKDIM, LOCAL_TILE_X, halo+1+isBOX, 2*halo+1, reg_folder_z==0?1:reg_folder_z,true, false, false, false>(input, output,  smbuffer_buffer_ptr,  r_smbuffer, global_z,  p_y,  p_x,  width_z,  width_y,  width_x,ps_y, ps_x, tile_x_with_halo,cpbase_y, cpend_y, index_y, tid_x, tid_y, stencilParaInput, sm_space, cache_z, 0, r_space, 0, cache_z_reg-halo, boundary_buffer, cache_z+reg_folder_z, boundary_east_step, boundary_west_step, boundary_north_step, boundary_south_step, boundary_step_yz);
      }
    }

    if(UseSMCache)
    {
      // // // // sm->sm
      for(int global_z=p_z_sm_start, cache_z=halo; global_z<p_z_sm_end-halo; global_z+=1, cache_z++)
      {
        process_one_layer<REAL, halo, LOCAL_ITEM_PER_THREAD, BLOCKDIM, LOCAL_TILE_X, halo+1+isBOX, 2*halo+1, reg_folder_z==0?1:reg_folder_z, true,true> (input, output, smbuffer_buffer_ptr, r_smbuffer, global_z,  p_y,  p_x, width_z,  width_y,  width_x, ps_y, ps_x, tile_x_with_halo,cpbase_y, cpend_y, index_y,tid_x, tid_y, stencilParaInput, sm_space, cache_z, cache_z-halo, r_space, 0, 0, boundary_buffer, cache_z+reg_folder_z,  boundary_east_step, boundary_west_step, boundary_north_step, boundary_south_step, boundary_step_yz  );
      }
      // // // // // global->sm
      for(int global_z=p_z_sm_end-halo, cache_z=max_sm_flder; global_z<p_z_sm_end; global_z+=1, cache_z++)
      {
        process_one_layer<REAL, halo, LOCAL_ITEM_PER_THREAD, BLOCKDIM, LOCAL_TILE_X, halo+1+isBOX, 2*halo+1,reg_folder_z==0?1:reg_folder_z, false,true>(input, output, smbuffer_buffer_ptr,  r_smbuffer, global_z,  p_y,  p_x, width_z,  width_y,  width_x, ps_y, ps_x, tile_x_with_halo,  cpbase_y, cpend_y, index_y,  tid_x, tid_y, stencilParaInput, sm_space, 0, cache_z-halo );
      }

    }
    if(!UseSMCache&&!UseRegCache)
    {
      for(int global_z=p_z; global_z<p_z_sm_end; global_z+=1)
      {
        process_one_layer<REAL, halo, LOCAL_ITEM_PER_THREAD, BLOCKDIM,LOCAL_TILE_X, halo+1+isBOX, 2*halo+1>(input, output,  smbuffer_buffer_ptr,  r_smbuffer, global_z,  p_y,  p_x,  width_z,  width_y,  width_x, ps_y, ps_x, tile_x_with_halo,cpbase_y, cpend_y, index_y, tid_x, tid_y, stencilParaInput); 
      }
    }

    __syncthreads();
    //sm boundary
    //sm east and west
    _Pragma("unroll")
    for(int l_z=0; l_z<max_sm_flder; l_z++)
    {
      for(int l_x=tid_y; l_x<halo; l_x+=dim_y)
      {
        for(int l_y=tid_x; l_y<LOCAL_TILE_Y;l_y+=LOCAL_TILE_X)
        {
          //east
          boundary_buffer[boundary_east_step + (l_z+reg_folder_z) *  (LOCAL_TILE_Y+2*isBOX)*halo + (l_y+isBOX) + l_x * (LOCAL_TILE_Y+2*isBOX)] =sm_space[l_z*(LOCAL_TILE_Y)*LOCAL_TILE_X+(l_y)*LOCAL_TILE_X+LOCAL_TILE_X-halo+l_x];

          //west
          boundary_buffer[boundary_west_step + (l_z+reg_folder_z) *  (LOCAL_TILE_Y+2*isBOX)*halo + (l_y+isBOX) + l_x * (LOCAL_TILE_Y+2*isBOX)] = sm_space[l_z*(LOCAL_TILE_Y)*LOCAL_TILE_X+(l_y)*LOCAL_TILE_X+l_x];
        }
      }
    }
    //sm south and north
    _Pragma("unroll")
    for(int l_z=0; l_z<max_sm_flder; l_z++)
    {
      int l_x=tid_x;
      {
        for(int l_y=tid_y; l_y<halo; l_y+=dim_y)
        {
          //south
          {
            boundary_buffer[boundary_south_step + (l_z+reg_folder_z) *  (LOCAL_TILE_X)*halo + (l_x) + l_y * (LOCAL_TILE_X)]
              = sm_space[l_z*(LOCAL_TILE_Y)*LOCAL_TILE_X+(l_y)*LOCAL_TILE_X+l_x];
          }
          //north
          {
            boundary_buffer[boundary_north_step + (l_z+reg_folder_z) *  (LOCAL_TILE_X)*halo + (l_x) + (l_y) * (LOCAL_TILE_X)]
              = sm_space[l_z*(LOCAL_TILE_Y)*LOCAL_TILE_X+(l_y+LOCAL_TILE_Y-halo)*LOCAL_TILE_X+l_x];
          } 
        }
      }
    }
    // general version
    for(int global_z=p_z_sm_end; global_z<p_z_end; global_z+=1)
    {
      process_one_layer<REAL, halo, LOCAL_ITEM_PER_THREAD, BLOCKDIM, LOCAL_TILE_X, halo+1+isBOX, 2*halo+1> (input, output, smbuffer_buffer_ptr,  r_smbuffer, global_z,  p_y,  p_x, width_z,  width_y,  width_x, ps_y, ps_x, tile_x_with_halo, cpbase_y, cpend_y, index_y, tid_x, tid_y, stencilParaInput); 
    }
    __syncthreads();
    if(iter>=iteration-1)break;
    //deal with east and west boundary
    //store to global memory in l2 cache pointer (hopefully)  
   
    {
      int bid_x=blockIdx.x;
      int gdimx=gridDim.x;
      int bid_y=blockIdx.y;
      int gdimy=gridDim.y;
      int bid_z=blockIdx.z;
      //x
      if(gdim_y>=2)
      {
        if(tid_y<dim_y/2)
        {
          for(int l_x=tid_y; l_x<halo; l_x+=dim_y/2)
          {
            //z
            for(int l_z=0; l_z<total_folder_z; l_z++)
            {
              //y
              for(int l_y=tid_x; l_y<LOCAL_TILE_Y; l_y+=LOCAL_TILE_X)
              {
                // //west
                l2_cache_o[l2_boundary_west_step + l_y + bid_y*LOCAL_TILE_Y + (l_x + bid_x*halo)*width_y + (l_z+bid_z*total_folder_z)*width_y*gdimx*halo ] 
                = boundary_buffer[boundary_west_step + (l_z) *  (LOCAL_TILE_Y+2*isBOX)*halo + (l_y+isBOX) + l_x * (LOCAL_TILE_Y+2*isBOX)];
              }
            }
          }
        }
        else
        {
          for(int l_x=tid_y-dim_y/2; l_x<halo; l_x+=dim_y/2)
          {
            //z
            for(int l_z=0; l_z<total_folder_z; l_z++)
            {
              //y
              for(int l_y=tid_x; l_y<LOCAL_TILE_Y; l_y+=LOCAL_TILE_X)
              {
                //east
                l2_cache_o[l2_boundary_east_step + l_y + bid_y*LOCAL_TILE_Y + (l_x + bid_x*halo)*width_y + (l_z+bid_z*total_folder_z)*width_y*gdimx*halo ]  
                = boundary_buffer[boundary_east_step + (l_z) *  (LOCAL_TILE_Y+2*isBOX)*halo + (l_y+isBOX) + l_x * (LOCAL_TILE_Y+2*isBOX)];
              }
            }
          }
        }
      }
      else
      {
        {
          for(int l_x=tid_y; l_x<halo; l_x+=1)
          {
            //z
            for(int l_z=0; l_z<total_folder_z; l_z++)
            {
              //y
              for(int l_y=tid_x; l_y<LOCAL_TILE_Y; l_y+=LOCAL_TILE_X)
              {
                // //west
                l2_cache_o[l2_boundary_west_step + l_y + bid_y*LOCAL_TILE_Y + (l_x + bid_x*halo)*width_y + (l_z+bid_z*total_folder_z)*width_y*gdimx*halo ] 
                = boundary_buffer[boundary_west_step + (l_z) *  (LOCAL_TILE_Y+2*isBOX)*halo + (l_y+isBOX) + l_x * (LOCAL_TILE_Y+2*isBOX)];
              }
            }
          }
        }
        {
          for(int l_x=tid_y; l_x<halo; l_x+=1)
          {
            //z
            for(int l_z=0; l_z<total_folder_z; l_z++)
            {
              //y
              for(int l_y=tid_x; l_y<LOCAL_TILE_Y; l_y+=LOCAL_TILE_X)
              {
                //east
                l2_cache_o[l2_boundary_east_step + l_y + bid_y*LOCAL_TILE_Y + (l_x + bid_x*halo)*width_y + (l_z+bid_z*total_folder_z)*width_y*gdimx*halo ]  
                = boundary_buffer[boundary_east_step + (l_z) *  (LOCAL_TILE_Y+2*isBOX)*halo + (l_y+isBOX) + l_x * (LOCAL_TILE_Y+2*isBOX)];
              }
            }
          }
        }
      }
      // // //north south
      if(gdim_y>=2)
      {
        if(tid_y<dim_y/2)
        {
          for(int l_y=tid_y; l_y<halo; l_y+=dim_y/2)
          {
            //z
            for(int l_z=0; l_z<total_folder_z; l_z++)
            {
              //y
              {
                int l_x=tid_x;
                // //north
                l2_cache_o[l2_boundary_north_step + l_x + bid_x * TILE_X + (l_y + bid_y * halo) * width_x + (l_z + bid_z * total_folder_z) * width_x * gdimy*halo ] 
                  = boundary_buffer[boundary_north_step + (l_z) *  (LOCAL_TILE_X)*halo + (l_x) + l_y * (LOCAL_TILE_X)];
              }
            }
          }
        }
        else
        {
          for(int l_y=tid_y-dim_y/2; l_y<halo; l_y+=dim_y/2)
          {
            //z
            for(int l_z=0; l_z<total_folder_z; l_z++)
            {
              //y
              {
                int l_x=tid_x;
                // south 
                l2_cache_o[l2_boundary_south_step + l_x + bid_x * TILE_X + (l_y + bid_y * halo) * width_x + (l_z + bid_z * total_folder_z) * width_x * gdimy*halo ]  
                  = boundary_buffer[boundary_south_step + (l_z) *  (LOCAL_TILE_X)*halo + (l_x) + l_y * (LOCAL_TILE_X)];
              }
            }
          }
        }
      }
      else
      {
        // if(tid_y<dim_y/2)
        {
          for(int l_y=tid_y; l_y<halo; l_y+=1)
          {
            //z
            for(int l_z=0; l_z<total_folder_z; l_z++)
            {
              //y
              {
                int l_x=tid_x;
                // //north
                l2_cache_o[l2_boundary_north_step + l_x + bid_x * TILE_X + (l_y + bid_y * halo) * width_x + (l_z + bid_z * total_folder_z) * width_x * gdimy*halo ] 
                  = boundary_buffer[boundary_north_step + (l_z) *  (LOCAL_TILE_X)*halo + (l_x) + l_y * (LOCAL_TILE_X)];
              }
            }
          }
        }
        // else
        {
          for(int l_y=tid_y; l_y<halo; l_y+=1)
          {
            //z
            for(int l_z=0; l_z<total_folder_z; l_z++)
            {
              //y
              {
                int l_x=tid_x;
                // south 
                l2_cache_o[l2_boundary_south_step + l_x + bid_x * TILE_X + (l_y + bid_y * halo) * width_x + (l_z + bid_z * total_folder_z) * width_x * gdimy*halo ]  
                  = boundary_buffer[boundary_south_step + (l_z) *  (LOCAL_TILE_X)*halo + (l_x) + l_y * (LOCAL_TILE_X)];
              }
            }
          }
        }
      }

    }

    gg.sync();
    //load frm global memory in l2 cache pointer (hopefully)
    REAL* tmp_ptr =output;
    output=input;
    input=tmp_ptr;

    tmp_ptr=l2_cache_o;
    l2_cache_o=l2_cache_i;
    l2_cache_i=tmp_ptr;

    {

      // int bid_y=blockIdx.x/gdim_x;
      int bid_x=blockIdx.x;
      int gdimx=gridDim.x;

      int bid_y=blockIdx.y;
      int gdimy=gridDim.y;
      
      int bid_z=blockIdx.z;
      //x
      if(gdim_y>=2)
      {
        if(tid_y<dim_y/2)
        {
          for(int l_x=tid_y; l_x<halo; l_x+=dim_y/2)
          {
            //z
            for(int l_z=0; l_z<total_folder_z; l_z++)
            {
              //y
              for(int l_y=tid_x-isBOX; l_y<LOCAL_TILE_Y+isBOX; l_y+=LOCAL_TILE_X)
              {
                int l2_cache_l_y=MAX(l_y+ bid_y*LOCAL_TILE_Y,0);
                l2_cache_l_y=MIN(l2_cache_l_y,width_y-1);

                //east
                boundary_buffer[boundary_east_step + (l_z) *  (LOCAL_TILE_Y+2*isBOX)*halo+ (l_y+isBOX) + l_x * (LOCAL_TILE_Y+2*isBOX)] =
                  (bid_x==gdimx-1?
                  l2_cache_i[l2_boundary_east_step+ l2_cache_l_y  + ((halo-1) + bid_x*halo)*width_y + (l_z+bid_z*total_folder_z)*width_y*gdimx*halo ]  
                 :
                 l2_cache_i[l2_boundary_west_step+l2_cache_l_y  + (l_x + (bid_x+1)*halo)*width_y + (l_z+bid_z*total_folder_z)*width_y*gdimx*halo  ]
                 )
                 ;

              }
            }
          }
        }
        else
        {
          for(int l_x=tid_y-dim_y/2; l_x<halo; l_x+=dim_y/2)
          {
            //z
            for(int l_z=0; l_z<total_folder_z; l_z++)
            {
              //y
              for(int l_y=tid_x-isBOX; l_y<LOCAL_TILE_Y+isBOX; l_y+=LOCAL_TILE_X)
              {
                int l2_cache_l_y=MAX(l_y+ bid_y*LOCAL_TILE_Y,0);
                l2_cache_l_y=MIN(l2_cache_l_y,width_y-1);

                //west
                boundary_buffer[boundary_west_step + (l_z) *  (LOCAL_TILE_Y+2*isBOX)*halo + (l_y+isBOX) + l_x * (LOCAL_TILE_Y+2*isBOX)] =
                  (bid_x==0?
                    l2_cache_i[l2_boundary_west_step+ l2_cache_l_y  + (0 + bid_x*halo)*width_y + (l_z+bid_z*total_folder_z)*width_y*gdimx*halo ] 
                    :
                    l2_cache_i[l2_boundary_east_step+ l2_cache_l_y  + (l_x + (bid_x-1)*halo)*width_y + (l_z+bid_z*total_folder_z)*width_y*gdimx*halo ])
                    ;
              }
            }
          }
        }
        if(tid_y<dim_y/2)
        {
          for(int l_y=tid_y; l_y<halo; l_y+=dim_y/2)
          {
            //z
            for(int l_z=0; l_z<total_folder_z; l_z++)
            {
              //y
              {
                int l_x=tid_x;
                if(tid_y<halo)
                //north
                boundary_buffer[boundary_north_step + (l_z) *  (LOCAL_TILE_X)*halo + (l_x) + l_y * (LOCAL_TILE_X)] =
                  (bid_y==gdimy-1?
                 boundary_buffer[boundary_north_step + (l_z) *  (LOCAL_TILE_X)*halo + (l_x) + (halo-1) * (LOCAL_TILE_X)]
                 :
                 l2_cache_i[l2_boundary_south_step + l_x + bid_x * LOCAL_TILE_X + (l_y + (bid_y+1) * halo) * width_x + (l_z + bid_z * total_folder_z) * width_x * gdimy*halo  ]
                 )
                 ;
                //south
                boundary_buffer[boundary_south_step + (l_z) *  (LOCAL_TILE_X)*halo + (l_x) + l_y * (LOCAL_TILE_X)] =
                  (bid_y==0?
                    boundary_buffer[boundary_south_step + (l_z) *  (LOCAL_TILE_X)*halo + (l_x) + 0 * (LOCAL_TILE_X)]
                    :
                    l2_cache_i[l2_boundary_north_step + l_x + bid_x * LOCAL_TILE_X + (l_y + (bid_y-1) * halo) * width_x + (l_z + bid_z * total_folder_z) * width_x * gdimy*halo ])
                    ;
              }
            }
          }
        }
        else
        {
          for(int l_y=tid_y-dim_y/2; l_y<halo; l_y+=dim_y/2)
          {
            //z
            for(int l_z=0; l_z<total_folder_z; l_z++)
            {
              //y
              {
                int l_x=tid_x;
                //north
                boundary_buffer[boundary_north_step + (l_z) *  (LOCAL_TILE_X)*halo + (l_x) + l_y * (LOCAL_TILE_X)] =
                  (bid_y==gdimy-1?
                 boundary_buffer[boundary_north_step + (l_z) *  (LOCAL_TILE_X)*halo + (l_x) + (halo-1) * (LOCAL_TILE_X)]
                 :
                 l2_cache_i[l2_boundary_south_step + l_x + bid_x * LOCAL_TILE_X + (l_y + (bid_y+1) * halo) * width_x + (l_z + bid_z * total_folder_z) * width_x * gdimy*halo  ]
                 )
                 ;

              }
            }
          }
        }

      }
      else
      {
        // if(tid_y<dim_y/2)
        {
          for(int l_x=tid_y; l_x<halo; l_x+=1)
          {
            //z
            for(int l_z=0; l_z<total_folder_z; l_z++)
            {
              //y
              for(int l_y=tid_x-isBOX; l_y<LOCAL_TILE_Y+isBOX; l_y+=LOCAL_TILE_X)
              {
                int l2_cache_l_y=MAX(l_y+ bid_y*LOCAL_TILE_Y,0);
                l2_cache_l_y=MIN(l2_cache_l_y,width_y-1);

                //east
                boundary_buffer[boundary_east_step + (l_z) *  (LOCAL_TILE_Y+2*isBOX)*halo+ (l_y+isBOX) + l_x * (LOCAL_TILE_Y+2*isBOX)] =
                  (bid_x==gdimx-1?
                  l2_cache_i[l2_boundary_east_step+ l2_cache_l_y  + ((halo-1) + bid_x*halo)*width_y + (l_z+bid_z*total_folder_z)*width_y*gdimx*halo ]  
                 :
                 l2_cache_i[l2_boundary_west_step+l2_cache_l_y  + (l_x + (bid_x+1)*halo)*width_y + (l_z+bid_z*total_folder_z)*width_y*gdimx*halo  ]
                 )
                 ;

              }
            }
          }
        }
        // else
        {
          for(int l_x=tid_y; l_x<halo; l_x+=1)
          {
            //z
            for(int l_z=0; l_z<total_folder_z; l_z++)
            {
              //y
              for(int l_y=tid_x-isBOX; l_y<LOCAL_TILE_Y+isBOX; l_y+=LOCAL_TILE_X)
              {
                int l2_cache_l_y=MAX(l_y+ bid_y*LOCAL_TILE_Y,0);
                l2_cache_l_y=MIN(l2_cache_l_y,width_y-1);

                //west
                boundary_buffer[boundary_west_step + (l_z) *  (LOCAL_TILE_Y+2*isBOX)*halo + (l_y+isBOX) + l_x * (LOCAL_TILE_Y+2*isBOX)] =
                  (bid_x==0?
                    l2_cache_i[l2_boundary_west_step+ l2_cache_l_y  + (0 + bid_x*halo)*width_y + (l_z+bid_z*total_folder_z)*width_y*gdimx*halo ] 
                    :
                    l2_cache_i[l2_boundary_east_step+ l2_cache_l_y  + (l_x + (bid_x-1)*halo)*width_y + (l_z+bid_z*total_folder_z)*width_y*gdimx*halo ])
                    ;
              }
            }
          }
        }
        {
          for(int l_y=tid_y; l_y<halo; l_y+=1)
          {
            //z
            for(int l_z=0; l_z<total_folder_z; l_z++)
            {
              //y
              {
                int l_x=tid_x;
                if(tid_y<halo)
                //north
                boundary_buffer[boundary_north_step + (l_z) *  (LOCAL_TILE_X)*halo + (l_x) + l_y * (LOCAL_TILE_X)] =
                  (bid_y==gdimy-1?
                 boundary_buffer[boundary_north_step + (l_z) *  (LOCAL_TILE_X)*halo + (l_x) + (halo-1) * (LOCAL_TILE_X)]
                 :
                 l2_cache_i[l2_boundary_south_step + l_x + bid_x * LOCAL_TILE_X + (l_y + (bid_y+1) * halo) * width_x + (l_z + bid_z * total_folder_z) * width_x * gdimy*halo  ]
                 )
                 ;
                //south
                boundary_buffer[boundary_south_step + (l_z) *  (LOCAL_TILE_X)*halo + (l_x) + l_y * (LOCAL_TILE_X)] =
                  (bid_y==0?
                    boundary_buffer[boundary_south_step + (l_z) *  (LOCAL_TILE_X)*halo + (l_x) + 0 * (LOCAL_TILE_X)]
                    :
                    l2_cache_i[l2_boundary_north_step + l_x + bid_x * LOCAL_TILE_X + (l_y + (bid_y-1) * halo) * width_x + (l_z + bid_z * total_folder_z) * width_x * gdimy*halo ])
                    ;
              }
            }
          }
        }
        {
          for(int l_y=tid_y; l_y<halo; l_y+=1)
          {
            //z
            for(int l_z=0; l_z<total_folder_z; l_z++)
            {
              //y
              {
                int l_x=tid_x;

                //north
                boundary_buffer[boundary_north_step + (l_z) *  (LOCAL_TILE_X)*halo + (l_x) + l_y * (LOCAL_TILE_X)] =
                  (bid_y==gdimy-1?
                 boundary_buffer[boundary_north_step + (l_z) *  (LOCAL_TILE_X)*halo + (l_x) + (halo-1) * (LOCAL_TILE_X)]
                 :
                 l2_cache_i[l2_boundary_south_step + l_x + bid_x * LOCAL_TILE_X + (l_y + (bid_y+1) * halo) * width_x + (l_z + bid_z * total_folder_z) * width_x * gdimy*halo  ]
                 )
                 ;

              }
            }
          }
        }
      }
      __syncthreads();
    }
  }

  for(int global_z=p_z_reg_start, cache_z_reg=halo; global_z<p_z_sm_start; global_z+=1, cache_z_reg++)
  {
      _Pragma("unroll")
      for(int l_y=0; l_y<LOCAL_ITEM_PER_THREAD; l_y++)
      {
        int local_y=l_y+LOCAL_ITEM_PER_THREAD*tid_y;

        output[global_z*width_x*width_y+(p_y+local_y)*width_x+p_x+tid_x]  = r_space[cache_z_reg-halo][l_y];
      }  
  } 
  for(int global_z=p_z_sm_start, cache_z=halo; global_z<p_z_sm_end; global_z+=1, cache_z++)
  {
      _Pragma("unroll")
      for(int l_y=0; l_y<LOCAL_ITEM_PER_THREAD; l_y++)
      {
        int local_y=l_y+LOCAL_ITEM_PER_THREAD*tid_y;

        output[global_z*width_x*width_y+(p_y+local_y)*width_x+p_x+tid_x]  =
          sm_space[(cache_z-halo)*LOCAL_TILE_X*LOCAL_TILE_Y+(local_y)*LOCAL_TILE_X+tid_x];
      }  
  }
 
  #undef UseRegCache
  #undef LOCAL_TILE_Y
  #undef gdim_y
}
\end{lstlisting}

==> COI.tex <==
Erez Petrank
Ganging Tan
Jiajia Li
Julian Shun
Naama Ben-David
Xu Liu

==> TABLES/Speedups.tex <==

\begin{comment}
\begin{table*}[t]
    \centering
    % \tiny
    \caption{Speedup of PERKS over baseline (non-persistent kernels) 
    for 2D/3D stencil benchmarks on A100 and V100 GPUs. For benchmarks two problem sizes are reported: 1) for domain sizes large enough to saturate the device (i.e. weak scaling simulations), and 2) for domain sizes that can be Full in PERKS (i.e. strong scaling simulations); Label Explanation: \emph{BM} = Benchmarks, \emph{\$ing} = Caching,  \emph{\% \$ed} = Percentage Cached, \emph{Perf} = Performance in Giga-cells Updated per Second, {$\uparrow$} = Speedup, GM: Geometric Mean.
    }
    \resizebox{\textwidth}{!}
    {%
    \begin{tabular}{|l|c|cccc|cccc|cccc|cccc|}\hline
 \multirow{3}{*}{\LARGE {\textbf{BM}}} & \multirow{3}{*}{\LARGE {\textbf{\$}}}&\multicolumn{8}{c|}{\LARGE {\textbf{Single Precision}}}&\multicolumn{8}{c|}{{\LARGE \textbf{Double Precision}}}\\ \cline{3-18}
                                 &                               &\multicolumn{4}{c|}{{\LARGE \textbf{A100}}} & \multicolumn{4}{c|}{{\LARGE \textbf{V100}}}  & \multicolumn{4}{c|}{{\LARGE \textbf{A100}}}  &\multicolumn{4}{c|}{{\LARGE \textbf{V100}}}   \\\cline{3-18}
                                  &                               &  {\Large Dom Size}       &       {\Large \% \$ed}         & {\Large Perf}       & {\Large \contour{black}{$\uparrow$}}         & 
                                   {\Large Dom Size}       &       {\Large \% \$ed}     &   {\Large Perf}               &  {\Large \contour{black}{$\uparrow$}}         & 
                                  {\Large Dom Size}      &       {\Large \% \$ed}     &     {\Large Perf}          & {\Large \contour{black}{$\uparrow$}}         & 
                               {\Large Dom Size}       &       {\Large \% \$ed}     &{\Large Perf}  & {\Large \contour{black}{$\uparrow$}}               \\\hline 

\rowcolor{Gray}\cellcolor{white}\multirow{2}{*}{{ \textbf{2d5pt}}}   
& Part & {\small$4608\times3072$}        & $59\% $ & $257.74$ & \textbf{1.66} & $4096\times2560$       & $38\% $ & $137.30$ & \textbf{1.49} & $2304\times2304$       & $88\% $  & $285.63$ & \textbf{3.69} & $2048\times1280$    & $88\% $ & $241.63$& \textbf{5.45} \\
& Full    & $3072\times2160$        & $100\%$ & $636.79$ & \textbf{4.34} & $2560\times1536$       & $100\%$ & $494.64$ & \textbf{5.56} & $2304\times1536$       & $100\%$  & $335.42$ & \textbf{4.46} & $2048\times1120$    & $100\%$ & $277.08$& \textbf{6.44} \\\hline 
\rowcolor{Gray}\cellcolor{white}\multirow{2}{*}{{ \textbf{2ds9pt}}} 
& Part & $4608\times3072$        & $64\% $ & $229.88$ & \textbf{1.51} & $2560\times2048$       & $94\% $ & $301.32$ & \textbf{3.48} & $2304\times2304$       & $79\% $  & $194.48$ & \textbf{2.70} & $2048\times1280$    & $75\% $ & $108.49$& \textbf{2.51} \\
& Full    & $4608\times1824$        & $100\%$ & $463.25$ & \textbf{3.59} & $2048\times1760$       & $100\%$ & $352.98$ & \textbf{4.20} & $2304\times1152$       & $100\%$  & $235.70$ & \textbf{3.20} & $1536\times1280$    & $100\%$ & $188.32$& \textbf{4.39} \\\hline 
\rowcolor{Gray}\cellcolor{white}\multirow{2}{*}{{ \textbf{2d13pt}}} 
& Part & $4608\times3072$        & $47\% $ & $197.83$ & \textbf{1.35} & $2560\times2048$       & $94\% $ & $222.71$ & \textbf{2.64} & $4608\times3072$       & $13\% $  & $84.40 $ & \textbf{1.10} & $2048\times2048$    & $47\% $ & $58.99 $& \textbf{1.40} \\
& Full    & $4608\times1440$        & $100\%$ & $357.40$ & \textbf{2.86} & $2560\times1408$       & $100\%$ & $266.54$ & \textbf{3.25} & $4608\times576 $       & $100\%$  & $181.19$ & \textbf{2.71} & $2048\times800 $    & $100\%$ & $141.26$& \textbf{3.62} \\\hline 
\rowcolor{Gray}\cellcolor{white}\multirow{2}{*}{{ \textbf{2d17pt}}}  
& Part & $4608\times3072$        & $50\% $ & $170.91$ & \textbf{1.28} & $5120\times4096$       & $14\% $ & $99.45 $ & \textbf{1.16} & $3072\times2304$       & $47\% $  & $91.77 $ & \textbf{1.34} & $4096\times2560$    & $14\% $ & $47.52 $& \textbf{1.18} \\
& Full    & $3072\times2448$        & $100\%$ & $280.19$ & \textbf{2.63} & $4096\times800 $       & $100\%$ & $207.62$ & \textbf{2.76} & $2304\times1440$       & $100\%$  & $145.53$ & \textbf{2.30} & $2560\times576 $    & $100\%$ & $109.57$& \textbf{3.18} \\\hline 
\rowcolor{Gray}\cellcolor{white}\multirow{2}{*}{{ \textbf{2d21pt}}}
& Part & $4608\times3072$        & $41\% $ & $151.78$ & \textbf{1.21} & $2560\times2048$       & $75\% $ & $124.12$ & \textbf{1.60} & $4608\times3072$       & $6\%  $  & $73.44 $ & \textbf{1.13} & $5120\times4096$    & $0\%  $ & $46.76 $& \textbf{1.12} \\
& Full    & $4608\times1536$        & $100\%$ & $233.71$ & \textbf{2.10} & $2560\times1408$       & $100\%$ & $178.40$ & \textbf{2.39} & $3072\times1008$       & $100.00\%$  & $118.98$ & \textbf{2.29} & $4096\times320 $    & $100\%$ & $89.87 $& \textbf{2.63} \\\hline 
\rowcolor{Gray}\cellcolor{white}\multirow{2}{*}{{ \textbf{2ds25pt}}}  
& Part & $4608\times4608$        & $13\% $ & $126.98$ & \textbf{1.05} & $2048\times2048$       & $78\% $ & $105.91$ & \textbf{1.41} & $4608\times4608$       & $2\%  $  & $69.29 $ & \textbf{1.22} & $5120\times4096$    & $0\%  $ & $46.79 $& {\textbf1.21} \\
& Full    & $4608\times672 $        & $100\%$ & $192.49$ & \textbf{1.81} & $2048\times1600$       & $100\%$ & $149.50$ & \textbf{2.06} & $4608\times576 $       & $100\%$  & $96.98 $  &\textbf{2.00} & $4096\times280 $    & $100.00\%$ & $61.96 $ &{\textbf2.13} \\\hline 
\rowcolor{Gray}\cellcolor{white}\multirow{2}{*}{{ \textbf{2d9pt}}}     
& Part & $3072\times3072$        & $98\% $ & $491.51$ & \textbf{3.44} & $2560\times2048$       & $97\% $ & $388.20$ & \textbf{4.30} & $2304\times2304$       & $83\% $  & $247.35$ & \textbf{3.27} & $2048\times1280$    & $88\% $ & $189.82$& \textbf{4.27} \\
& Full    & $3072\times2592$        & $100\%$ & $547.10$ & \textbf{4.03} & $2560\times1664$       & $100\%$ & $408.36$ & \textbf{4.61} & $2304\times1920$       & $100\%$  & $289.90$ & \textbf{3.89} & $1792\times1280$    & $100\%$ & $227.56$& \textbf{5.15} \\\hline 
\rowcolor{Gray}\cellcolor{white}\multirow{2}{*}{{ \textbf{2d25pt}}}  
& Part & $4608\times3072$        & $47\% $ & $187.21$ & \textbf{1.26} & $2560\times2048$       & $91\% $ & $196.04$ & \textbf{2.29} & $4608\times3072$       & $13\% $  & $82.56 $ & \textbf{1.13} & $2048\times1280$    & $63\% $ & $67.39 $& \textbf{1.58} \\
& Full    & $4608\times1536$        & $100\%$ & $274.74$ & \textbf{2.04} & $2560\times1408$       & $100\%$ & $212.94$ & \textbf{2.56} & $4608\times816 $       & $100\%$  & $139.38$ & \textbf{2.28} & $2048\times720 $    & $100\%$ & $105.13$& \textbf{2.64} \\\hhline{|=|=|====|====|====|====|}
 \textbf{GM(2D)}& - & -& -&-&  \textbf{2.04}& -& -& -& \textbf{2.60}&- &- &- & \textbf{2.19}& -& -& -& \textbf{2.63}\\\hhline{|=|=|====|====|====|====|}

\rowcolor{Gray}\cellcolor{white}\multirow{2}{*}{{ \textbf{3d7pt}}}    
& Part & $256\times288\times256$ & $21\%  $& $159.95 $& \textbf{1.19}& $256\times160\times256 $& $27\%  $& $99.49  $& \textbf{1.21}& $256\times288\times256 $& $0 \%  $& $77.58  $& \textbf{1.08}& $128\times128\times128 $& $47\%  $& $56.47  $& \textbf{1.67}\\
& Full    & $126\times192\times256$ & $100\% $& $274.37 $& \textbf{2.23}& $68\times160\times256  $& $100\% $& $212.58 $& \textbf{3.21}& $39\times288\times256  $& $100\% $& $146.25 $& \textbf{2.24}& $80\times128\times128  $& $100\% $& $98.33  $& \textbf{2.99}\\\hline 
\rowcolor{Gray}\cellcolor{white}\multirow{2}{*}{{ \textbf{3d13pt}}}  
& Part & $256\times288\times256 $& $0\%   $& $129.16 $& \textbf{1.12}& $256\times320\times256 $& $0\%   $& $86.94 $ & \textbf{1.06}& $256\times288\times256 $& $2\%   $& $70.15$  & \textbf{1.18}& $256\times320\times256 $& $0\%   $& $41.04  $& \textbf{1.03}\\
& Full    & $81\times288\times256  $& $100\% $& $152.15 $& \textbf{1.47}& $32\times320\times256  $& $100\% $& $137.67$ & \textbf{2.46}& $33\times288\times256  $& $100\% $& $92.62$  & \textbf{1.77}& $8\times320\times256   $& $100\% $& $46.93  $& \textbf{1.90}\\\hline 
\rowcolor{Gray}\cellcolor{white}\multirow{2}{*}{{ \textbf{3d17pt}}}   
& Part & $256\times288\times256 $& $28\%  $& $138.53 $& \textbf{1.07}& $160\times160\times256 $& $45\%  $&$ 94.45  $& \textbf{1.34}& $256\times288\times256 $& $2\%   $& $75.16$  & \textbf{1.13}& $160\times160\times256 $& $13\%  $& $45.54$  & \textbf{1.40}\\
& Full    & $84\times288\times256  $& $100\% $& $170.66 $& \textbf{1.51}& $160\times64\times256  $& $100\% $&$ 131.01 $& \textbf{2.12}& $36\times288\times256  $& $100\% $& $87.97$  & \textbf{1.53}& $32\times160\times256  $& $100\% $& $64.43$  & \textbf{2.37}\\\hline 
\rowcolor{Gray}\cellcolor{white}\multirow{2}{*}{{ \textbf{3d27pt}}}   
& Part & $256\times288\times256 $& $14\%  $& $130.88$ & \textbf{1.01}& $160\times160\times256 $& $45\%  $& $94.32  $& \textbf{1.34}& $256\times288\times256 $& $5\%   $& $75.22  $& \textbf{1.14}& $160\times160\times256 $& $13\%  $& $45.69$  & \textbf{1.40}\\
& Full    & $81\times192\times256  $& $100\% $& $162.22$ & \textbf{1.33}& $160\times64\times256  $& $100\% $& $130.99 $& \textbf{2.12}& $33\times288\times256  $& $100\% $& $86.89  $& \textbf{1.43}& $32\times160\times256  $& $100\% $& $64.01$  & \textbf{2.35}\\\hline 
\rowcolor{Gray}\cellcolor{white}\multirow{2}{*}{{ \textbf{Poisson}}}  
& Part & $256\times288\times256$& $14\%  $& $130.50 $&  \textbf{1.01}& $160\times160\times256 $& $30\%  $& $94.70  $& \textbf{1.35}& $256\times288\times256 $& $2\%   $& $73.13  $& \textbf{1.12}& $160\times160\times256 $& $13\%  $& $45.78  $& \textbf{1.41}\\
& Full    & $90\times288\times256 $& $100\% $& $164.00 $&  \textbf{1.45}& $160\times64\times256  $& $100\% $& $130.89 $& \textbf{2.12}& $36\times288\times256  $& $100\% $& $87.59  $& \textbf{1.54}& $32\times160\times256  $& $100\% $& $64.92  $& \textbf{2.39}\\\hhline{|=|=|====|====|====|====|}
 \textbf{GM(3D)}& - & - &- &-&  \textbf{1.30}& -& -& -& \textbf{1.72}& -& -& -& \textbf{1.38}& -& -& -& \textbf{1.80}\\\hhline{|=|=|====|====|====|====|}
    \end{tabular}
    }
    \label{tab:stencil_speedups}
\end{table*}
\end{comment}

\begin{table*}[t]
    \centering
    % \tiny
    \caption{Speedup of PERKS over baseline (non-persistent kernels) 
    for 2D/3D stencil benchmarks on A100 and V100 GPUs. For benchmarks two problem sizes are reported: 1) for domain sizes large enough to saturate the device (i.e. weak scaling simulations), and 2) for domain sizes that can be Full in PERKS (i.e. strong scaling simulations); Label Explanation: \emph{BM} = Benchmarks, \emph{\$} = Cache, \emph{P} = Partially Cache, \emph{F} = Fully Cache, \emph{\% \$ed} = Percentage Cached, \emph{Perf.} = Performance in Giga-cells Updated per Second, {$\uparrow$} = Speedup, GM: Geometric Mean.
    }
    \resizebox{\textwidth}{!}
    {%
    \begin{tabular}{|l|c|cccc|cccc|cccc|cccc|}\hline
 \multirow{3}{*}{\LARGE {\textbf{BM}}} & \multirow{3}{*}{\LARGE {\textbf{\$}}}&\multicolumn{8}{c|}{\LARGE {\textbf{Single Precision}}}&\multicolumn{8}{c|}{{\LARGE \textbf{Double Precision}}}\\ \cline{3-18}
                                 &                               &\multicolumn{4}{c|}{{\LARGE \textbf{A100}}} & \multicolumn{4}{c|}{{\LARGE \textbf{V100}}}  & \multicolumn{4}{c|}{{\LARGE \textbf{A100}}}  &\multicolumn{4}{c|}{{\LARGE \textbf{V100}}}   \\\cline{3-18}
                                  &                               &  {\Large Domain Size}       &       {\Large \% \$ed}         & {\Large Perf.}       & {\Large \contour{black}{$\uparrow$}}         & 
                                   {\Large Domain Size}       &       {\Large \% \$ed}     &   {\Large Perf.}               &  {\Large \contour{black}{$\uparrow$}}         & 
                                  {\Large Domain Size}      &       {\Large \% \$ed}     &     {\Large Perf.}          & {\Large \contour{black}{$\uparrow$}}         & 
                               {\Large Domain Size}       &       {\Large \% \$ed}     &{\Large Perf.}  & {\Large \contour{black}{$\uparrow$}}               \\\hline 

\rowcolor{Gray}\cellcolor{white}\multirow{2}{*}{{\LARGE \textbf{2d5pt}}}   
& P & $4608\times3072$        & $59\% $ & $257.74$ & {\Large\textbf{1.66}} & {$4096\times2560$ }      & $38\% $ & $137.30$ & {\Large\textbf{1.49}} & $2304\times2304$       & $88\% $  & $285.63$ & {\Large\textbf{3.69}} & $2048\times1280$    & $88\% $ & $241.63$& {\Large\textbf{5.45}} \\
& F    & $3072\times2160$        & $100\%$ & $636.79$ & {\Large\textbf{4.34}} & $2560\times1536$       & $100\%$ & $494.64$ & {\Large\textbf{5.56}} & $2304\times1536$       & $100\%$  & $335.42$ & {\Large\textbf{4.46}} & $2048\times1120$    & $100\%$ & $277.08$& {\Large\textbf{6.44}} \\\hline 
\rowcolor{Gray}\cellcolor{white}\multirow{2}{*}{{\LARGE \textbf{2ds9pt}}} 
& P & $4608\times3072$        & $64\% $ & $229.88$ & {\Large\textbf{1.51}} & $2560\times2048$       & $94\% $ & $301.32$ & {\Large\textbf{3.48}} & $2304\times2304$       & $79\% $  & $194.48$ & {\Large\textbf{2.70}} & $2048\times1280$    & $75\% $ & $108.49$& {\Large\textbf{2.51}} \\
& F    & $4608\times1824$        & $100\%$ & $463.25$ & {\Large\textbf{3.59}} & $2048\times1760$       & $100\%$ & $352.98$ & {\Large\textbf{4.20}} & $2304\times1152$       & $100\%$  & $235.70$ & {\Large\textbf{3.20}} & $1536\times1280$    & $100\%$ & $188.32$& {\Large\textbf{4.39}} \\\hline 
\rowcolor{Gray}\cellcolor{white}\multirow{2}{*}{{\LARGE \textbf{2d13pt}}} 
& P & $4608\times3072$        & $47\% $ & $197.83$ & {\Large\textbf{1.35}} & $2560\times2048$       & $94\% $ & $222.71$ & {\Large\textbf{2.64}} & $4608\times3072$       & $13\% $  & $84.40 $ & {\Large\textbf{1.10}} & $2048\times2048$    & $47\% $ & $58.99 $& {\Large\textbf{1.40}} \\
& F    & $4608\times1440$        & $100\%$ & $357.40$ & {\Large\textbf{2.86}} & $2560\times1408$       & $100\%$ & $266.54$ & {\Large\textbf{3.25}} & $4608\times576 $       & $100\%$  & $181.19$ & {\Large\textbf{2.71}} & $2048\times800 $    & $100\%$ & $141.26$& {\Large\textbf{3.62}} \\\hline 
\rowcolor{Gray}\cellcolor{white}\multirow{2}{*}{{\LARGE \textbf{2d17pt}}}  
& P & $4608\times3072$        & $50\% $ & $170.91$ & {\Large\textbf{1.28}} & $5120\times4096$       & $14\% $ & $99.45 $ & {\Large\textbf{1.16}} & $3072\times2304$       & $47\% $  & $91.77 $ & {\Large\textbf{1.34}} & $4096\times2560$    & $14\% $ & $47.52 $& {\Large\textbf{1.18}} \\
& F    & $3072\times2448$        & $100\%$ & $280.19$ & {\Large\textbf{2.63}} & $4096\times800 $       & $100\%$ & $207.62$ & {\Large\textbf{2.76}} & $2304\times1440$       & $100\%$  & $145.53$ & {\Large\textbf{2.30}} & $2560\times576 $    & $100\%$ & $109.57$& {\Large\textbf{3.18}} \\\hline 
\rowcolor{Gray}\cellcolor{white}\multirow{2}{*}{{\LARGE \textbf{2d21pt}}}
& P & $4608\times3072$        & $41\% $ & $151.78$ & {\Large\textbf{1.21}} & $2560\times2048$       & $75\% $ & $124.12$ & {\Large\textbf{1.60}} & $4608\times3072$       & $6\%  $  & $73.44 $ & {\Large\textbf{1.13}} & $5120\times4096$    & $0\%  $ & $46.76 $& {\Large\textbf{1.12}} \\
& F    & $4608\times1536$        & $100\%$ & $233.71$ & {\Large\textbf{2.10}} & $2560\times1408$       & $100\%$ & $178.40$ & {\Large\textbf{2.39}} & $3072\times1008$       & $100.00\%$  & $118.98$ & {\Large\textbf{2.29}} & $4096\times320 $    & $100\%$ & $89.87 $& {\Large\textbf{2.63}} \\\hline 
\rowcolor{Gray}\cellcolor{white}\multirow{2}{*}{{\LARGE \textbf{2ds25pt}}}  
& P & $4608\times4608$        & $13\% $ & $126.98$ & {\Large\textbf{1.05}} & $2048\times2048$       & $78\% $ & $105.91$ & {\Large\textbf{1.41}} & $4608\times4608$       & $2\%  $  & $69.29 $ & {\Large\textbf{1.22}} & $5120\times4096$    & $0\%  $ & $46.79 $& {{\Large\textbf1.21}} \\
& F    & $4608\times672 $        & $100\%$ & $192.49$ & {\Large\textbf{1.81}} & $2048\times1600$       & $100\%$ & $149.50$ & {\Large\textbf{2.06}} & $4608\times576 $       & $100\%$  & $96.98 $  &{\Large\textbf{2.00}} & $4096\times280 $    & $100.00\%$ & $61.96 $ &{{\Large\textbf2.13}} \\\hline 
\rowcolor{Gray}\cellcolor{white}\multirow{2}{*}{{\LARGE \textbf{2d9pt}}}     
& P & $3072\times3072$        & $98\% $ & $491.51$ & {\Large\textbf{3.44}} & $2560\times2048$       & $97\% $ & $388.20$ & {\Large\textbf{4.30}} & $2304\times2304$       & $83\% $  & $247.35$ & {\Large\textbf{3.27}} & $2048\times1280$    & $88\% $ & $189.82$& {\Large\textbf{4.27}} \\
& F    & $3072\times2592$        & $100\%$ & $547.10$ & {\Large\textbf{4.03}} & $2560\times1664$       & $100\%$ & $408.36$ & {\Large\textbf{4.61}} & $2304\times1920$       & $100\%$  & $289.90$ & {\Large\textbf{3.89}} & $1792\times1280$    & $100\%$ & $227.56$& {\Large\textbf{5.15}} \\\hline 
\rowcolor{Gray}\cellcolor{white}\multirow{2}{*}{{\LARGE \textbf{2d25pt}}}  
& P & $4608\times3072$        & $47\% $ & $187.21$ & {\Large\textbf{1.26}} & $2560\times2048$       & $91\% $ & $196.04$ & {\Large\textbf{2.29}} & $4608\times3072$       & $13\% $  & $82.56 $ & {\Large\textbf{1.13}} & $2048\times1280$    & $63\% $ & $67.39 $& {\Large\textbf{1.58}} \\
& F    & $4608\times1536$        & $100\%$ & $274.74$ & {\Large\textbf{2.04}} & $2560\times1408$       & $100\%$ & $212.94$ & {\Large\textbf{2.56}} & $4608\times816 $       & $100\%$  & $139.38$ & {\Large\textbf{2.28}} & $2048\times720 $    & $100\%$ & $105.13$& {\Large\textbf{2.64}} \\\hhline{|=|=|====|====|====|====|}
\LARGE \textbf{GM(2D)}& - & -& -&-&  {\LARGE\textbf{2.04}}& -& -& -& {\LARGE\textbf{2.60}}&- &- &- & {\LARGE\textbf{2.19}}& -& -& -& {\LARGE\textbf{2.63}}\\\hhline{|=|=|====|====|====|====|}

\rowcolor{Gray}\cellcolor{white}\multirow{2}{*}{{\LARGE \textbf{3d7pt}}}    
& P & $256\times288\times256$ & $21\%  $& $159.95 $& {\Large\textbf{1.19}}& $256\times160\times256 $& $27\%  $& $99.49  $& {\Large\textbf{1.21}}& $256\times288\times256 $& $0 \%  $& $77.58  $& {\Large\textbf{1.08}}& $128\times128\times128 $& $47\%  $& $56.47  $& {\Large\textbf{1.67}}\\
& F    & $126\times192\times256$ & $100\% $& $274.37 $& {\Large\textbf{2.23}}& $68\times160\times256  $& $100\% $& $212.58 $& {\Large\textbf{3.21}}& $39\times288\times256  $& $100\% $& $146.25 $& {\Large\textbf{2.24}}& $80\times128\times128  $& $100\% $& $98.33  $& {\Large\textbf{2.99}}\\\hline 
\rowcolor{Gray}\cellcolor{white}\multirow{2}{*}{{\LARGE \textbf{3d13pt}}}  
& P & $256\times288\times256 $& $0\%   $& $129.16 $& {\Large\textbf{1.12}}& $256\times320\times256 $& $0\%   $& $86.94 $ & {\Large\textbf{1.06}}& $256\times288\times256 $& $2\%   $& $70.15$  & {\Large\textbf{1.18}}& $256\times320\times256 $& $0\%   $& $41.04  $& {\Large\textbf{1.03}}\\
& F    & $81\times288\times256  $& $100\% $& $152.15 $& {\Large\textbf{1.47}}& $32\times320\times256  $& $100\% $& $137.67$ & {\Large\textbf{2.46}}& $33\times288\times256  $& $100\% $& $92.62$  & {\Large\textbf{1.77}}& $8\times320\times256   $& $100\% $& $46.93  $& {\Large\textbf{1.90}}\\\hline 
\rowcolor{Gray}\cellcolor{white}\multirow{2}{*}{{\LARGE \textbf{3d17pt}}}   
& P & $256\times288\times256 $& $28\%  $& $138.53 $& {\Large\textbf{1.07}}& $160\times160\times256 $& $45\%  $&$ 94.45  $& {\Large\textbf{1.34}}& $256\times288\times256 $& $2\%   $& $75.16$  & {\Large\textbf{1.13}}& $160\times160\times256 $& $13\%  $& $45.54$  & {\Large\textbf{1.40}}\\
& F    & $84\times288\times256  $& $100\% $& $170.66 $& {\Large\textbf{1.51}}& $160\times64\times256  $& $100\% $&$ 131.01 $& {\Large\textbf{2.12}}& $36\times288\times256  $& $100\% $& $87.97$  & {\Large\textbf{1.53}}& $32\times160\times256  $& $100\% $& $64.43$  & {\Large\textbf{2.37}}\\\hline 
\rowcolor{Gray}\cellcolor{white}\multirow{2}{*}{{\LARGE \textbf{3d27pt}}}   
& P & $256\times288\times256 $& $14\%  $& $130.88$ & {\Large\textbf{1.01}}& $160\times160\times256 $& $45\%  $& $94.32  $& {\Large\textbf{1.34}}& $256\times288\times256 $& $5\%   $& $75.22  $& {\Large\textbf{1.14}}& $160\times160\times256 $& $13\%  $& $45.69$  & {\Large\textbf{1.40}}\\
& F    & $81\times192\times256  $& $100\% $& $162.22$ & {\Large\textbf{1.33}}& $160\times64\times256  $& $100\% $& $130.99 $& {\Large\textbf{2.12}}& $33\times288\times256  $& $100\% $& $86.89  $& {\Large\textbf{1.43}}& $32\times160\times256  $& $100\% $& $64.01$  & {\Large\textbf{2.35}}\\\hline 
\rowcolor{Gray}\cellcolor{white}\multirow{2}{*}{{\LARGE \textbf{Poisson}}}  
& P & $256\times288\times256$& $14\%  $& $130.50 $&  {\Large\textbf{1.01}}& $160\times160\times256 $& $30\%  $& $94.70  $& {\Large\textbf{1.35}}& $256\times288\times256 $& $2\%   $& $73.13  $& {\Large\textbf{1.12}}& $160\times160\times256 $& $13\%  $& $45.78  $& {\Large\textbf{1.41}}\\
& F    & $90\times288\times256 $& $100\% $& $164.00 $&  {\Large\textbf{1.45}}& $160\times64\times256  $& $100\% $& $130.89 $& {\Large\textbf{2.12}}& $36\times288\times256  $& $100\% $& $87.59  $& {\Large\textbf{1.54}}& $32\times160\times256  $& $100\% $& $64.92  $& {\Large\textbf{2.39}}\\\hhline{|=|=|====|====|====|====|}
 \LARGE\textbf{GM(3D)}& - & - &- &-&  {\LARGE\textbf{1.30}}& -& -& -& {\LARGE\textbf{1.72}}& -& -& -& {\LARGE\textbf{1.38}}& -& -& -& {\LARGE\textbf{1.80}}\\\hhline{|=|=|====|====|====|====|}
    \end{tabular}
    }
    \label{tab:stencil_speedups}
\end{table*}


==> TABLES/StencilDomain.tex <==
% \begin{table}[t]
%     \centering
%     \caption{Minimum domain sizes that would saturate the device for different benchmarks.}
%     \resizebox{\columnwidth}{!}
%     {%
%     \begin{tabular}{|l|cc|cc|}\hline
%     &\multicolumn{2}{c|}{\textbf{single precision}}&\multicolumn{2}{c|}{\textbf{double precision}}\\
% \textbf{Type}     & \textbf{A100}           & \textbf{V100}           & \textbf{A100}             & \textbf{V100}           \\\hline 
% \textbf{2d5pt}  & $4608\times3072$        & $4096\times2560$        & $2304\times2304$          & $2048\times1280$        \\
% \textbf{2ds9pt}  & $4608\times3072$        & $2560\times2048$        & $2304\times2304$          & $2048\times1280$        \\
% \textbf{2d13pt} & $4608\times3072$        & $2560\times2048$        & $4608\times3072$          & $2048\times2048$        \\
% \textbf{2d17pt} & $4608\times3072$        & $5120\times4096$        & $3072\times2304$          & $4096\times2560$        \\
% \textbf{2d21pt} & $4608\times3072$        & $2560\times2048$        & $4608\times3072$          & $5120\times4096$        \\
% \textbf{2ds25pt} & $4608\times4608$        & $2048\times2048$        & $4608\times4608$          & $5120\times4096$        \\\hline
% \textbf{2d9pt}  & $3072\times3072$        & $2560\times2048$        & $2304\times2304$          & $2048\times1280$        \\
% \textbf{2d25pt} & $4608\times3072$        & $2560\times2048$        & $4608\times3072$          & $2048\times1280$        \\\hline 
% \textbf{3d7pt}   & $256\times288\times256$ & $256\times160\times256$ & $256\times288\times256$   & $128\times128\times128$ \\
% \textbf{3d13pt}  & $256\times288\times256$ & $256\times320\times256$ & $256\times288\times256$   & $256\times320\times256$ \\\hline
% \textbf{3d17pt}  & $256\times288\times256$ & $160\times160\times256$ & $256\times288\times256$   & $160\times160\times256$ \\
% \textbf{3d27pt}  & $256\times288\times256$ & $160\times160\times256$ & $256\times288\times256$   & $160\times160\times256$ \\
% \textbf{poisson}  & $256\times288\times256$ & $160\times160\times256$ & $256\times288\times256$   & $160\times160\times256$ \\\hline
% %\textbf{{merge}}  & $9,753,570$             & $14,148,858$            & $7,339,667$               & $9,753,570$             \\
% %\textbf{{SpMV}}   & (D[15-20])              & (D19,D20)               & (D[15-20])                & (D[15-20])             \\\hline  
%     \end{tabular}
%     }
%     \label{tab:domain}
% \end{table}


\begin{table}[t]
    \centering
    \caption{Minimum domain sizes that would saturate the device for different benchmarks.}
    % \resizebox{\columnwidth}{!}
    {%
    \begin{tabular}{|l|cc|}\hline
    &\multicolumn{2}{c|}{\textbf{double precision}}\\
\textbf{Type}          & \textbf{A100}             & \textbf{V100}           \\\hline 
\textbf{2d5pt}    & $2304\times2304$          & $2048\times1280$        \\
\textbf{2ds9pt}        & $2304\times2304$          & $2048\times1280$        \\
\textbf{2d13pt}      & $4608\times3072$          & $2048\times2048$        \\
\textbf{2d17pt}      & $3072\times2304$          & $4096\times2560$        \\\hline
% \textbf{2d21pt}     & $4608\times3072$          & $5120\times4096$        \\
% \textbf{2ds25pt}       & $4608\times4608$          & $5120\times4096$        \\\hline
\textbf{2d9pt}        & $2304\times2304$          & $2048\times1280$        \\
\textbf{2d25pt}       & $4608\times3072$          & $2048\times1280$        \\\hhline{|=|==|}
\textbf{3d7pt}    & $256\times288\times256$   & $128\times128\times128$ \\
\textbf{3d13pt}   & $256\times288\times256$   & $256\times320\times256$ \\\hline
\textbf{3d17pt}   & $256\times288\times256$   & $160\times160\times256$ \\
\textbf{3d27pt}   & $256\times288\times256$   & $160\times160\times256$ \\
\textbf{poisson}   & $256\times288\times256$   & $160\times160\times256$ \\\hline
%\textbf{{merge}}  & $9,753,570$             & $14,148,858$            & $7,339,667$               & $9,753,570$             \\
%\textbf{{SpMV}}   & (D[15-20])              & (D19,D20)               & (D[15-20])                & (D[15-20])             \\\hline  
    \end{tabular}
    }
    \label{tab:domain}
\end{table}

==> TABLES/stencilbenchs.tex <==
% \begin{table}[t]
%     \centering\small
%     \caption{Stencil benchmarks. A detailed description of the stencil benchmarks can be found in~\cite{zhao2019exploiting,rawat2016effective}}
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{|cccc|}
%     \hline
%         \multicolumn{4}{|c|}{ \textbf{Benchmark(Stencil Order, FLOPs/Cell)}}\\\hline
%         2d5pt(1,10) & 2ds9pt(2,18) & 2d13pt(3,26) & 2d17pt(4,34)\\
%         2d21pt(5,42) & 2ds25pt(6,50)  & 2d9pt(1,18) & 2d25pt(2,50)\\
%         3d7pt(1,14) & 3d13pt(2,26) & 3d17pt(1,34) & 3d27pt(1,54)\\ 
%         poisson(1,38) &---&---&---\\\hline
%     \end{tabular}}
%     \label{tab:stencilbenchmark}
% \end{table}

\begin{table}[t]
    \centering\small
    \caption{Stencil benchmarks. A detailed description of the stencil benchmarks can be found in~\cite{zhao2019exploiting,rawat2016effective}}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{|cccc|}
    \hline
        \multicolumn{4}{|c|}{ \textbf{Benchmark(Stencil Order, FLOPs/Cell)}}\\\hline
        2d5pt(1,10) & 2ds9pt(2,18) & 2d13pt(3,26) & 2d17pt(4,34)\\
        2d9pt(1,18) & 2d25pt(2,50)&3d7pt(1,14) & 3d13pt(2,26)\\
        3d17pt(1,34) & 3d27pt(1,54)&poisson(1,38)&-\\ \hline
    \end{tabular}}
    \label{tab:stencilbenchmark}
\end{table}

==> clschange.tex <==
% \acmISBN{978-x-xxxx-xxxx-x/YY/MM}
\acmISBN{)%978-x-xxxx-xxxx-x/YY/MM}
% \acmDOI{10.1145/nnnnnnn.nnnnnnn}
\acmDOI{}
